Sliding-Window QPS (SW-QPS): A Perfect Parallel Iterative Switching Algorithm for Input-Queued Switches

In this work, we first propose a parallel batch switching algorithm called Small-Batch Queue-Proportional Sampling (SB-QPS). Compared to other batch switching algorithms, SB-QPS significantly reduces the batch size without sacrificing the throughput performance and hence has much lower delay when traffic load is light to moderate. It also achieves the lowest possible time complexity of $O(1)$ per matching computation per port, via parallelization. We then propose another algorithm called Sliding-Window QPS (SW-QPS). SW-QPS retains and enhances all benefits of SB-QPS, and reduces the batching delay to zero via a novel switching framework called sliding-window switching. In addition, SW-QPS computes matchings of much higher qualities, as measured by the resulting throughput and delay performances, than QPS-1, the state-of-the-art regular switching algorithm that builds upon the same underlying bipartite matching algorithm.

==> SW-QPS-PERF2020(arxiv)/libs/common_used_packages.tex <==
%% packages for figures
\usepackage{graphicx}
\usepackage{color}
\usepackage{graphics}

%\usepackage[sort,compress]{cite}
%\usepackage{enumerate}

%% packages for citation
% \usepackage[sort]{cite}
%% for highlighting
%\usepackage{soul}
\newcommand{\st}[1]{}

%% packages for math
%\usepackage{bbm}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
%\usepackage{latexsym}
%\usepackage{mathtools}
%\usepackage{cuted}
% This package reimplements the LATEX verbatim and verbatim* environments.
% In addition it provides a comment environment that skips any
% commands or text between \begin{comment} and the next \end{comment}.
\usepackage{verbatim}


\usepackage{textcomp}
% The pack­age trans­lates var­i­ous stan­dard and other in­put en­cod­ings into a 
% ‘LATEX in­ter­nal lan­guage’. The in­ter­nal lan­guage is ex­pressed en­tirely in
% TEX's base en­cod­ing (stan­dard ASCII print­able char­ac­ters, car­riage con­trol
% to­kens and TEX con­trol se­quences, the lat­ter mostly de­fined by LATEX).
\usepackage[latin1]{inputenc}


%% packages for multirow
\usepackage{multirow}


%% for tables 
\usepackage{booktabs}

%% packages for url
\usepackage{url}

%% newly added
% \usepackage{floatrow}

%% for balanced columns
\usepackage{balance}
% % captions and subcaptions
% % \usepackage[caption=false,position=bottom]{subfig}
% \usepackage{caption}
% % % \let\subcaption\relax
% % % \let\subfloat\relax
% % %\usepackage{subcaption}
% % % \usepackage[caption=false,position=bottom]{subcaption}
% % % \let\subbottom\subfloat % to allow use of \subbottom instead of \subfloat
% % %% comment out since acmart has its own setting
% \captionsetup[figure]{textfont={small}}
% \captionsetup[table]{textfont={small}}
% \captionsetup[subfloat]{textfont={footnotesize},subrefformat=parens}

% hyperlinks, which caused some fof the grief above
%\let\captioncaption\caption
% \usepackage{aliascnt} % for custom autoref
\hypersetup{
	colorlinks = true,
linkcolor=blue,
citecolor=blue,
urlcolor=blue,
pdftitle={Sliding Window QPS}
} % hyperref is load by acmart
%\PassOptionsToPackage{unicode}{hyperref}
% \usepackage[colorlinks,
% linkcolor={red!50!black},
% citecolor={blue!50!black},
% urlcolor={blue!80!black},
% pdftitle={SERENADE}]{hyperref}
%% packages for algorithms
% \usepackage[lined,boxed,linesnumbered,commentsnumbered]{algorithm2e}
\usepackage[lined,boxed,linesnumbered,vlined]{algorithm2e}
% \usepackage{algpseudocode}

% The etoolbox package is a toolbox of programming tools geared primarily towards
% LaTeX class and package authors. It provides LaTeX frontends to some of the new
% primitives provided by e-TeX as well as some generic tools which are not related to
% e-TeX but match the profile of this package.
\usepackage{etoolbox}


% use "autoref" the way I want
%   autoref is nice because the text or brackets of a ref are part of link
%   see http://tex.stackexchange.com/questions/36575/autorefs-inserted-text-has-not-the-correct-case
%       http://en.wikibooks.org/wiki/LaTeX/Labels_and_Cross-referencing
%       http://www.tug.org/applications/hyperref/manual.html#TBL-23

%% define autoref name for sections
% \ifx\sectionautorefname\defined
\def\sectionautorefname{\S\!\!}
\def\subsectionautorefname{\S\!\!}
\def\subsubsectionautorefname{\S\!\!}
% \fi
% from http://tex.stackexchange.com/questions/52410/how-to-use-the-command-autoref-to-implement-the-same-effect-when-use-the-comman
% \ifx\equationautorefname~#1\undefined
\def\equationautorefname~#1\null{%
  (#1)\null
}
% \fi

%% change ref of algorithm from 'algorithm x' to 'Procedure x'
\renewcommand*{\algorithmautorefname}{Procedure}
\renewcommand{\algorithmcfname}{Procedure}% Update algorithm name
\renewcommand{\algorithmcflinename}{Line}
\newcommand*{\subfigureautorefname}{Figure}


%% change alg settings
\setlength{\algomargin}{6mm}
\SetKwInput{Problem}{problem}
\SetKwInput{Input}{input}
\SetKwInput{Output}{output}
\SetAlgoSkip{smallskip} % default
\SetAlgoInsideSkip{smallskip} %
\setlength{\AlCapSkip}{1mm} 
\SetKwComment{tcp}{\#\ }{}
\SetKwComment{tcc}{\#\ }{}
% \SetAlFnt{\small}
% \SetAlCapFnt{\small}
% \SetAlCapNameFnt{\small}
% \SetAlCapHSkip{0pt}
% \IncMargin{-\parindent}
    
%% change theorem style
\usepackage{amsthm}
\newtheoremstyle{saber}% name
  {}%      Space above, empty = `usual value'
  {}%      Space below
  {\itshape}% Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\bfseries}% Thm head font
  {.}%        Punctuation after thm head
  {.5em}% Space after thm head: \newline = linebreak
  {}%         Thm head spec

\theoremstyle{saber}
%% definitions for theorem related environment and their autoref names
\ifcsundef{theorem}{% theorem is not defined yet
\newtheorem{theorem}{Theorem}%[section]
}{}
\ifcsundef{corollary}{%
\newtheorem{corollary}{Corollary}%[theorem]
}{}
\ifcsundef{lemma}{%
\newtheorem{lemma}{Lemma}%[theorem]
}{}
\ifcsundef{definition}{%
\newtheorem{definition}{Definition}%[theorem]
}{}
\ifcsundef{fact}{%
\newtheorem{fact}{Fact}%[theorem]
}{}
\ifcsundef{remark}{%
\newtheorem{remark}{Remark}%[theorem]
}{}
\ifcsundef{property}{%
\newtheorem{property}{Property}%[theorem]
}{}



%% change autoref names for theorem related
\ifx\theoremautorefname\undefined
\newcommand*{\theoremautorefname}{Theorem}
\fi
\ifx\lemmaautorefname\undefined
\newcommand*{\lemmaautorefname}{Lemma}
\fi
\ifx\definitionautorefname\undefined
\newcommand*{\definitionautorefname}{Definition}
\fi
\ifx\corollaryautorefname\undefined
\newcommand*{\corollaryautorefname}{Corollary}
\fi
\ifx\factautorefname\undefined
\newcommand*{\factautorefname}{Fact}
\fi
\ifx\propertyautorefname\undefined
\newcommand*{\propertyautorefname}{Property}
\fi


%% commonly used math commands
\ifx\argmax\undefined
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\fi
\ifx\argmin\undefined
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\fi
\ifx\limsup\undefined
\newcommand{\limsup}{\operatornamewithlimits{limsup}}
\fi
\ifx\liminf\undefined
\newcommand{\liminf}{\operatornamewithlimits{liminf}}
\fi
\ifx\norm\undefined
\newcommand{\norm}[1]{\lVert#1\rVert}
\fi
\ifx\abs\undefined
\newcommand{\abs}[1]{\lvert#1\rvert}
\fi
\ifx\set\undefined
\newcommand{\set}[1]{\left\{#1\right\}}
\fi
\ifx\mset\undefined
\newcommand{\mset}[1]{\lbrack #1\rbrack}
\fi
\ifx\etal\undefined
\newcommand{\etal}[1]{{\em #1 et al.}~}
\fi
\ifx\ie\undefined
\newcommand{\ie}{{\em i.e.,} }
\fi
\ifx\eg\undefined
\newcommand{\eg}{{\em e.g.,} }
\fi
\ifx\etc\undefined
\newcommand{\etc}{{\em etc.,} }
\fi
\ifx\wrt\undefined
\newcommand{\wrt}{{\em w.r.t.} }
\fi
\ifx\dotprod\undefined
\newcommand{\dotprod}[2]{
  \langle #1, #2 \rangle
}
\fi
\ifx\iid\undefined 
\newcommand{\iid}{i.i.d.}
\fi
\ifx\bigParenthes\undefined 
\newcommand{\bigParenthes}[1]{
  \big(#1\big)
}
\fi
\ifx\bigBracket\undefined 
\newcommand{\bigBracket}[1]{
  \big\{#1\big\}
}
\fi
\ifx\bigSqBracket\undefined 
\newcommand{\bigSqBracket}[1]{
  \big[#1\big]
}
\fi
\ifx\BigParenthes\undefined 
\newcommand{\BigParenthes}[1]{
  \Big(#1\Big)
}
\fi
\ifx\BigBracket\undefined 
\newcommand{\BigBracket}[1]{
  \Big\{#1\Big\}
}
\fi
\ifx\BigSqBracket\undefined 
\newcommand{\BigSqBracket}[1]{
  \Big[#1\Big]
}
\fi
\ifx\biggParenthes\undefined 
\newcommand{\biggParenthes}[1]{
  \bigg(#1\bigg)
}
\fi
\ifx\biggBracket\undefined 
\newcommand{\biggBracket}[1]{
  \bigg\{#1\bigg\}
}
\fi
\ifx\biggSqBracket\undefined 
\newcommand{\biggSqBracket}[1]{
  \bigg[#1\bigg]
}
\fi
\ifx\BiggParenthes\undefined 
\newcommand{\BiggParenthes}[1]{
  \Bigg(#1\Bigg)
}
\fi
\ifx\BiggBracket\undefined 
\newcommand{\BiggBracket}[1]{
  \Bigg\{#1\Bigg\}
}
\fi
\ifx\BiggSqBracket\undefined 
\newcommand{\BiggSqBracket}[1]{
  \Bigg[#1\Bigg]
}
\fi
\ifx\bracket\undefined
\newcommand{\bracket}[1]{
  \{#1\}
}
\fi
\ifx\parenthes\undefined
\newcommand{\parenthes}[1]{
  (#1)
}
\fi
\ifx\sqBracket\undefined
\newcommand{\sqBracket}[1]{
  [#1]
}
\fi
\ifx\prob\undefined 
\newcommand{\prob}[1]{\mathbb{P}[#1]}
\fi
\ifx\Prob\undefined 
\newcommand{\Prob}[1]{\mathbb{P}\big[#1\big]}
\fi
\ifx\probb\undefined 
\newcommand{\Probb}[1]{\mathbb{P}\bigg[#1\bigg]}
\fi
\ifx\expect\undefined 
\newcommand{\expect}[1]{\mathbb{E}[#1]}
\fi
\ifx\Expect\undefined 
\newcommand{\Expect}[1]{\mathbb{E}\big[#1\big]}
\fi
\ifx\expectt\undefined 
\newcommand{\expectt}[1]{\mathbb{E}\bigg[#1\bigg]}
\fi
\ifx\walk\undefined 
\makeatletter
\newcommand{\walk}[1]{%
  \@tempswafalse
  \@for\next:=#1\do
    {\if@tempswa\!\!\rightarrow\!\!\else\@tempswatrue\fi\next}%
}
\makeatother
\fi
\ifx\seq\undefined 
\newcommand{\seq}{\!=\!}
\fi
\ifx\sminus\undefined 
\newcommand{\sminus}{\!-\!}
\fi
\ifx\sm\undefined 
\newcommand{\sm}[1]{\!#1\!}
\fi

\ifx\union\undefined
\newcommand{\union}[2]{#1\!\cup\!#2}
\fi

\ifx\hl\undefined 
\newcommand{\hl}[2]{{\color{#1}#2}}
\fi

\ifx\hlb\undefined 
\newcommand{\hlb}[1]{{\color{blue}#1}}
\fi

\ifx\hlr\undefined 
\newcommand{\hlr}[1]{{\color{red}#1}}
\fi

\ifx\hlp\undefined 
\newcommand{\hlp}[1]{{\color{purple}#1}}
\fi

\ifx\hlc\undefined 
\newcommand{\hlc}[3]{{\color{#1}#2 [remark: #3]}}
\fi

%% reduce spacing
\setlength{\textfloatsep}{8.0pt plus 1.0pt minus 2.0pt}
%% Redefining itemize to save space
\ifcsdef{sitemize}{}{
\newenvironment{sitemize}{%
  \begin{list}{$\bullet$}{%
    %\setlength{\rightmargin}{\leftmargin}
    \setlength{\itemsep}{0.1cm}%
    \setlength{\leftmargin}{1.0em}%
    \setlength{\topsep}{0.1cm}%
    \setlength{\parsep}{0mm}}%
  }{\end{list}}
}

\ifcsdef{senumerate}{}{
\newenvironment{senumerate}{%
   \begin{list}{\arabic{enumi}.}{%
    \setlength\labelwidth{3.5em}%
    \setlength\leftmargin{2.5em}%
    \setlength{\topsep}{2pt plus 2pt minus 2pt}%
    \setlength\itemsep{0.0cm}%
    \usecounter{enumi}}%
  }{\end{list}}
}

\ifcsdef{spenumerate}{}{
\newenvironment{spenumerate}{%
   \begin{list}{(\arabic{enumi})}{%
    \setlength\labelwidth{3.5em}%
    \setlength\leftmargin{2.5em}%
    \setlength{\topsep}{2pt plus 2pt minus 2pt}%
    \setlength\itemsep{0.0cm}%
    \usecounter{enumi}}%
  }{\end{list}}
}

\ifcsdef{slenumerate}{}{
\newenvironment{slenumerate}{%
   \begin{list}{(\alph{enumi})}{%
    \setlength\labelwidth{3.5em}%
    \setlength\leftmargin{2.5em}%
    \setlength{\topsep}{2pt plus 2pt minus 2pt}%
    \setlength\itemsep{0.0cm}%
    \usecounter{enumi}}%
  }{\end{list}}
}



%% COPY from internet
%% This part goes in preamble
\newcommand{\dummyfig}[2]{
  \centering
  \fbox{
    \begin{minipage}[t][#1][t]{#2}
      \centering{Dummy figure}
    \end{minipage}
  }
}







==> SW-QPS-PERF2020(arxiv)/libs/figure_confs.tex <==
\def \SerenaDemo {
    \input{figures/serena-demo-new}
}

\def \SerenaDemoSmall {
    \input{figures/serena-demo-new-small}
}

%% comparison for different serenade schemes
% \def \ComparisonSerenade   {\includegraphics[width=\fullup]{figures/v2/serenade_mean_delay_logy_new}}
%% remove hybrid
\def \ComparisonSerenade   {\includegraphics[width=\fullup]{figures/v2/serenade_woh_mean_delay_logy_new}}

==> SW-QPS-PERF2020(arxiv)/libs/packages-macros-for-acm.tex <==
\usepackage{balance}
% % captions and subcaptions
% % \usepackage[caption=false,position=bottom]{subfig}
% \usepackage{caption}
% % % \let\subcaption\relax
% % % \let\subfloat\relax
% % %\usepackage{subcaption}
% % % \usepackage[caption=false,position=bottom]{subcaption}
% % % \let\subbottom\subfloat % to allow use of \subbottom instead of \subfloat
% % %% comment out since acmart has its own setting
% \captionsetup[figure]{textfont={small}}
% \captionsetup[table]{textfont={small}}
% \captionsetup[subfloat]{textfont={footnotesize},subrefformat=parens}

% hyperlinks, which caused some fof the grief above
%\let\captioncaption\caption
% \usepackage{aliascnt} % for custom autoref
\usepackage{hyperref}
\hypersetup{
	colorlinks = true,
linkcolor=blue,
citecolor=blue,
urlcolor=blue,
pdftitle=SW-QPS}
 % hyperref is load by acmart
%\PassOptionsToPackage{unicode}{hyperref}
% \usepackage[colorlinks,
% linkcolor={red!50!black},
% citecolor={blue!50!black},
% urlcolor={blue!80!black},
% pdftitle={SERENADE}]{hyperref}
%% packages for algorithms
% \usepackage[lined,boxed,linesnumbered,commentsnumbered]{algorithm2e}
\usepackage[lined,boxed,linesnumbered,vlined]{algorithm2e}
% \usepackage{algpseudocode}

% The etoolbox package is a toolbox of programming tools geared primarily towards
% LaTeX class and package authors. It provides LaTeX frontends to some of the new
% primitives provided by e-TeX as well as some generic tools which are not related to
% e-TeX but match the profile of this package.
\usepackage{etoolbox}
\usepackage{comment}
% 

% use "autoref" the way I want
%   autoref is nice because the text or brackets of a ref are part of link
%   see http://tex.stackexchange.com/questions/36575/autorefs-inserted-text-has-not-the-correct-case
%       http://en.wikibooks.org/wiki/LaTeX/Labels_and_Cross-referencing
%       http://www.tug.org/applications/hyperref/manual.html#TBL-23

%% define autoref name for sections
% \ifx\sectionautorefname\defined
\def\sectionautorefname{\S\!\!}
\def\subsectionautorefname{\S\!\!}
\def\subsubsectionautorefname{\S\!\!}
% \fi
% from http://tex.stackexchange.com/questions/52410/how-to-use-the-command-autoref-to-implement-the-same-effect-when-use-the-comman
% \ifx\equationautorefname~#1\undefined
\def\equationautorefname~#1\null{%
  (#1)\null
}
% \fi

%% change ref of algorithm from 'algorithm x' to 'Procedure x'
\renewcommand*{\algorithmautorefname}{Procedure}
\renewcommand{\algorithmcfname}{Procedure}% Update algorithm name
\renewcommand{\algorithmcflinename}{Line}
\newcommand*{\subfigureautorefname}{Figure}


%% change alg settings
\setlength{\algomargin}{6mm}
\SetKwInput{Problem}{problem}
\SetKwInput{Input}{input}
\SetKwInput{Output}{output}
\SetAlgoSkip{smallskip} % default
\SetAlgoInsideSkip{smallskip} %
\setlength{\AlCapSkip}{1mm} 
\SetKwComment{tcp}{\#\ }{}
\SetKwComment{tcc}{\#\ }{}
% \SetAlFnt{\small}
% \SetAlCapFnt{\small}
% \SetAlCapNameFnt{\small}
% \SetAlCapHSkip{0pt}
% \IncMargin{-\parindent}
    \begin{comment}
%% change theorem style
\usepackage{amsthm}
\newtheoremstyle{saber}% name
  {}%      Space above, empty = `usual value'
  {}%      Space below
  {\itshape}% Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\bfseries}% Thm head font
  {.}%        Punctuation after thm head
  {.5em}% Space after thm head: \newline = linebreak
  {}%         Thm head spec

\theoremstyle{saber}
%% definitions for theorem related environment and their autoref names
\ifcsundef{theorem}{% theorem is not defined yet
\newtheorem{theorem}{Theorem}%[section]
}{}
\ifcsundef{corollary}{%
\newtheorem{corollary}{Corollary}%[theorem]
}{}
\ifcsundef{lemma}{%
\newtheorem{lemma}{Lemma}%[theorem]
}{}
\ifcsundef{definition}{%
\newtheorem{definition}{Definition}%[theorem]
}{}
\ifcsundef{fact}{%
\newtheorem{fact}{Fact}%[theorem]
}{}
\ifcsundef{remark}{%
\newtheorem{remark}{Remark}%[theorem]
}{}
\ifcsundef{property}{%
\newtheorem{property}{Property}%[theorem]
}{}



%% change autoref names for theorem related
\ifx\theoremautorefname\undefined
\newcommand*{\theoremautorefname}{Theorem}
\fi
\ifx\lemmaautorefname\undefined
\newcommand*{\lemmaautorefname}{Lemma}
\fi
\ifx\definitionautorefname\undefined
\newcommand*{\definitionautorefname}{Definition}
\fi
\ifx\corollaryautorefname\undefined
\newcommand*{\corollaryautorefname}{Corollary}
\fi
\ifx\factautorefname\undefined
\newcommand*{\factautorefname}{Fact}
\fi
\ifx\propertyautorefname\undefined
\newcommand*{\propertyautorefname}{Property}
\fi


%% commonly used math commands
\ifx\argmax\undefined
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\fi
\ifx\argmin\undefined
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\fi
\ifx\limsup\undefined
\newcommand{\limsup}{\operatornamewithlimits{limsup}}
\fi
\ifx\liminf\undefined
\newcommand{\liminf}{\operatornamewithlimits{liminf}}
\fi
\ifx\norm\undefined
\newcommand{\norm}[1]{\lVert#1\rVert}
\fi
\ifx\abs\undefined
\newcommand{\abs}[1]{\lvert#1\rvert}
\fi
\ifx\set\undefined
\newcommand{\set}[1]{\left\{#1\right\}}
\fi
\ifx\mset\undefined
\newcommand{\mset}[1]{\lbrack #1\rbrack}
\fi
\ifx\etal\undefined
\newcommand{\etal}[1]{{\em #1 et al.}~}
\fi
\ifx\ie\undefined
\newcommand{\ie}{{\em i.e.,} }
\fi
\ifx\eg\undefined
\newcommand{\eg}{{\em e.g.,} }
\fi
\ifx\etc\undefined
\newcommand{\etc}{{\em etc.,} }
\fi
\ifx\wrt\undefined
\newcommand{\wrt}{{\em w.r.t.} }
\fi
\ifx\dotprod\undefined
\newcommand{\dotprod}[2]{
  \langle #1, #2 \rangle
}
\fi
\ifx\iid\undefined 
\newcommand{\iid}{i.i.d.}
\fi
\ifx\bigParenthes\undefined 
\newcommand{\bigParenthes}[1]{
  \big(#1\big)
}
\fi
\ifx\bigBracket\undefined 
\newcommand{\bigBracket}[1]{
  \big\{#1\big\}
}
\fi
\ifx\bigSqBracket\undefined 
\newcommand{\bigSqBracket}[1]{
  \big[#1\big]
}
\fi
\ifx\BigParenthes\undefined 
\newcommand{\BigParenthes}[1]{
  \Big(#1\Big)
}
\fi
\ifx\BigBracket\undefined 
\newcommand{\BigBracket}[1]{
  \Big\{#1\Big\}
}
\fi
\ifx\BigSqBracket\undefined 
\newcommand{\BigSqBracket}[1]{
  \Big[#1\Big]
}
\fi
\ifx\biggParenthes\undefined 
\newcommand{\biggParenthes}[1]{
  \bigg(#1\bigg)
}
\fi
\ifx\biggBracket\undefined 
\newcommand{\biggBracket}[1]{
  \bigg\{#1\bigg\}
}
\fi
\ifx\biggSqBracket\undefined 
\newcommand{\biggSqBracket}[1]{
  \bigg[#1\bigg]
}
\fi
\ifx\BiggParenthes\undefined 
\newcommand{\BiggParenthes}[1]{
  \Bigg(#1\Bigg)
}
\fi
\ifx\BiggBracket\undefined 
\newcommand{\BiggBracket}[1]{
  \Bigg\{#1\Bigg\}
}
\fi
\ifx\BiggSqBracket\undefined 
\newcommand{\BiggSqBracket}[1]{
  \Bigg[#1\Bigg]
}
\fi
\ifx\bracket\undefined
\newcommand{\bracket}[1]{
  \{#1\}
}
\fi
\ifx\parenthes\undefined
\newcommand{\parenthes}[1]{
  (#1)
}
\fi
\ifx\sqBracket\undefined
\newcommand{\sqBracket}[1]{
  [#1]
}
\fi
\ifx\prob\undefined 
\newcommand{\prob}[1]{\mathbb{P}[#1]}
\fi
\ifx\Prob\undefined 
\newcommand{\Prob}[1]{\mathbb{P}\big[#1\big]}
\fi
\ifx\probb\undefined 
\newcommand{\Probb}[1]{\mathbb{P}\bigg[#1\bigg]}
\fi
\ifx\expect\undefined 
\newcommand{\expect}[1]{\mathbb{E}[#1]}
\fi
\ifx\Expect\undefined 
\newcommand{\Expect}[1]{\mathbb{E}\big[#1\big]}
\fi
\ifx\expectt\undefined 
\newcommand{\expectt}[1]{\mathbb{E}\bigg[#1\bigg]}
\fi
\ifx\walk\undefined 
\makeatletter
\newcommand{\walk}[1]{%
  \@tempswafalse
  \@for\next:=#1\do
    {\if@tempswa\!\!\rightarrow\!\!\else\@tempswatrue\fi\next}%
}
\makeatother
\fi
\ifx\seq\undefined 
\newcommand{\seq}{\!=\!}
\fi
\ifx\sminus\undefined 
\newcommand{\sminus}{\!-\!}
\fi
\ifx\sm\undefined 
\newcommand{\sm}[1]{\!#1\!}
\fi

\ifx\union\undefined
\newcommand{\union}[2]{#1\!\cup\!#2}
\fi

\ifx\hl\undefined 
\newcommand{\hl}[2]{{\color{#1}#2}}
\fi

\ifx\hlb\undefined 
\newcommand{\hlb}[1]{{\color{blue}#1}}
\fi

\ifx\hlr\undefined 
\newcommand{\hlr}[1]{{\color{red}#1}}
\fi

\ifx\hlp\undefined 
\newcommand{\hlp}[1]{{\color{purple}#1}}
\fi

\ifx\hlc\undefined 
\newcommand{\hlc}[3]{{\color{#1}#2 [remark: #3]}}
\fi

\end{comment}
\newcommand{\ie}{{\em i.e.,} }
%% reduce spacing
\setlength{\textfloatsep}{8.0pt plus 1.0pt minus 2.0pt}
%% Redefining itemize to save space
\ifcsdef{sitemize}{}{
\newenvironment{sitemize}{%
  \begin{list}{$\bullet$}{%
    %\setlength{\rightmargin}{\leftmargin}
    \setlength{\itemsep}{0.1cm}%
    \setlength{\leftmargin}{1.0em}%
    \setlength{\topsep}{0.1cm}%
    \setlength{\parsep}{0mm}}%
  }{\end{list}}
}

\ifcsdef{senumerate}{}{
\newenvironment{senumerate}{%
   \begin{list}{\arabic{enumi}.}{%
    \setlength\labelwidth{3.5em}%
    \setlength\leftmargin{2.5em}%
    \setlength{\topsep}{2pt plus 2pt minus 2pt}%
    \setlength\itemsep{0.0cm}%
    \usecounter{enumi}}%
  }{\end{list}}
}

\ifcsdef{spenumerate}{}{
\newenvironment{spenumerate}{%
   \begin{list}{(\arabic{enumi})}{%
    \setlength\labelwidth{3.5em}%
    \setlength\leftmargin{2.5em}%
    \setlength{\topsep}{2pt plus 2pt minus 2pt}%
    \setlength\itemsep{0.0cm}%
    \usecounter{enumi}}%
  }{\end{list}}
}

\ifcsdef{slenumerate}{}{
\newenvironment{slenumerate}{%
   \begin{list}{(\alph{enumi})}{%
    \setlength\labelwidth{3.5em}%
    \setlength\leftmargin{2.5em}%
    \setlength{\topsep}{2pt plus 2pt minus 2pt}%
    \setlength\itemsep{0.0cm}%
    \usecounter{enumi}}%
  }{\end{list}}
}


==> SW-QPS-PERF2020(arxiv)/sections/abstract.tex <==
\begin{abstract}
% In an input-queued switch, a crossbar schedule, 
% or a matching between the input ports
% and the output ports, needs to be computed for each time slot.
% It is a challenging research problem to design switching algorithms 
% that produce high-quality matchings, 
% yet have a very low time complexity 
% when the switch has a large number of ports.  

In this work, we first propose a parallel batch switching algorithm called Small-Batch Queue-Proportional Sampling (SB-QPS).  
Compared to other batch switching algorithms, SB-QPS significantly reduces the batch size without sacrificing the throughput performance and hence has much lower delay 
when traffic load is light to moderate.  It also 
%and 
achieves
the lowest possible time complexity of $O(1)$ per matching computation per port, via parallelization. 
We then propose another algorithm called Sliding-Window QPS (SW-QPS).  SW-QPS retains and enhances 
all benefits of SB-QPS, and reduces the batching delay to zero via 
a novel switching framework called sliding-window switching. 
%We consider SW-QPS the only research product of this work, since SW-QPS strictly outperforms SB-QPS. 
In addition, SW-QPS computes matchings of much higher qualities, 
as measured by the resulting throughput and delay performances, than QPS-1, the state-of-the-art regular switching algorithm 
that builds upon the same 
underlying bipartite matching algorithm. 
% In this work, we propose two switching algorithms for input-queued switches, namely, 
% Small-Batch QPS (SB-QPS) and Sliding-Window QPS (SW-QPS), that both have the lowest possible computational 
% complexity of $O(1)$. 

% We show, through simulations, that both SB-QPS and SW-QPS have much better throughput 
% performances than the state-of-the-art, and that SW-QPS has better delay performances than the 
% state-of-the-art, under various load conditions and traffic patterns. 
%
% In this work, we propose two algorithms that generate high-quality crossbar schedules fast enough to scale to high-link-rate high-radix packet switches. Our first algorithm, SB-QPS, combines the frameworks of parallel iterative algorithms and batch switching, and our second algorithm, SW-QPS, adopts a novel framework called Sliding Window switching, which solves the batching delay issue of batch switching. Both SB-QPS and SW-QPS has $O(1)$ computational complexity and $O(1)$ communication complexity per port per time slot. We show, through 
% simulations, that SW-QPS achieves at least $90\%$ throughput, 
% and its delay performance is close to that of MWM when the traffic 
% load is not extremely heavy (say $<0.9$) 
% under all the $4$ standard traffic patterns. These salient properties make SW-QPS as excellent 
% candidate switching algorithm that is fast
% enough computationally and can deliver excellent throughput and
% delay performances for high-link-rate high-radix switches. 
\end{abstract}
% \keywords{Sliding-window switching, SW-QPS, SB-QPS}
\keywords{Switching, input-queued switch, bipartite matching}

==> SW-QPS-PERF2020(arxiv)/sections/ack.tex <==
%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
% \section{Acknowledgements}
\smallskip
\noindent
{\bf Acknowledgments.}
This material is based upon work supported by the National Science Foundation under Grant No. CNS-1909048 and CNS-2007006.


==> SW-QPS-PERF2020(arxiv)/sections/background-long.tex <==
% \section{Background}\label{sec:backg}
% % qpsr
% In this section, we provide some background on the switching (crossbar scheduling) problem and the batch switching framework. 
% In this section, we formulate the crossbar switching problem and then briefly introduce the two frameworks of batch switching and sliding window switching, corresponding to our two algorithms SB-QPS and SW-QPS.


\begin{comment}
from qps-r
\end{comment}
% \subsection{Formulation of the Switching Problem}\label{subsec:sys-module}

% \subsection{Assumptions and Problem Models}\label{subsec:sys-module}

% \subsection{Assumptions and Problem Model}\label{sec:sys-module}
\section{Assumptions and Problem Model}\label{sec:sys-module}
\begin{comment}
from serenade

We consider the switching problem of input-queued crossbar switches, which commonly employ Virtual Output Queues (VOQs) to solve the Head-of-Line (HOL) blocking issue~\cite{Karol1987VOQHOL} that severely limits the throughput of input-queued switch systems. In such a $N\times N$ input-queued crossbar switch, each input port has $N$ Virtual Output Queues (VOQs)~\cite{Tamir_HighperformanceMulti_1988}, each of which serves as a dedicated buffer for packets going to one output port. The length of the $j^{th}$ VOQ at input port $i$ is defined as the number of buffered packets from input port $i$ to output port $j$ that are currently waiting for switching.
\end{comment}

% \cite{McKeownMekkittikulAnantharamEtAl1999,McKeown99iSLIP,GiacconePrabhakarShah2003SERENA,qpsr}
In this work, we make the following two assumptions that are widely adopted in the % Mekkittikul98stability,
literature ({\it e.g.,}~\cite{McKeown99iSLIP,Gong_QPSr_2019}). 
First, we assume that all incoming variable-length packets are first segmented into fixed-length packets, 
which are then reassembled before leaving the switch.  Hence, we consider the switching 
of only fixed-length packets in the sequel, and each such fixed-length packet takes exactly one time slot to transmit. 
Second, we assume that input ports, output ports and the crossbar operate at the same speed. 

% \textcolor{green}{[Do we need to reiterate here why we consider input-queued crossbar switches?]}
An $N\times N$ input-queued crossbar can be modeled as a weighted bipartite graph, of which the
two disjoint vertex sets are the $N$ input ports and the $N$ output ports 
respectively.
% Note that we will use ``input/output port'' to stand for the
% vertices in the bipartite graph. For example, we will use ``input port i'' to represent the vertex
% corresponds to input port $i$ in the bipartite graph.
% The edges between those input ports and
% output ports are determined by the lengths of the respective VOQs.
We note that the edge set in this bipartite graph might change from a time slot to another. 
In this bipartite graph during a certain time slot $t$, there is an
edge between input port $i$ and output port $j$, if and only if
% VOQ$_{ij}$,
the $j^{th}$ VOQ at input port $i$,
the corresponding VOQ,
is nonempty (at $t$).  The weight of this edge is defined
as the length of ({\it i.e.,} the number of packets buffered at) this VOQ. 
A set of such edges constitutes a {\it valid crossbar schedule}, or a {\it matching},
if any two of them do not share a common vertex. 
% The weight of a matching
% is the total weight of all the edges belonging to it ({\it i.e.,} the total length of all corresponding VOQs).

% With the assumptions above, the switching problem of an input-queued crossbar switch can be modeled as a weighted matching problem on a bipartite graph that is constructed in the following manner.
% \begin{itemize}
% 	\item The two disjoint vertex sets of this graph are the $N$ input ports and the $N$ output ports, respectively.
% 	\item Each edge (from the vertex of input port $i$ to output port $j$) in this graph correspond to a non-empty VOQ (the $j^{th}$ VOQ at input port $i$). 
% 	\item The weight of each edge equals to the length of its corresponding VOQ.
% \end{itemize}
% A {\it valid crossbar schedule}, or a {\it matching}, consists of edges that do not share a common vertex between any two of them, and the quality (weight) of a matching is defined as the total weight of all the edges belonging to it. The desired switching algorithm solves this problem with a matching of the highest possible quality (maximum possible weight). Under this formulation, MWM is the optimal solution to this switching problem, but because of its high complexity, it cannot be computed within one time slot. Therefore, we design switching algorithms that has low enough complexities to generate one matching per time slot, yet its matchings are still of pretty high quality.

% \subsection{Batch Switching Algorithms}
% \subsection{Batch Switching and Sliding Window Switching}\label{subsec:back-batching}
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.85\columnwidth]{figures/IQ-sched-graph/scheduling-graph-standalone}
% \caption{The joint calendar. ``--" means unmatched.}\label{fig:sched-graph}
% \Description{A joint calendar for batch switching algorithms.}
% \end{figure}

\begin{comment}
\begin{figure}
\centering
\includegraphics[width=0.80\columnwidth]{figures/IQ-sched-graph/scheduling-graph-standalone}
\caption{A joint calendar. ``--" means unmatched.}\label{fig:sched-graph}
\Description{A joint calendar for batch switching algorithms.}
\end{figure}
\subsection{Batch Switching Framework}\label{subsec:back-batching}
As mentioned earlier in~\autoref{subsec:ours},  in a batch switching algorithm, multiple (say $T$) consecutive 
time slots are grouped as a batch and these $T$ matching decisions are batch-computed. 
As shown in~\autoref{fig:sched-graph}, the joint calendar (schedule) of the $N$ output ports over a batch of $T$ time slots can be viewed as a $T \times N$ table with $TN$ cells in it.
Each column corresponds to the calendar of an output port and each row a time slot.  
The content of the cell at the $t^{th}$ row and $j^{th}$ column is the input port that $O_j$ is paired with during time slot $t$. 
For example, in~\autoref{fig:sched-graph}, output port $O_1$ is paired with $I_3$ in time slot $1$, $I_5$ in time slot $2$, and is unmatched 
in time slot $T$.
At each input port, 
all packets that were in queue before a cutoff time (for the current batch), including those that belong to either the current batch, 
or previous batches but could not be served then,
are waiting to be inserted into the respective calendars ({\it i.e.,} columns of cells) of the corresponding output ports.  
In a batch switching algorithm, the goal, 
is to pack as many such packets across the $N$ input ports as possible into the $TN$ cells in this joint calendar.  
Note that the total number of such packets can exceed $TN$, in which case at most $TN$ of them can be served in this batch.   
\end{comment}

% As mentioned in~\autoref{sec:intro}, batch switching algorithms  compute the matchings of $T$ consecutive time slots collectively in {\it joint calendars}. 
% As shown in~\autoref{fig:sched-graph}, a joint calendar of $N$ output ports over a batch of $T$ time slots can be viewed as a $T \times N$ table with $TN$ cells in it, each column of which corresponds to the calendar of an output port and each row of which corresponds to a time slot. The cell at the $t^{th}$ row and $j^{th}$ column contains the input port that matches $O_j$ for time slot $t$. For example, in~\autoref{fig:sched-graph}, output port $O_1$ matches $I_3$ for time slot $1$, $I_5$ for time slot $2$, ..., and is still unmatched for time slot $T$ (shown by a ``--"). The goal of a batch switching algorithm is to pack as many cells in this joint calendar as possible, using all packets that have joined the VOQs before a cutoff time (for the current batch), including those that belong to either the current batch, or previous batches but could not be served till now. Note that the total number of such packets can exceed $TN$, in which case at most $TN$ of them can be served in this batch.   

% Most of the existing batch switching algorithms pack the joint calendar in a centralized manner, which lead to high computation complexities. For example, one approach~\cite{Neely2007FrameBased} resolves the batch switching problem to a graph-algorithmic problem called edge-coloring, whose exact solution has a complexity of $O(N^{1.5}T^2)$ per batch using Birkhoff von Neumann Decomposition (BvND) \cite{vonNeumann53TwoPerson}. Although a parallel batch switching approach with low complexity as $O(\log N)$ per time slot per port has been recently proposed in \cite{Wang2018ParallelEdgeColoring}, it requires a large batch size $T$: $T\!=\!\num{3096}$ for port number $N \!=\! 300$. As explained before, this approach has a drawback of large batching delay when the traffic load is light.

% A straightforward idea to overcome this batching delay issue is to output one matching per time slot while computing the current batch instead of producing $T$ matchings altogether at the end of this batch. Unfortunately, in most of the existing batch switching algorithms, these $T$ matchings are collectively computed and refined, which have high quality at the end of each run of these algorithms. As a result, naively outputting one matching per time slot only generates lower-quality matchings. 

% To steadily generate one high-quality matching at each time slot, we propose a new batch switching framework, called \emph{Sliding Window} (SW) switching. Like a traditional batch switching algorithm, a SW switching algorithm packs the joint calendar that has $TN$ cells during each run, but each run of a SW switching algorithm takes only one time slot (instead of $T$ time slots). At the end of each run, the first row (say  the $t^{th}$ row) of the joint calendar is used for switching and removed from the joint calendar, and an empty schedule for time slot $t+T$ is added, as the last row, to the joint calendar. In this framework, a SW switching algorithm refines each row, 
% except the first $T$ rows in the initial joint calendar, for $T$ times, providing similar quality guarantees to its results as traditional batch switching algorithms. 

% As shown in \autoref{fig:batch-vs-sw}, in contrast to batch switching, as long as there are enough empty positions in the joint calendar, SW switching allows new packets to directly jump to the first row of the joint calendar and to be switched immediately, without having to wait for the beginning of next batch. This flexible behavior, having one matching ready at each time slot, is crucial to the reduction of batching delay to a $O(1)$ order under low traffic loads. Meanwhile, Sliding Window Switching is simple to implement and preserves the advantage of of Batch Switching: achieving high throughput with low complexity. 


==> SW-QPS-PERF2020(arxiv)/sections/background.tex <==
\section{Background}\label{sec:backg}
% qpsr
In this section, we provide a brief introduction to the crossbar scheduling (switching) problem.
%Like the vast majority of other works in the switching
%literature~\cite{Anderson1993PIM,McKeownMekkittikulAnantharamEtAl1999,McKeown99iSLIP},
\begin{comment}
from serenade
\end{comment}
We assume that
all incoming
variable-length packets are segmented into fixed-length packets,
% (sometimes referred to as cells), 
which are then reassembled when \textcolor{green}{ before} leaving the switch.
Hence we consider the switching of only fixed-length packets in the sequel, and each
such fixed-length packet takes exactly one time slot to transmit.
% \modifiedHL{
We also assume that both the output ports and  
the crossbar operate at the same speed as the input ports. 
% }
Both assumptions above are widely adopted in the 
% Mekkittikul98stability,
literature~\cite{McKeownMekkittikulAnantharamEtAl1999,McKeown99iSLIP,GiacconePrabhakarShah2003SerenaJSAC,Gupta09Node}. 


%from serenade
%We assume that all incoming
%variable-size packets are segmented into fixed-size packets,
% (sometimes referred to as cells), 
%which are then reassembled when leaving the switch.
%Hence we consider the switching of only fixed-size packets in the sequel, and each
%such fixed-size packet takes exactly one time slot to transmit.
%\modifiedHL{
%We also assume that both the output ports and  
%the crossbar operate at the same speed as the input ports. 
%}
%Both assumptions above are widely adopted in the 
%literature~\cite {Mekkittikul98stability,McKeownMekkittikulAnantharamEtAl1999,McKeown99iSLIP,GiacconePrabhakarShah2003SerenaJSAC,Gupta09Node}. 
%\modifiedHL{
%Like in~\cite{GiacconePrabhakarShah2003SerenaJSAC}, we further assume that the arrival processes for those 
%fixed-size packets are {\it i.i.d.} Bernoulli. 
%}
\begin{comment}
from qps-r
\end{comment}
\subsection{Input-Queued Crossbar Switch}\label{subsec:sys-module}

%Almost all nowadays switches adopt an input-queued crossbar switch architecture.

In an $N\times N$ input-queued crossbar switch, 
% that
%interconnects $N$ input with $N$ output ports.
%is shown in~\autoref{fig:IQ}.
each input port has $N$ Virtual Output Queues
(VOQs)~\cite{Tamir_HighperformanceMulti_1988}.  The $j^{th}$ VOQ at input port $i$
% , denoted as VOQ$_{ij}$ in the sequel,
serves as a buffer for packets
going from input port $i$ to output port $j$. The use of VOQs solves the Head-of-Line
(HOL) blocking issue~\cite{Karol1987VOQHOL}, which
severely limits the throughput of the
switch system.


An $N\times N$ input-queued crossbar can be modeled as a weighted bipartite graph, of which the
two disjoint vertex sets are the $N$ input ports and the $N$ output ports
respectively.
% Note that we will use ``input/output port'' to stand for the
% vertices in the bipartite graph. For example, we will use ``input port i'' to represent the vertex
% corresponds to input port $i$ in the bipartite graph.
% The edges between those input ports and
% output ports are determined by the lengths of the respective VOQs.
In this bipartite graph, there is an
edge between input port $i$ and output port $j$, if and only if
% VOQ$_{ij}$,
the $j^{th}$ VOQ at input port $i$,
the corresponding VOQ,
is nonempty.  The weight of this edge is defined
as the length of ({\it i.e.,} the number of packets buffered at) this VOQ.
A set of such edges constitutes a {\it valid crossbar schedule}, or a {\it matching},
if any two of them do not share a common vertex. The weight of a matching
is the total weight of all the edges belonging to it ({\it i.e.,} the total length of all corresponding VOQs).

%serenade 

%An $N \!\times\! N$ input-queued crossbar switch is usually modeled as a weighted complete bipartite graph $G(I\bigcup O)$, with
%the $N$ input ports and the $N$ output ports represented as the two disjoint vertex sets $I \!=\! \{I_1, I_2, \dots, I_N\}$ and $O \!=\! \{O_1, O_2, \dots, O_N\}$ respectively.
% \existingHL{
%Each edge
%\footnote{Note that we use $(u, v)$ to represent a undirected edge, and $u\!\rightarrow\!v$ to represent a {\bf directed edge} throughout this paper.} 
% between two vertexes $(I_i, O_j)$
%$(I_i, O_j)$ corresponds to the $j^{th}$ VOQ at input port $i$ and its weight is defined as the number of packets in the VOQ. 
% }
% \addedHL{
%We denote this edge also as $I_i\!\rightarrow\!O_j$ when its direction is emphasized. 
% \modifiedHL{
% Unless otherwise stated, we shall follow the notational convention used in~\cite{Wilson1996GT} 
% for graph-related notations ({\it e.g.,} vertex sets and walks) throughout this paper. 
% }
% }
%(\ie the queue length of VOQ).
%(for $1 \!\le\! i,j \!\le\! N$)

%A valid schedule, or
%\textit{matching}, is a set of edges between $I$ and $O$
%n which no two distinct edges share a vertex.
%The weight of a matching is defined as the total weight of all edges belonging to the matching.
%A vertex is called {\bf matched} if it is an endpoint of an edge in the matching.
% its corresponding input/output port is called as {\bf matched}.  
%therwise the port is {\bf unmatched}. 
%We say that a matching is {\it full} if all vertices in $G(I\bigcup O)$ are an endpoint of an edge in the matching, and is {\it partial} otherwise.
%Clearly, in an $N \!\times\! N$ switch, any full matching contains exactly $N$ edges.  
\subsection{Batch Switching Algorithms}

Since SB-QPS is a batch switching algorithm~\cite{Aggarwal2003EdgeColoring,Neely2007FrameBased,Wang2018ParallelEdgeColoring}, 
we provide some background on it here.
Unlike in a regular switching algorithm, where a matching decision is computed for every time slot, 
in a batch switching algorithm, multiple (say $T$) consecutive time slots are grouped as
a batch and these $T$ matching decisions are batch-computed.  



\begin{wrapfigure}{R}{0.3\textwidth}
	\centering
	\includegraphics[width=0.295\textwidth]{figures/IQ-sched-graph/scheduling-graph-standalone}
	\caption{The joint calendar.}\label{fig:sched-graph}
\end{wrapfigure}

As shown in~\autoref{fig:sched-graph}, the joint calendar (schedule) of the $N$ output ports over a batch of $T$ time slots can be viewed as a $T \times N$ table with $TN$ cells in it.
Each column corresponds to the calendar of an output port and each row a time slot.  
The content of the cell at the $t^{th}$ row and $j^{th}$ column is the input port that $O_j$ is to pair with with during time slot $t$.  
For example, in~\autoref{fig:sched-graph}, output port $O_1$ is paired with $I_3$ in time slot $1$, $I_5$ in time slot $2$, and $I_N$
in time slot $T$.
At each input port, 
all packets that were in queue before a cutoff time (for the current batch), including those that belong to either the current batch, or a previous batch but could not be served then,
are waiting to be inserted into the respective calendars (i.e., columns of cells) of the corresponding output ports.  
In a batch switching algorithm, the goal, 
is to pack as many such packets across the $N$ input ports as possible into the $TN$ cells in this joint calendar.  
Note that the total number of such packets can exceed $TN$, in which case at most $TN$ of them can be served in this batch.   

Most of the existing batch switching algorithms are centralized.  In such algorithms, the switch controller packs this joint calendar for all input and output ports.  
%How to pack this joint calendar can be precisely modeled as a graph-algorithmic problem called edge-coloring. 
\textbf{For example, }an optimal way (generally not unique) of packing the joint calendar can be solved using Birkhoff von Neumann Decomposition (BvND)~\cite{vonNeumann53TwoPerson}, as was 
done in the batch switching algorithm proposed in~\cite{Neely2007FrameBased}, with $O(N^{1.5}T)$ complexity per time slot.
%note that in this particular application (of batch switching), in which the bipartite multigraph (that the crossbar is modeled as) to be edge-colored 
%often either already is or is populated (by adding
%artificial edges to it) into a regular bipartite multigraph (in which every vertex has the same degree), an optimal ({\it i.e.}, using minimum number of colors) edge-coloring
%roughly corresponds to a BvND, and vice versa.  
%%% By Long: here O(N^{1.5}T) should be O(N^{1.5}T^2) and O(N^{1.5}) should be O(N^{2.5})
%However, the computational complexities of BvND-based batching switching algorithms are quite high:  for example $O(N^{1.5}T^2)$ per batch or $O(N^{1.5}T)$ per time slot in~\cite{Neely2007FrameBased} 
%where the classical maximum matching algorithm~\cite{HopcroftKarp1973MSM} is
%used to find each of the $T$ matchings in the BvND;  
Although 
using~\cite{Goel2010PerfectMacthing} or the edge-coloring algorithm proposed in~\cite{cole2001edge} instead of BvND can reduce this asymptotic time complexity slightly, it is not clear whether that
can reduce the execution time.  Furthermore, most of these centralized algorithms cannot be effectively parallelized to reduce their computational complexities per port.  
%Later in \autoref{sec-related}, we will provide a brief survey of batching switching algorithms.

In this paper, we present two switching algorithms, both using small batches of constant size $T$ and having low complexity $O(\log T)$ per time slot. Specifically, in the second algorithm, SW-QPS, we propose a new batch switching framework called Sliding Window Switching, which is compared with Batch Switching in Figure \ref{fig:batch-vs-sw}.
 
\begin{figure}[ht]
	\centering
	\includegraphics[width=0.295\textwidth]{figures/drafts/batch-vs-sw.jpg}
	\caption{Comparison of Batch Switching with Sliding Window Switching.}\label{fig:batch-vs-sw}
\end{figure}

As in the left side of Figure \ref{fig:batch-vs-sw}, each batch in Batch Switching contains $T$ consecutive time slots and different batches do not overlap. The scheduler packs incoming packets into Batch 1 during the period $t+1$ to $t+T$. At time slot $t+T$, all $T$ matchings in Batch 1 become ready for switching and the scheduler moves to Batch 2. 

In Sliding Window Switching, however, consecutive batches overlap on $T-1$ time slots. At time slot $t+1$, the first time slot of the Batch 1 becomes ready for switching and leaves the batch. All other time slots then join Batch 2, together with a new empty time slot appended to the end of Batch 2.

In contrast to Batch Switching, Sliding Window Switching allows new packets to directly jump to the first time slot of the joint calendar and to be switched immediately, without having to wait for the beginning of next batch, as long as there are enough empty positions in the joint calendar. This flexible behavior, having one matching ready at each time slot, is crucial to the reduction of batching delay to a $O(1)$ order under low traffic loads. Meanwhile, Sliding Window Switching is simple to implement and preserves the advantage of of Batch Switching: achieving high throughput with low complexity. 
 

==> SW-QPS-PERF2020(arxiv)/sections/conclusion.tex <==
\section{Conclusion}\label{sec:con}

In this work, we first propose a batch switching algorithm called SB-QPS that significantly reduces the batch size without 
sacrificing the throughput performance much, and achieves 
a time complexity of $O(1)$ 
per matching computation per port via parallelization. 
%To further reduce the batching delay of SB-QPS, 
We then propose a regular switching algorithm called SW-QPS that improves on SB-QPS using a novel sliding-window switching framework. 
SW-QPS inherits and enhances all benefits of SB-QPS and reduces the batching delay to zero. 
We show, through 
simulations, that the throughput and delay performances of SW-QPS are much better than those of QPS-1, the state-of-the-art regular switching algorithm 
based on the same underlying bipartite matching algorithm. 


% two switching algorithms, namely, SB-QPS and SW-QPS, that both have the lowest possible 
% computational complexity: $O(1)$ per port per time slot. 
%
% that generate high-quality crossbar schedules fast enough to scale to high-link-rate high-radix packet switches. Our first algorithm, SB-QPS, combines the frameworks of parallel iterative algorithms and batch switching, and our second algorithm, SW-QPS, adopts a novel framework called Sliding Window switching, which solves the batching delay issue of batch switching. Both SB-QPS and SW-QPS has $O(1)$ computational complexity and $O(1)$ communication complexity per port per time slot. 
% We show, through 
% simulations, that the throughputs of both SB-QPS and SW-QPS are much higher than those of the state-of-the-art, 
% and the delay performances of SW-QPS is better than those of the state-of-the-art, 
% under the $4$ standard traffic patterns. 

% These salient properties make SW-QPS as excellent 
% candidate switching algorithm that is fast
% enough computationally and can deliver excellent throughput and
% delay performances for high-link-rate high-radix switches. 

==> SW-QPS-PERF2020(arxiv)/sections/evaluation-long.tex <==


\section{Performance Evaluation}\label{sec:eva}

In this section, we evaluate, through simulations, the throughput and delay performances of SB-QPS and SW-QPS 
under various load conditions and traffic patterns.  Our algorithms are compared against 
% iSLIP~\cite{McKeown99iSLIP}, a classical switching algorithm that is commonly used in commercial switches, 
% and QPS-r, the state-of-the-art switching algorithm. 
iSLIP~\cite{McKeown99iSLIP}, which runs $\log_2 N$ request-grant-accept iterations and is hence much more
% expensive than our algorithms computationally.
expensive computationally.
Our algorithms are also compared against QPS-1 
(QPS-r with $r$=1 iteration)~\cite{Gong_QPSr_2019}.  This is a fair comparison because QPS-1, like our 
algorithms, runs only a single iteration to compute a matching.  
The MWM algorithm, which delivers near-optimal delay performance~\cite{ShahWischik2006MWM0}, %{Long: Shah and/or Mckeown should have a paper talking about that},
is also compared against as a benchmark. 
% \textbf{why we do not compare with other state-of-art studies.} 

% We have drawn the following three conclusions from the simulations. First, both SB-QPS and SW-QPS have much better throughput 
% performances than QPS-r under the four standard traffic patterns (to be detailed in~\autoref{subsec: sim-setting}). 
% Second, SB-QPS 
% has worse delay performances than all other algorithms, under the light and 
% moderate traffic, and hence it is not as preferable as SW-QPS. 
% Third, the delay performances of SW-QPS   
% are close to those of MWM under the light and moderate traffic, and are generally better than those of SB-QPS, 
% iSLIP (except under the uniform traffic), and QPS-r, the four standard traffic patterns. 

% Our simulations show conclusively the delay and throughput performances of SW-QPS are better than those of SB-QPS and QPS-r under all four traffic patterns, and even better than those of iSLIP under three over four patterns except uniform. 
% \begin{figure*}[!ht]
% 	\centering
% 	\includegraphics[width=0.85\textwidth]{figures/delay_frame.eps}
% 	\caption{Mean delays of SW-QPS with batch sizes 4, 8, 16 and 32 under the $4$ traffic load patterns.}\label{fig: delay-frame2}
% 	\Description{Tuning batch size.}
% \end{figure*}
% \vspace{-10pt}


\subsection{Simulation Setup}
\label{subsec: sim-setting}

In our simulations, we %first 
fix the number of input and output ports $N$ to $64$;  we however will investigate in \autoref{app-sec:delay-vs-port}
how the mean delay performances of these algorithms scale with respect to $N$.
To accurately measure throughput and delay, we assume that each VOQ has an infinite buffer size, so no packet is dropped at any input port. Each simulation run follows the stopping rule in \cite{Flegal2010MCStopRule, Glynn1992MCStopRule}:   The number of time slots simulated is at least $500N^2$ and guarantees the difference between the estimated and the actual average delays to be within $0.01$ time slots with at least $0.98$ probability.

We assume in our simulations that each traffic arrival matrix $A(t)$ is {\it i.i.d.} Bernoulli with its traffic rate matrix  equal to the product of the offered load and a traffic pattern
matrix (defined next). Similar Bernoulli arrivals were studied in  ~\cite{GiacconePrabhakarShah2003SERENA,McKeown99iSLIP,Gong2017QPS}. 
Later, in~\autoref{app-sec: bursty-arrivals-bench}, we will look at burst traffic arrivals. 
% that the traffic arrival processes to different input ports are mutually independent, and each
% such arrival process is {\it i.i.d.}~Bernoulli (\ie at any given input port,
% a packet arrives with a constant probability $\rho \in (0,1)$ during each time slot).
Note that only synthetic traffic (instead of that derived from packet traces) is used in our simulations
because, to the best of our knowledge, there is no meaningful way to combine
packet traces into switch-wide traffic workloads. 
The following four standard types of normalized (with each row or column sum equal to $1$) traffic patterns are used:
%for generating the switch's workloads:
% (I) \emph{Uniform}, (II) \emph{Quasi-diagonal},
% (III) \emph{Log-diagonal}, and (IV) \emph{Diagonal}. For detailed definitions
% of these traffic patterns, please refer to~\cite{GiacconePrabhakarShah2003SERENA,Gong2017QPS}.
% \begin{comment}
(I) \emph{Uniform}: packets arriving at any input port go
to each output port with probability $\frac{1}{N}$.
(II) \emph{Quasi-diagonal}: packets arriving at input port $i$ go to
output port $j \!=\! i$ with probability $\frac{1}{2}$ and go to any other output port
with probability $\frac{1}{2(N-1)}$.
(III) \emph{Log-diagonal}: packets arriving at input port $i$ go
to output port $j = i$ with probability $\frac{2^{(N-1)}}{2^N - 1}$ and
go to any other output port $j$ with probability equal $\frac{1}{2}$ of the
probability of output port $j - 1$ (note: output port $0$ equals output port $N$).
(IV) \emph{Diagonal}: packets arriving at input port $i$ go to
output port $j \!=\! i$ with probability $\frac{2}{3}$, or go to output port
$(i\, \text{mod} \, N) + 1$ with probability $\frac{1}{3}$.
These traffic patterns are listed in order of how skewed the volumes of traffic arrivals to different output
ports are: from uniform being the least skewed, to diagonal being the most skewed.

% \subsection{Selection of Batch Size}

% \begin{figure*}
% 	\centering
% 	\includegraphics[width=0.84\textwidth]{figures/delay_frame}
% 	\caption{Mean delays of SW-QPS with different batch sizes under the $4$ traffic patterns.}\label{fig: delay-frame2}
% 	\Description{Tuning batch size.}
% \end{figure*}
% \subsection{How Large Should Batch Size {\texorpdfstring{$T$}{T}} Be?}\label{subsec:tuning-t}

% When implementing SB-QPS and SW-QPS, we have to first decide the value of batch size $T$. Intuitively, the larger $T$ is, the 
% higher-quality matchings would be produced. However, in practice, we can not use an arbitrary large $T$. 
% On one hand, to keep the computational complexity as low as possible, we should make sure that the 
% $T$-bit-long bitmap can be fit into a single CPU word. On the other hand, as mentioned earlier in~\autoref{subsec:sw-qps}, 
% a larger $T$ means more memory consumptions in both SB-QPS and SW-QPS and furthermore, higher batching delay in SB-QPS. 
% Therefore, we should select a proper value of $T$ that is not too large. 

% We use simulations to decide the value of $T$. In these simulations, 
% we have investigated different values of $T$ varying between $4$ and $32$ for both SB-QPS and SW-QPS. 
% In the interest of space, we only present the simulation results of SW-QPS with four different 
% batch sizes: $4$, $8$, $16$ and $32$; 
% those of SB-QPS are similar. \textcolor{green}{those of SB-QPS are presented in the appendix.} %The results are shown in~\autoref{fig: delay-frame2}. 

% \autoref{fig: delay-frame2} 
% presents the mean delays (in number of time slots) of SW-QPS with the four different batch sizes under the aforementioned four different 
% traffic patterns. 
% %
% \autoref{fig: delay-frame2} clearly shows that the larger the batch size $T$ is, the better the throughput and delay performances are.\textcolor{green}{from delay data, throughput only has 1 precision.}
% \autoref{fig: delay-frame2} also shows that $T$=16 appears to be a sweet point: The throughput increases significantly when $T$ 
% increases from $4$ and $8$ ($7\%$, $6\%$, $5\%$, and $2\%$ under the four traffic patterns respectively) and from $8$ to $16$ ($5\%$, $4\%$, $2\%$, and $1\%$ under the four traffic patterns respectively), whereas increases 
% only slightly when $T$ increases from $16$ to $32$ ($3\%$, $3\%$, $2\%$, and $1\%$ under the four traffic patterns respectively). 
% Similar trends were found for SB-QPS. 
% Hence, we set the batch size $T$ to $16$ in this following simulations in both SB-QPS and SW-QPS. 
% At first, we evaluate the delay performance of SW-QPS schedulers with four different batch sizes: $4$, $8$, $16$ and $32$ and use the results to select the best batch size that balances performance and complexity.

% \autoref{fig: delay-frame2} shows their mean delays (in number of time slots) under the aforementioned four traffic patterns respectively. Each subfigure shows how the mean delay (on a {\it log scale} along the y-axis) varies with the offered load (along the x-axis).

% \begin{figure*}
% 	\centering
% 	\includegraphics[width=0.84\textwidth]{figures/delay_frame}
% 	\caption{Mean delays of SW-QPS with different batch sizes under the $4$ traffic patterns.}\label{fig: delay-frame2}
% 	\Description{Tuning batch size.}
% \end{figure*}

% As  the larger $T$ is, the better the throughput and delay performances are. However, 
% We  make three observations from~\autoref{fig: delay-frame2}. First, when the offered load is no larger than $0.7$, average delays are very low and not affected by batch size, under all four traffic patterns. However, the mean packet delay surges very quickly as the normalized load approaches the critical point where the VOQs becomes unstable\textbf{, which is a common behavior for queueing systems near the critical load.} Second, the maximum sustainable throughputs (where the delays start to ``go through the roof'' in the subfigures) increases with batch size under uniform, quasi-diagonal and log-diagonal traffic, but the difference is less obvious under more skewed traffic patterns. Under the most skewed diagonal traffic, different frame sizes result in almost the same delay curve. \textbf{That is because skewed traffic tend to consume more slots of the joint calendar due to higher contention levels.} Third, the throughput and delay performances of batch sizes $16$ and $32$ are similar. Further increasing batch size only have limited returns. 

% From the results of this experiment, we choose $16$ as the best frame size that balances performance and complexity, which is used in all SB-QPS and SW-QPS schedulers for the rest of our experiments. \textbf{As for delay-sensitive applications where diagonal traffic is rare, it is sometimes advisable to choose higher frame sizes as $32$ for a more stable performance under high loads.}


\begin{comment}

\begin{figure*}
    % \begin{minipage}{\textwidth}
    % \centering
    % \includegraphics[width=\fourfull]{figures/frame_sbqps}
    % \caption{Mean delays of SB-QPS with different batch sizes under the $4$ traffic patterns.}\label{fig: sbqps-batchsize}
    % \Description{Tuning batch size.}
    % \end{minipage}
    \centering
    \begin{minipage}{\textwidth}
    \centering
    \includegraphics[width=\fourfull]{figures/frame_swqps}
    \caption{Mean delays of SW-QPS with different batch sizes under the $4$ traffic patterns.}\label{fig: delay-frame2}
    \Description{Tuning batch size.}
    \end{minipage}
\end{figure*}
\subsection{Tuning the Batch or Window Size {\texorpdfstring{$T$}{T}}}\label{app-sec:tuning-t}

\end{comment}


When implementing SB-QPS and SW-QPS, we have to first decide on the value of batch (for SB-QPS) or window (for SW-QPS) size $T$. 
As explained earlier in~\autoref{sec:intro}, 
for SB-QPS, a larger batch size $T$ generally results in matchings of higher qualities and hence leads to better throughput performances.
However, a larger $T$ results in longer batching delays and hence can lead to worse overall delay performances for SB-QPS.     
In addition, since the availability information in a proposal message is $T$ bits long, a larger $T$ leads to a higher communication complexity for SB-QPS.  
Through simulations (results not shown here in the interest of space), 
we have found that $T = 16$ strikes a nice performance-cost 
tradeoff:   The batching delay is reasonably low and the proposal message size is
small when $T = 16$, yet the throughput gains when increasing $T$ beyond 16 (say to 32) are marginal for SB-QPS.   
Hence we set $T = 16$ for SB-QPS.  SB-QPS clearly deserves its  
name (small-batch) since this tiny batch size of 16 is much smaller than 
that of any other batch switching algorithm.  

Since SW-QPS completely eliminates the batching delay, the only cost of increasing $T$ for SW-QPS is the larger proposal message size.  
Nonetheless, we have found that $T = 16$ is a nice performance-cost tradeoff point, and hence is adopted, also for SW-QPS.  
%Hence we set $T = 16$ for SW-QPS also.    
%Note that for both SB-QPS and 
For SW-QPS, $T$ does not have to grow with $N$ (to deliver similar throughput and delay performances),
as we will show in~\autoref{app-sec:delay-vs-port} that the delay performance of SW-QPS (with $T = 16$) 
does not degrade when $N$ grows larger.   

%The same can be said about SB-QPS.  

\begin{comment}
However, in practice, we can not use an arbitrary large $T$. 
On one hand, to keep the time complexity as low as possible, we should make sure that a 
$T$-bit-long bitmap can be fit into a single or a few CPU words. On the other hand, %as mentioned earlier in~\autoref{subsec:sw-qps}, 
a larger $T$ results in higher message complexities for both SB-QPS and SW-QPS. 
Furthermore, it results in higher batching delay for SB-QPS. 
Therefore, we should decide a proper value of $T$. 

We use simulations to decide the value of $T$. In these simulations, 
we have investigated different values of $T$ varying between $4$ and $32$ for both SB-QPS and SW-QPS. 
% In the interest of space, 
Here, to avoid too many curves in a single figure making it hard to read, 
we only present the simulation results with four different 
batch sizes: $4$, $8$, $16$ and $32$; 
the results for SW-QPS are shown in~\autoref{fig: delay-frame2}. 
In the interest of space, those of SB-QPS are not presented here, since they are similar. 
% In the following, we will only analyze those of SW-QPS, as the analysis for those of SB-QPS is similar.  
% the results for SB-QPS and SW-QPS are shown in~\autoref{fig: sbqps-batchsize} and~\autoref{fig: delay-frame2} respectively. In the following, we will only analyze those of SW-QPS, as the analysis for those of SB-QPS is similar.  
% those of SB-QPS are similar. \textcolor{green}{those of SB-QPS are presented in the appendix.} %The results are shown in~\autoref{fig: delay-frame2}. 




% TODO: explain "missing point"
\autoref{fig: delay-frame2} presents the mean delays, more precisely, the average queueing delays in number of time slots, 
of SW-QPS with the four different batch sizes under the aforementioned four different traffic patterns. 
Each subfigure shows how the mean delay (on a {\it log scale} along the y-axis) varies with the offered load (along the x-axis).  
%

\autoref{fig: delay-frame2} clearly shows that the larger the batch size $T$ is, the better the throughput and delay performances are.
% \textcolor{green}{from delay data, throughput only has 1 precision.}
\autoref{fig: delay-frame2} also shows that $T$=16 appears to be a good enough tradeoff point (for SW-QPS). 
Similarly, we find that $T$=16 is also a good tradeoff point for SB-QPS. 
% be a sweet point: The throughput increases significantly when $T$ 
% increases from $4$ and $8$ ($7\%$, $6\%$, $5\%$, and $2\%$ under the four traffic patterns respectively) and from $8$ to $16$ ($5\%$, $4\%$, $2\%$, and $1\%$ under the four traffic patterns respectively), whereas increases 
% only slightly when $T$ increases from $16$ to $32$ ($3\%$, $3\%$, $2\%$, and $1\%$ under the four traffic patterns respectively). 
% Similar trends were found for SB-QPS. 
Therefore, we set the batch size $T$ to $16$ in both SB-QPS and SW-QPS for all simulations throughout this paper. 

\end{comment}

\begin{figure*}
    \centering
    \includegraphics[width=\fourfull]{figures/comp_qps1}
    \caption{Mean delays of SB-QPS, SW-QPS, iSLIP, QPS-1, and MWM under the $4$ traffic patterns.}\label{fig: delay-load-bench}
    %\Description{Delay vs. load.}
\end{figure*}

\subsection{Throughput Performance Results}\label{subsec:throughput-results}
% \subsection{Throughput and Delay Performances}\label{subsec:results}\label{subsec:throughput-results}\label{subsec:delay-results}

\begin{comment}
\label{subsec: benchmark-performance}
\begin{table}
	% \setlength{\tabcolsep}{2pt}
    \centering 
    \caption{Maximum throughput of SW-QPS, SB-QPS, QPS-r, and iSLIP.}\label{tab:thru-comp}
    \begin{tabular}{@{}|l|c|c|c|c|@{}}
    \hline
    \textbf{Traffic} &  Uniform  & Quasi-diag  &  Log-diag & Diag  \\
    \hline
    \textbf{SB-QPS}& 86.88\% & 87.10\% & 87.31\% & 86.47\% \\
    \hline
    \textbf{SW-QPS} & 92.56\% & 91.71\% & 91.40\% & 87.74\% \\
    \hline 
    \textbf{iSLIP} & 99.56\% & 80.43\% & 83.16\% & 82.96\% \\
    \hline
    \textbf{QPS-r} & 80.51\% & 83.01\% &  84.03\% &84.48\%\\
    \hline
    \end{tabular}%
   
\end{table}
\begin{figure*}
	\centering
	\includegraphics[width=\textwidth]{figures/delay_comparison.eps}
		\caption{Mean delays of SB-QPS, SW-QPS, iSLIP, MWM, and QPS-r under the $4$ traffic load patterns.}\label{fig: delay-load-bench}
\end{figure*}

We then compare the throughput and delay performances of SB-QPS (traditional batch switching), SW-QPS (Sliding Window switching), iSLIP ($\log_2 64$ = 6 iterations), QPS-r ($r=3$ iterations), and MWM (length of VOQ as the weight measure).

\autoref{tab:thru-comp} shows the maximal achievable throughputs of these algorithms under four traffic patterns. It shows that SW-QPS achieves more than $90\%$ throughput under uniform, quasi-diagonal and log-diagonal traffic, and $87\%$ throughput under diagonal traffic, which is higher than SB-QPS and QPS-r. 
In comparison with iSLIP, although SW-QPS cannot achieve $100\%$ throughput under uniform traffic, it achieves higher throughput than iSLIP under the three other traffic patterns.
\end{comment}

% We then compare the maximum achievable throughputs (measured under normalized load $0.9999$) of SB-QPS, SW-QPS, 
% iSLIP ($\log_2 64$=6 iterations), QPS-r ($r=3$ iterations), and MWM (length of VOQ as the weight measure). 
% We use a batch size of $T$=16 in both SB-QPS and SW-QPS, as we will show in~\autoref{app-sec:tuning-t}, it appears to be  
% a sweet spot.

\begin{table}[ht!]
    % \setlength{\tabcolsep}{2pt}
    \centering
    %%% by Long: the convention is to put the caption of tables at the top
    \caption{Maximum achievable throughput.}\label{tab:thru-comp}
    \begin{tabular}{@{}|l|c|c|c|c|@{}}
        \hline
        \textbf{Traffic} &  Uniform  & Quasi-diag  &  Log-diag & Diag  \\
        \hline
        \textbf{SB-QPS}& 86.88\% & 87.10\% & 87.31\% & 86.47\% \\
        \hline
        \textbf{SW-QPS} & 92.56\% & 91.71\% & 91.40\% & 87.74\% \\
        \hline 
        %%%% by Long: suggest to change to >99\%
        \textbf{iSLIP} & 99.56\% & 80.43\% & 83.16\% & 82.96\% \\
        \hline
        \textbf{QPS-1} & 63.54\% & 66.60\% &  68.78\% &75.16\%\\
        %\textbf{QPS-3} & 80.51\% & 83.01\% &  84.03\% &84.48\%\\
        \hline
    \end{tabular}%
    % \caption{Maximum achievable throughput of SW-QPS, SB-QPS, QPS-r, and iSLIP.}\label{tab:thru-comp}
\end{table}

\autoref{tab:thru-comp} presents the maximum achievable throughput of SB-QPS, SW-QPS, iSLIP, and QPS-1, under 
the aforementioned four standard traffic patterns and an offered load close to $1$ (more precisely, 0.9999). 
We do not include the throughout of MWM in~\autoref{tab:thru-comp}, because it can provably attain $100\%$ throughput. 
We make three observations from \autoref{tab:thru-comp}.  First, SW-QPS significantly 
improves the throughput performance of QPS-1, increasing it by an additive term of 
0.2902, 0.2511, 0.2262, and 0.1258 for the uniform, quasi-diagonal, log-diagonal, and diagonal traffic patterns respectively. 
Second, the throughput of SW-QPS is consistently higher than that of SB-QPS under the four traffic patterns. 
Third, under all traffic patterns except uniform, SW-QPS significantly outperforms iSLIP, which is much more expensive computationally as it runs $\log_2 N$ iterations for each matching computation. 
% Moreover, SB-QPS also outperforms iSLIP under 
% all non-uniform traffic patterns. 
% We note that iSLIP is much more expensive computationally than both SW-QPS and SB-QPS. 


\subsection{Delay Performance Results}\label{subsec:delay-results}

\autoref{fig: delay-load-bench} shows the mean delays of SB-QPS, SW-QPS, iSLIP, QPS-1, and MWM 
under the aforementioned four traffic patterns.  As we have shown in~\autoref{subsec:throughput-results}, 
SB-QPS, SW-QPS, iSLIP and QPS-1 generally cannot attain 100\% throughput, so we only measure their delay performances for  
the offered loads under which they are stable; in all figures in the sequel, each ``missing point'' on a plot indicates 
that the corresponding algorithm is not stable under the corresponding traffic pattern and offered load. 
%
\autoref{fig: delay-load-bench} shows that, when the offered load is not very high (say $<0.6$), 
SB-QPS has a much higher mean overall delay than others thanks to its batching delay that is still relatively 
quite high (despite a small batch size of $T = 16$);  in comparison, SW-QPS completely eliminates this batching delay. 
\autoref{fig: delay-load-bench} also shows that SW-QPS outperforms QPS-1 everywhere and outperforms 
iSLIP under all traffic patterns except uniform.  
Since as shown in~\autoref{tab:thru-comp} and~\autoref{fig: delay-load-bench}, the throughput and the delay performances 
of SW-QPS are strictly better than those of SB-QPS, we will show the performance results of only SW-QPS in~\autoref{app-sec:more-results}, 
in which we present more evaluation results.

\begin{comment}
delay performance is better than 
shows that, 
when the offered load is not very high (say $<0.6$), SW-QPS, like iSLIP and QPS-1, 
has low average delays that are close to those of MWM, under all four traffic patterns, 
whereas those of SB-QPS are much higher due to the batching delay. In other words, SW-QPS, unlike 
SB-QPS, does not suffer from the batching delay. 
In addition, 
\autoref{fig: delay-load-bench} also shows that SW-QPS have the best delay performances among these algorithms except MWM. 
\end{comment}


%  of 
% \autoref{sec:eva}. 
% We make three observations from~\autoref{fig: delay-load-bench}. 
% First, when the offered load is not very high (say $<0.6$), SW-QPS, like iSLIP and QPS-1, 
% has low average delays that are close to those of MWM, under all four traffic patterns, 
% whereas those of SB-QPS are much higher due to the batching delay. In other words, SW-QPS, unlike 
% SB-QPS, does not suffer from the batching delay. 
% Second, the maximum sustainable throughputs (where the delays start to ``go through the roof'' 
% in each subfigure in~\autoref{fig: delay-load-bench}) of both SB-QPS and SW-QPS are much higher 
% than those of iSLIP (except under the uniform traffic) and QPS-r, under all four traffic 
% patterns. The additive throughput performance gains of SB-QPS over QPS-r are $6.4\%$, $4.1\%$, $3.3\%$, and $2.0\%$
% for the uniform, quasi-diagonal, log-diagonal, and diagonal traffic patterns, respectively.  
% Those of SW-QPS over QPS-r are even higher, which are $12.0\%$, $8.7\%$, $7.4\%$, and $3.3\%$, respectively. 
% Third, SW-QPS have the best delay performances among these algorithms except MWM. 


% % These observations hold generally under four traffic patterns, although under diagonal traffic, they are not as obvious as under other traffic patterns.
% \begin{enumerate}
% 	\item When the offered load is no larger than $0.5$, all algorithms except SB-QPS have low average delays that are close to each other. The average delay of SB-QPS is much higher than other algorithms due to the batching delay issue, but that issue is eliminated in SW-QPS by the SW switching framework.
% 	\item When the offered load reaches 0.5, MWM starts to have lower delay than SW-QPS, iSLIP and QPS-r. When the offered load reaches $0.7$, SW-QPS starts to perform better than QPS-r and iSLIP (for iSLIP, only under non-uniform traffic). Meanwhile, as the batching delay becomes dominated by queueing delay, SB-QPS outperforms QPS-r and iSLIP (also under non-uniform traffic for iSLIP).
% 	\item As the offered load approaches the maximal throughput of each algorithm, the mean delay surges. Notably, both SB-QPS and SW-QPS are stable even when the offered load is slightly below the maximal throughput. That is because QPS proposing enables our algorithms to generate high-quality matchings without requiring the buildup of long VOQs.

% \end{enumerate}

% Comparing \autoref{tab:thru-comp} and \autoref{fig: delay-load-bench}, we observe that SW-QPS simultaneously achieves higher throughput and lower delay than SB-QPS and QPS-r under all traffic patterns, and iSLIP under non-uniform traffic. SW-QPS is also stable under higher offered load in all the cases above.


\begin{comment}
\subsection{Bursty Arrivals}\label{subsubsec: bursty-arrivals-bench}

In real networks, packet arrivals are likely to be bursty.
In this section, we evaluate the performances of SB-QPS, SW-QPS, iSLIP, MWM, and QPS-r under bursty traffic, generated by a two-state ON-OFF arrival
process described in~\cite{Neely2008DelayMM}.
The durations of each ON (burst) stage and OFF (no burst) stage are
geometrically distributed: the probabilities that the ON and OFF states last for $t \ge 0$ time slots are given by
\begin{equation*}
P_{ON}(t) = p(1-p)^t \text{ and } P_{OFF}(t) = q(1-q)^t,
\end{equation*}
with the parameters $p, q \in (0,1)$ respectively. As such, the average duration of the
ON and OFF states are $(1-p)/p$ and $(1-q)/q$ time slots
respectively.

In an OFF state, an incoming packet's destination (\ie output
port) is generated according to the corresponding load matrix. In an
ON state, all incoming packet arrivals to an input port would be destined
to the same output port, thus simulating a burst of packet
arrivals. By controlling $p$, we can control the desired
average burst size while by adjusting $q$,
we can control the load of the traffic.

We evaluate the mean delay performances of SB-QPS, SW-QPS, iSLIP, MWM, and QPS-r, with the average burst size ranging from $8$ to $1024$ packets, under a lower load lever of $0.6$ and a higher load level of $0.8$. Some data points of the high load figure are missing because corresponding VOQs are not stable. The simulation results are plotted in \autoref{fig: delay-burst60} and \autoref{fig: delay-burst80}. Similar to Bernoulli {\it i.i.d.} arrivals, under bursty arrival, the delay performances of SW-QPS are always better than SB-QPS and QPS-r, but worse than MWM. The difference becomes more significant as the burst size increases. Compared with iSLIP, SW-QPS has lower delay under three over four traffic patterns except the uniform, while it has similar, although slightly higher, delay under uniform traffic.

\begin{figure*}
	\centering
	\includegraphics[width=\textwidth]{figures/burst60.eps}
	\caption{The delay performance of SB-QPS, SW-QPS, iSLIP, MWM, and QPS-r under bursty traffic, medium load $0.6$.}\label{fig: delay-burst60}
\end{figure*}
\begin{figure*}
	\centering
	\includegraphics[width=\textwidth]{figures/burst80.eps}
	\caption{The delay performance of SB-QPS, SW-QPS, iSLIP, MWM, and QPS-r under bursty traffic, high load $0.8$.}\label{fig: delay-burst80}
\end{figure*}
%\begin{figure*}
%	\centering
%	\includegraphics[width=0.95\textwidth]{figures/burst85.eps}
%	\caption{The delay performance of SB-QPS, SW-QPS and MWM under bursty traffic, high load $0.85$.}\label{fig: delay-burst85}
%\end{figure*}

\subsection{Scaling with Port Number}\label{subsubsec:delay-vs-port}
Since our ultimate goal is to achieve efficient packet scheduling on high-radix switches, our algorithm must have high throughput and low delay performance even when the number of ports is high. Therefore, in this experiment, we evaluate delay performances of SB-QPS, SW-QPS, iSLIP, MWM, and QPS-r under normalized load $0.8$ under the aforementioned four traffic patterns, respectively.

We keep the number of input ports equal to that of output ports, which ranges geometrically from $8$ to $512$, and plot the scaling law of mean packet delay with the number of input (or output) ports in \autoref{fig: delay-port}. The data point of $MWM$ with $512$ ports is missing because it takes too much time to compute. 

From ~\autoref{fig: delay-port}, we observe that the mean packet delays of SW-QPS and SB-QPS are almost unaffected by the increase of port number, which means they effectively scale to high-radix switches. SW-QPS performs better than SB-QPS, QPS-r, and iSLIP (not as well as iSLIP under uniform traffic, but the margin is very small) and is even close to MWM under all four traffic patterns. SB-QPS has poor delay performance due to batching delays.

\begin{figure*}
	\centering
	\includegraphics[width=\textwidth]{figures/delay_port.eps}
	\caption{The delay performance of SB-QPS, SW-QPS, iSLIP, MWM, and QPS-r with port number ranging from $8$ to $512$ under load $0.8$.}\label{fig: delay-port}
\end{figure*}
\end{comment}

% \subsection{Scaling with Port Number}\label{app-sec:delay-vs-port}
%     \begin{figure*}
%     \centering
%     \includegraphics[width=\fourfull]{figures/delay_port}
%     \Description{Scaling with port number under an offered load of 0.8.}
%     \caption{Mean delays v.s. port numbers under
%   i.i.d.~Bernoulli traffic arrivals (offered load: $0.8$).}\label{fig: delay-port}
%     \end{figure*}
% % Since our ultimate goal is to achieve efficient packet scheduling on high-radix switches, our algorithm must have high throughput and low delay performance even when the number of ports is high. 
% % Therefore, in this experiment, we evaluate delay performances of SB-QPS, SW-QPS, iSLIP, MWM, and QPS-r under normalized load $0.8$ under the aforementioned four traffic patterns, respectively.
% In this section, we investigate how the mean delays of SB-QPS and SW-QPS scale with the number of input/output 
% ports $N$ under (non-bursty) i.i.d. Bernoulli traffic. Like in~\autoref{sec:eva}, the MWM is also simulated as a benchmark. 
% We have simulated five different $N$ values: $N=8, 16, 32, 64, 128, 256, 512$. 
% \autoref{fig: delay-port} compares the mean delays for SB-QPS, SW-QPS and MWM, under the $4$ different traffic load matrices 
% with an offered load of $0.8$.  The missing points for MWM are because we are not able to obtain its mean delays when $N$=512 in a reasonable amount of time due to its high computational complexity. 
% \autoref{fig: delay-port} shows that the scaling behaviors of SB-QPS and 
% SW-QPS are almost the same as that of MWM in terms of mean delays, for all values of $N$. 
% More precisely, their mean delays are almost independent of $N$. 

==> SW-QPS-PERF2020(arxiv)/sections/evaluation.tex <==
\section{Evaluation}\label{sec:eva}

In this section, we evaluate, through simulations, the performance of
SB-QPS and SW-QPS under various load conditions and traffic patterns.
We compare its \st{delay} performance with
that of iSLIP~\cite{McKeown99iSLIP}, a refined and optimized representative parallel maximal matching
algorithm (adapted for switching).  The \st{delay} performance of the \st{ideal (but computationally
expensive) algorithm} MWM (Maximum Weighted Matching) is also included in the
comparison as a benchmark.  
\textbf{We might need to compare with state-of-art works.}
 Our simulations show bla..bla..
\subsection{Simulation Setup}
\label{subsec: sim-setting}

In our simulations, we fix the number of input/output ports, $N$ to $64$.
%, and the findings are reported
%in \autoref{subsec: delay-vs-port}.
To measure throughput and delay accurately, we assume each VOQ has an infinite
buffer size and hence there is no packet drop at any input port.
Each simulation run is guided by the following stopping
rule~\cite{Flegal2010MCStopRule,Glynn1992MCStopRule}:   The number of time slots simulated is the larger between $500N^2$ and
that is needed
for the difference between the estimated and the actual average delays to be within $0.01$ time slots
with probability at least $0.98$.



% Let $\hat{\sigma}_k$
% be the empirical standard deviation of the average delay up to the $k^{th}$
% time slot, $T^*$ be the minimum simulation effort ({\it i.e.,} number of
% time slots to be simulated), and $\delta$ be the desired half-width of the
% confidence interval. The
% simulation terminates the first time when the following condition holds
% \[
% A\frac{\hat{\sigma}_T}{T} + \delta I_{T\leq T^*} + \frac{1}{T} < \delta.
% \]
% Here $A$ is a Student's t quantile, $T$ is
% number of time slots to be simulated, and
% $I_{T\leq T^*}$ is an indicator, which equals
% $1$ if $T\leq T^*$, otherwise $0$. In all our simulations, we set $A\!=\!2.326$
% ({\it i.e.,} $98\%$ for two-sided when the degree of freedom is $\infty$),
% $T^*\!=\!500N^2$, and $\delta=0.01$.

We assume in our simulations that
each traffic arrival matrix $A(t)$ is Bernoulli {\it i.i.d.} with its traffic
rate matrix $\Lambda$ being equal to the product of the offered load $\rho$ and a traffic pattern
matrix (defined next). Similar Bernoulli arrivals were studied in  ~\cite{GiacconePrabhakarShah2003SERENA,McKeown99iSLIP,Gong2017QPS}.
% that the traffic arrival processes to different input ports are mutually independent, and each
% such arrival process is {\it i.i.d.}~Bernoulli (\ie at any given input port,
% a packet arrives with a constant probability $\rho \in (0,1)$ during each time slot).
\hlb{Note that only synthetic traffic (instead of that derived from packet traces) is used in our simulations
because, to the best of our knowledge, there is no meaningful way to combine
packet traces into switch-wide traffic workloads.}
The following four standard types of normalized (with each row or column sum equal to $1$) traffic patterns are used:
%for generating the switch's workloads:
% (I) \emph{Uniform}, (II) \emph{Quasi-diagonal},
% (III) \emph{Log-diagonal}, and (IV) \emph{Diagonal}. For detailed definitions
% of these traffic patterns, please refer to~\cite{GiacconePrabhakarShah2003SERENA,Gong2017QPS}.
% \begin{comment}
(I) \emph{Uniform}: packets arriving at any input port go
to each output port with probability $\frac{1}{N}$.
(II) \emph{Quasi-diagonal}: packets arriving at input port $i$ go to
output port $j \!=\! i$ with probability $\frac{1}{2}$ and go to any other output port
with probability $\frac{1}{2(N-1)}$.
(III) \emph{Log-diagonal}: packets arriving at input port $i$ go
to output port $j = i$ with probability $\frac{2^{(N-1)}}{2^N - 1}$ and
go to any other output port $j$ with probability equal $\frac{1}{2}$ of the
probability of output port $j - 1$ (note: output port $0$ equals output port $N$).
(IV) \emph{Diagonal}: packets arriving at input port $i$ go to
output port $j \!=\! i$ with probability $\frac{2}{3}$, or go to output port
$(i\, \text{mod} \, N) + 1$ with probability $\frac{1}{3}$.
These traffic patterns are listed in order of how skewed the volumes of traffic arrivals to different output
ports are: from uniform being the least skewed, to diagonal being the most skewed.

==> SW-QPS-PERF2020(arxiv)/sections/intro-longlong.tex <==
\section{Introduction}\label{sec:intro}
% % [Long: faster traffic, large network]
The volume of network traffic across the Internet and in data-centers continues to grow relentlessly,
thanks to existing and emerging data-intensive applications, such as big data analytics, cloud computing,
and video streaming.  At the same time, the number of network-connected devices is exploding,
fueled by the wide adoption of 
%mobile hand-held devices
smart phones and the emergence of the Internet of things.
To transport and ``direct" such massive traffic volume to such a diverse range of destinations, 
switches and routers that are capable of 
connecting a large number of ports (called {\it high-radix} switching \cite{Cakir2015HighRadix, Cakir2016HighRadixCrossbar}) and operating at very high line rates are badly needed. However, the growing line rates and the number of ports are making it increasingly challenging to design the switching algorithm, whose functionality is to generate the crossbar schedule by solving the following matching problem.

% \subsection{Matching Problem}\label{subsec:mp}
\subsection{Matching Problem and Prior Work}\label{subsec:mp}
% % [Long: difficult]
% Most present day switching systems in Internet routers and
% data-center switches employ an input-queued crossbar switch to interconnect the $N$ input ports with the $N$ output ports. 

Many present day switching systems in Internet routers and
data-center switches employ an input-queued crossbar to interconnect their input ports and output ports. In an $N\times N$ input-queued crossbar switch, for each switching cycle or time slot, each input port can only connect to at most one output port and vice versa. In other words, the the connection patterns between input and output ports ({\it i.e.}, the crossbar schedule) is a one-to-one matching. In order to achieve high throughput and low delay performances, the switching algorithm has to generate ``high quality'' matchings, which have high cardinality and low VOQ starvation, as fast as one matching per time slot. 

Unfortunately, it appears to be hard to achieve both high matching quality and low computation complexity as required by high-link-rate high-radix switches. On one hand, Maximum Weighted Matchings (MWM) can achieve 100\% switch throughput and near-optimal queueing delays for various traffic patterns~\cite{McKeownMekkittikulAnantharamEtAl1999}, but each MWM takes $O(N^{2.5}\log W)$ time to compute using the state-of-the-art algorithm~\cite{Duan2012BpMWMScaling}, where
$W$ is the maximum possible length of a VOQ. \textbf{This complexity is too high to scale to high-radix switches.} On the other hand, a family of distributed switching algorithms, called parallel iterative algorithms, have lower computational complexity but worse throughput. A well-known example is iSLIP~\cite{McKeown99iSLIP}, which has $O(\log^2 N)$ per-port computational complexity but cannot attain 100\% throughput except under uniform traffic. Besides, even with hardware optimization, iSLIP has a high communication complexity of $O(N)$ per port in return for its low computational complexity.

Another recent example of parallel iterative algorithms, called QPS-r \cite{Gong_QPSr_2019}, generates each matching with $r$ iterations, each of which consists of two phases: proposing and accepting. In the proposing phase, each input port independently sends a proposal to at most one output port, and then in the accepting phase, each output port independently accepts the received proposals. When multiple proposals are sent to a single output port, at most one proposal can be accepted, and the only accepted proposal will never be changed or canceled. QPS-r has the lowest possible asymptotic complexity of $O(1)$ per port, but in return, it cannot achieve 100\% throughput.  

\begin{figure}[h]
	\centering
	\includegraphics[width=0.455\textwidth]{figures/IQ-sched-graph/scheduling-graph-standalone}
	\caption{A sample joint calendar of port number $N=8$ and batch size $T$: Cells with ``--" are unmatched.}\label{fig:sched-graph}
\end{figure}

Most of the switching algorithms \cite{Anderson1993PIM, McKeown99iSLIP, GiacconePrabhakarShah2003SERENA, AtallaCudaGiacconeEtAl2013BPAssist, Hu2018HRF}, including MWM, iSLIP, and QPS-r, are ``regular" (cycle-by-cycle) algorithms that produce each matching individually in each cycle (time slot), whereas an alternative approach called batch switching \cite{bianco2002frame, rojas2007frame, Aggarwal2003EdgeColoring, Neely2007FrameBased, Wang2018ParallelEdgeColoring, Bianco2004BatchSched} groups multiple (say $T$) consecutive time slots as a batch. Such a batch of matchings, called a {\it joint calendar}, as illustrated in \autoref{fig:sched-graph} as a $T \times N$ table with $TN$ cells, is computed collectively throughout the $T$-time-slot duration of this batch. Each row of the joint calendar, which is a matching for the corresponding time slot, can be packed with packets not only in the corresponding time slot as in regular switching, but in any of the $T$ time slots within the current batch. Therefore, batch switching algorithms can achieve higher throughput than their regular switching counterparts for various traffic patterns ~\cite{bianco2002frame, rojas2007frame}.

However, compared with regular switching algorithms, batch switching algorithms suffer from an additional batching delay of $O(T)$: A packet arriving at the beginning of a batch has to wait till at least the beginning of the next batch to be switched. This $O(T)$ delay is a pronounced issue especially in the following two cases. Firstly, it is unnecessary when the traffic load is low, because in this case even regular switching algorithms can easily achieve packet delay as low as $O(1)$. Secondly, it is unacceptably high in many existing switching algorithms that use a large batch size $T$ to attain high throughputs ({\it e.g.} in ~\cite{Aggarwal2003EdgeColoring}, batch size $T$ is as large as $\omega(N^2)$ ).

In summary, even with the batch switching framework available, designing efficient switching algorithms that achieve excellent throughput and delay performances yet have low computation complexities remains to be a challenging problem.

\subsection{Our Work}\label{subsec:our-work}
To address the aforementioned challenges, we combine parallel iterative algorithms with batch switching algorithms for the advantages of both frameworks: low per-port complexity and high throughput. To achieve this combination, we adopt a \textcolor{green}{novel} accepting strategy, which will be described in \autoref{subsec:sb-qps}. Furthermore, because of the greediness of our accepting strategy, we can break the boundary of batches and propose a new framework called Sliding Window (SW) switching, which solves the batching delay issue of batch switching algorithms.

The result of our study is the following two algorithms: Small-Batch QPS (SB-QPS) and Sliding-Window QPS (SW-QPS), corresponding to the batch switching and SW switching frameworks. The term QPS (short for Queue-Proportional Sampling) refers to an add-on matching technique that is proposed in~\cite{Gong2017QPS} and later extended to a standalone ``regular" parallel iterative matching algorithm called QPS-r~\cite{Gong_QPSr_2019}, whose proposing phase (to be described in in~\autoref{subsec:qps}) is used in both of our algorithms because it has low complexity and delivers high throughput. In fact, besides QPS, both of our algorithms are compatible with any parallel iterative switching algorithm with greedy packing schemes.

Our first algorithm, SB-QPS, has two features over previous works. The first feature is that it is fully distributed with low complexity. Most of the existing batch switching algorithms \cite{Aggarwal2003EdgeColoring, Neely2007FrameBased, Wang2018ParallelEdgeColoring} model the process to pack the joint calendar as an edge-coloring problem, but until now, all practical solutions to the latter problem are centralized and have high complexity. In contrast, SB-QPS is a fully distributed parallel iterative algorithm that resembles QPS-r, having a much lower $O(1)$ computation complexity per port per time slot, in contrast to the Birkhoff von Neumann Decomposition (BvND)-based algorithm in \cite{Neely2007FrameBased} that has $O(N^{1.5}T)$ complexity per time slot.

The second feature of SB-QPS is that it reduces batching delay without sacrificing too much throughput. As we have mentioned above, batching delay is proportional to batch size, but larger batch sizes, associated with more chances to refine the joint calendar, are essential for the high throughput performances of previous batching algorithms. Because of the high efficiency of the QPS proposing scheme and our greedy accepting scheme, SB-QPS only requires a small number of refinements to achieve at least 87\% throughput under all four traffic patterns, reducing its batch size to a small number $T$ that is independent to $N$. Therefore, it has significantly low batching delay compared with the algorithm in \cite{Aggarwal2003EdgeColoring}, whose batch size is $\omega(N^2)$.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.295\textwidth]{figures//IQ-sched-graph/sliding-schedule}
	\caption{An illustration of the joint calendar of Sliding Window switching: The label of each row (matching) is its time slot of completion.}\label{fig:batch-vs-sw}
\end{figure}

Our second algorithm, SW-QPS, is based on a new switching framework called \emph{Sliding Window (SW) switching}, which aims for overcoming the batching delay issue of batch switching algorithms. In the sliding window framework, at arbitrary time slot $t$, the scheduler also refines a joint calendar of $T$ matchings as in batch switching, shown as the bold frame in \autoref{fig:batch-vs-sw}. However, unlike batch switching, these $T$ matchings are not finalized all together at the end of this batch but at different time slots ranging from $t$ to $t+T-1$, one matching per time slot. 

We use the following analogy to illustrate the evolution of the joint calendar in a sliding window algorithm. An $N\times N$ crossbar switch can be viewed as a school with $N$ teachers (input ports) and $N$ departments (output ports), and the row (matching) that is finalized at time slot $t$ is referred to as Class $t$. Each cell (entry with fixed time slot and output port in the joint calendar) is a student, who needs to finish one course required by his corresponding department to receive a degree. Such a course may be taught by any teacher, but one teacher can only teach one student one course at each time slot. 

In the setting above, at an arbitrary time slot $t$, the joint calendar contains students of $T$ different grades from Class $t$ to Class $t+T-1$, shown as the bold frame in \autoref{fig:batch-vs-sw}. Students of Class $t$ are enrolled at the beginning of time slot $t-T+1$, when the joint calendar covers Class $t-T+1$ to Class $t$ (the first three rows of \autoref{fig:batch-vs-sw}), and have $T$ time slots to take the degree course before graduating at the end of time slot $t$. After the graduation of Class $t$, the joint calendar moves one time slot downwards to cover Classes $t+1$ to $t+T$ (the last four rows of \autoref{fig:batch-vs-sw}). 

As is mentioned above, a desirable switching algorithm achieves both high throughput and low delay. In order for high throughput, it maximizes the ratio of granted input requests, which is equivalent to matching many student as possible for courses given the teachers' schedules, and in order for low delay, it minimizes the waiting time from granting to switching, which is the time interval for a student from taking a degree course to graduation. Sliding window switching addresses both objectives by giving each teacher $T$ classes of students as candidates for the courses and giving priority to senior students who will graduate soon to take these courses. Therefore, it gets the better of both worlds:  
low packet delay comparable to regular switching and high throughput comparable to batch switching.

SW-QPS is a fully distributed iterative algorithm, which is an adaptation of SB-QPS to sliding window switching with same operations in the two phases of each time slot. As in \autoref{sec:eva},it achieves 87\% throughput under diagonal traffic, and over 90\% throughput under other three traffic patterns with only $O(1)$ computational complexity per port per time slot. It also has excellent delay performance that is close to that of MWM when the traffic load is under $0.8$. In comparison, iSLIP~\cite{McKeown99iSLIP}, a well-known parallel iterative regular switching algorithm, can only attain roughly $80\%$ throughput under the $4$ standard traffic patterns except the uniform traffic and as mentioned earlier, it has a computational complexity of $O(\log^2 N)$ per port and a communication complexity of $O(N)$ per port. 

% \textbf{Our contributions}

The rest of this paper is organized as follows. In \autoref{sec:backg}, we provide some
background on the input-queued crossbar switches, batch switching and sliding-window \textcolor{green}{SW} switching.  
In \autoref{sec:schemes},  we first review
QPS, and then we describe our schemes: SB-QPS and SW-QPS. 
Then we evaluate the performance of our schemes in~\autoref{sec:eva}. 
In~\autoref{sec:related}, we survey
related work before concluding this paper in~\autoref{sec:con}.

==> SW-QPS-PERF2020(arxiv)/sections/intro-verylong.tex <==
\section{Introduction}\label{sec:intro}
\begin{comment}


% % [Long: faster traffic, large network]
The volume of network traffic across the Internet and in data-centers continues to grow relentlessly,
thanks to existing and emerging data-intensive applications, such as big data analytics, cloud computing,
and video streaming.  At the same time, the number of network-connected devices is exploding,
fueled by the wide adoption of 
%mobile hand-held devices
smart phones and the emergence of the Internet of things.
To transport and ``direct" such massive traffic volume to such a diverse range of destinations, 
switches and routers that are capable of 
connecting a large number of ports (called {\it high-radix} switching~\cite{Cakir2015HighRadix, Cakir2016HighRadixCrossbar}) and operating at very high line rates are badly needed. 
Motivated by this rapidly growing need, much research has been devoted to, and significant breakthroughs
made, on the hardware designs for fast high-radix switching fabrics recently ({\it e.g.},~\cite{Cakir2016HighRadixCrossbar,Dai2017HighRadix}). Indeed,
these recent breakthroughs have made fast high-radix switching hardware not only technologically feasible
but also economically and environmentally (more energy-efficient) favorable, as compared to low-radix
switching hardware~\cite{Cakir2016HighRadixCrossbar}.
% However, the growing line rates and number of ports results in a challenging algorithmic problem: Switching algorithms are forced to generate ``high-quality" crossbar schedules under increasingly strict complexity restrictions.

% \subsection{Matching Problem}\label{subsec:mp}
\subsection{Matching Problem and Prior Work}\label{subsec:mp}
% % [Long: difficult]
% Most present day switching systems in Internet routers and
% data-center switches employ an input-queued crossbar switch to interconnect the $N$ input ports with the $N$ output ports. 
\end{comment}

Many present day switching systems in Internet routers and data-center switches employ 
an input-queued crossbar to interconnect their input ports and output ports. 
In an $N\times N$ input-queued crossbar switch, 
each input port has $N$ Virtual Output Queues
(VOQs). A VOQ $j$ at input port $i$ serves as a buffer for the packets
going into input port $i$ destined for output port $j$. The use of VOQs solves the Head-of-Line
(HOL) blocking issue~\cite{KarolHluchyjMorgan1987HOL}, which
severely limits the throughput of input-queued switches.

% In an $N\times N$ input-queued crossbar switch, for each switching cycle or time slot, 
% each input port can only connect to at most one output port and vice versa. 
% In other words, the the connection patterns between input and output ports ({\it i.e.}, the crossbar schedule) 
% is a one-to-one matching, and the functionality of the switching algorithm is to 
% generate ``high quality'' matchings as fast as one matching per time slot. 
% The quality of the matchings is formalized in \autoref{subsec:sys-module} as the total weight 
% of its edges in a bipartite graph model, and empirically, 
% high-quality matchings are required by the switches to deliver high 
% throughput and low delay, especially under heavy traffic loads.
In an $N\times N$ input-queued crossbar switch, each input port can be connected to only one output
port and vice versa in each switching cycle or time slot.
Hence, in every time slot, the switch needs to compute
a one-to-one \textit{matching} ({\it i.e.}, the crossbar schedule) between input and output ports .
A major research challenge
of designing high-link-rate 
% Cakir2015HighRadix,
switches with a large number of ports (called {\it high-radix}~\cite{Cakir2016HighRadixCrossbar}) 
is to develop switching algorithms that can
compute ``high quality'' matchings -- those that result in
high switch throughput and low queueing
delays for packets -- in a short time slot.

%Clearly, with such a stringent (matching) computational time constraint, only a parallel iterative algorithm can possibly fit the bill.  

%It is apparently  to design a serial (i.e., not parallel) switching algorithm for high-radix high-link-rate switches.  

% Unfortunately, there appears to be a (folklore) tradeoff 
% between the quality of a matching and the amount of 
% time needed to compute it ({\it i.e.,} time complexity). 
% For example, %when used for crossbar scheduling, 
% using Maximum Weighted Matchings (MWM) as crossbar schedules
% %, with a suitable weight measure,
% is known to result in 100\% switch throughput and
% near-optimal 
% queueing delays for various traffic patterns~\cite{McKeownMekkittikulAnantharamEtAl1999}, but
% %For a switch with $N$ input/output ports, however,
% each MWM takes $O(N^{2.5}\log W)$ time to compute using the state-of-the-art algorithm~\cite{Duan2012BpMWMScaling}, where
% $W$ is the maximum possible length of a VOQ.  

% Unfortunately, it appears hard to achieve both high matching quality and low computation complexity as is required by high-link-rate high-radix switches. On one hand, Maximum Weighted Matchings (MWM) are of the highest possible quality and can achieve 100\% switch throughput and near-optimal queueing delays for various traffic patterns~\cite{McKeownMekkittikulAnantharamEtAl1999}, but each MWM takes $O(N^{2.5}\log W)$ time to compute using the state-of-the-art algorithm~\cite{Duan2012BpMWMScaling}, where
% $W$ is the maximum possible length of a VOQ. \textbf{This complexity is too high to scale to high-radix switches.} On the other hand, a family of distributed switching algorithms, called parallel iterative algorithms, have lower computational complexity but produce matchings of lower quality. A well-known example is iSLIP~\cite{McKeown99iSLIP}, which has $O(\log^2 N)$ per-port computational complexity but cannot attain 100\% throughput except under uniform traffic. In addition, even with hardware optimization, iSLIP has a high communication complexity of $O(N)$ per port in return for its low computational complexity.

\subsection{Existing Approaches}\label{subsec:existing}



While %considerable research was performed on switching, %around the turn of the century, 
many switching algorithms have been proposed for input-queued switches, 
%they appear to fall into a (folklore) tradeoff 
%between the quality of a matching and the amount of 
%time needed to compute it ({\it i.e.,} computational complexity): 
%These algorithms 
they either have a (relatively) high time complexity that 
prevents a matching computation from being completed in a short time slot, or cannot produce high-quality matchings 
that translate into 
excellent throughput and delay performances.   For example, the widely-used iSLIP algorithm~\cite{McKeown99iSLIP} 
can empirically achieve over 80\% throughputs under most of traffic patterns, as will be shown in~\autoref{subsec:throughput-results}.   
However, even with 
a parallel iterative implementation, its time complexity per port is $O(\log^2 N)$, which is still
too high when the switch size $N$ is large and the time slot is short (say a few nanoseconds long).  


%For example, among all switching algorithms 
%that can provably guarantee 100\% throughput under all traffic patterns, SERENA~\cite{} has the lowest time complexity of $O(N)$ 
%per matching computation, but this complexity is still too high when the switch size $N$ is large and the time slot is short (say a few %nanoseconds long).  

%Although this complexity is asymptotically the lowest possible for a centralized algorithm (since just to ``write down" the computed matching takes $O(N)$ time),

%One possible approach to get around this apparent 

%It is possible to obtain a better tradeoff between the time complexity and the matching quality through batch 

%A family of batch switching algorithms 

It is possible to improve the quality of the matching without increasing the time complexity of the switching algorithm using a strategy 
called batching~\cite{Aggarwal2003EdgeColoring,Neely2007FrameBased,Wang2018ParallelEdgeColoring}. 
%obtain a better tradeoff between the time complexity and the matching quality using so-called 
%batch switching algorithms~\cite{Aggarwal2003EdgeColoring,Neely2007FrameBased,Wang2018ParallelEdgeColoring}.
Unlike in a regular switching algorithm, where a matching decision is computed for every time slot, 
in a batch switching algorithm, multiple (say $T$) consecutive time slots are grouped as
a batch and these $T$ matching decisions are batch-computed.  Hence, in a batch switching algorithm, each of the $T$ matchings-under-compuation in a batch
has a period of $T$ time slots to find opportunities to have the quality of the matching 
improved by the underlying bipartite matching algorithm, 
whereas in a regular switching algorithm, each matching has only a single time slot to find such opportunities.  
As a result, a batch switching algorithm can usually produce matchings of 
higher qualities than a regular switching algorithm using the same underlying bipartite matching algorithm, 
because such opportunities for improving the quality of a certain matching usually do not all present 
themselves in a single designated time slot (for a regular switching algorithm to compute this matching).   
Intuitively, the larger the batch size $T$ is, the better the quality of a resulting matching is, since 
a larger $T$ provides a wider ``window of opportunities" for improving the quality 
of the matching as just explained.  
%We will highlight this subtle point a few times in the sequel.  

\begin{comment}
Since the $T$ tasks of computing the $T$ matchings often have overlapping subtasks, 
the batch-computation of these $T$ matchings
can have lower time complexity than
$T$ independent matching computations.  As a result, for computing matchings of similar quality, 
the amortized (over the $T$ time slots) time complexity of a batch switching
algorithm can be lower than that of a regular switching algorithm. We will elaborate on this point in ???.
\end{comment}

However, existing batch switching algorithms are not without shortcomings.  
They all suffer from at least one of the following two problems.
First, all existing batch switching algorithms except~\cite{Wang2018ParallelEdgeColoring} are 
serial algorithms and it is not known whether any of them can be parallelized.
As a result, they all have a time complexity of at least $O(N)$ per matching computation, 
since it takes $O(N)$ time just to ``print out" the computed result.  
This $O(N)$ time complexity is clearly too high for high-radix high-line-rate switches as just explained.  
%% all --> most
Second, most existing switching algorithms require a large batch size $T$ to produce high-quality matchings 
that can lead to high throughputs, as will be elaborated in~\autoref{sec:related}. For example, 
%although among them, ??? requires the smallest asymptotic batch size of $O(\log N)$, the constant 
%factor within the Big-O is gigantic:
% 3,000    
it was reported in~\cite{Wang2018ParallelEdgeColoring} that the batch size had to be \num{3096} 
(for $N\!=\!300$ ports) for the algorithm to attain 96\% throughputs under some
traffic patterns.   A large batch size $T$ is certain to lead to poor delay performance: 
Regardless of the offered load condition, the average packet delay for any batch switching algorithm due to batching 
is at least $T/2$, since 
any packet belonging to the current batch has to wait till at least the beginning of the next batch to be switched.

\subsection{Our Contributions}

The first contribution of this work is a novel batch switching algorithm, called SB-QPS (Small-Batch QPS), 
that addresses both weaknesses of existing batch switching algorithms.  
First, it can attain a high throughout of over 85\%, under various traffic load patterns, 
using only a small batch size of $T = 16$ time slots.  This much smaller batch size translates into much better delay 
performances than those of existing batch switching algorithms, as will be shown in~\autoref{subsec:delay-results}.  
Second, SB-QPS is a fully distributed algorithm so that the matching computation load can be efficiently 
divided evenly across the $2N$ input and output ports.
As a result, its time complexity is the lowest possible:  $O(1)$ per matching computation per port.  

The design of the SB-QPS algorithm is extremely simple.  Only $T$ rounds of request-accept message exchanges 
by the input and the output ports are required for computing the $T$ matchings used (as the crossbar configurations) 
in a batch of $T$ time slots.  In each round, each input port $i$ sends a pairing request to an output port that is
sampled (by input port $i$) in a random queue-proportional fashion:  Each output port $j$ is sampled with a probability proportional to the
length of the corresponding VOQ. %$VOQ(i, j)$.  
For this reason, we call this algorithm small-batch QPS (queue-proportional sampling).  
Since each QPS operation can be performed in $O(1)$ time using a simple data structure as shown in~\cite{Gong2017QPS}, 
the time complexity 
of SB-QPS is $O(1)$ per matching computation per port.  As will be explained in~\autoref{subsec:sb-qps-alg}, 
the way QPS is used in this work (SB-QPS) is very different than 
that in~\cite{Gong2017QPS}.  
For one thing, whereas in~\cite{Gong2017QPS} QPS is used as an auxiliary component to other switching algorithms such as iSLIP~\cite{McKeown99iSLIP} and SERENA~\cite{GiacconePrabhakarShah2003SERENA}, 
in this work, QPS serves the primary building block for SB-QPS.

Even though SB-QPS has a much smaller batching delay than other batch switching algorithms due to its much smaller $T$, 
the batching delay accounts for the bulk of the total packet delay under light to moderate traffic loads, when all other delays are
comparatively much smaller.  The second contribution of the work is to achieve the unthinkable:  a novel switching algorithm
called SW-QPS (SW for sliding window) that inherits and enhances all the good features of SB-QPS yet pays zero batching
delay.  More precisely, it has the same $O(1)$ 
time complexity as and achieves strictly better throughput and delay performances than SB-QPS.  


%As just mentioned, SW-QPS is a strict improvement over SB-QPS.  It reduces the batching delay to 0 and delivers higher throughputs than SB-QPS.  
%It inherits all advantages of ???.  It does not pay $O(T)$ delay penalty that dogs all 
%batching algorithms.  Its throughput is even higher than SB-QPS.  
SW-QPS does so by 
solving the switching problem under a novel framework
called {\it sliding-window switching}.  A sliding-window switching algorithm is different than a batch algorithm only in the following aspect.  
In a batch switching algorithm, a batch of $T$ matchings are produced every $T$ time slots.
% (say at the end of
%$T^{th}$ cycle, $2T^{th}$ cycle, and so on).  
In contrast, in a sliding-window switching algorithm, each window is still of size $T$ but 
a single matching is produced every time slot just like in a regular switching algorithm.   More precisely, at the beginning
of time slot $t$, the sliding window contains matchings-under-computation for the $T$ time slots $t$, $t+1$, $\cdots$, $t + T - 1$.   
The ``leading edge of the window", corresponding to the matching for the time slot $t$ (the ``senior class"), ``graduates" and is used as the crossbar configuration for the current time slot $t$.   
Then at the end of time slot $t$, a new and currently empty matching is added to the ``tail end of the window" as the ``freshman class".  
This matching 
will be computed in the next $T$ time slots and hopefully becomes a high-quality matching by the time $t + T$, when it ``graduates".  
SW-QPS completely removes the batching delay because ``it graduates a class every year" and furthermore always schedules an incoming packet to ``graduate"
at the earliest ``year" possible.

We consider SW-QPS to be the only research outcome of this work, since it strictly outperforms SB-QPS.  However, we describe both SB-QPS and SW-QPS
in detail for two reasons.  First, the incremental contributions of SB-QPS over existing batch switching algorithms and that of SW-QPS over SB-QPS are orthogonal 
to each other:  The former is to significantly reduce the batch size without sacrificing the throughput performance much and to reduce the time complexity to 
$O(1)$ via parallelization, whereas the latter is to retain the 
full benefits of batching without paying the batching delay.  Second, thanks to this orthogonality, explaining the 
differences between SB-QPS and existing batch switching algorithms and
that between SW-QPS and SB-QPS separately and incrementally makes the presentation much easier, as will become apparent in~\autoref{sec:sb-qps} and~\autoref{sec:sw-qps}.


\begin{comment}


========= xu stops here ===============

%This matching, which corresponds to the time slot $t + T$, 
%will be updated in the next $T$ cycles and hopefully populated into a high-quality matching by the time $t + T$, when it ``graduates" from the sliding window.  







The second algorithm solves the switching problem under a new framework, 
called the {\it sliding-window (SW) switching}, that is first proposed in this work. This new switching framework will be 
detailed in~\autoref{sec:sws}. All existing works are based on 
either the regular or the batching switching frameworks and fall victim to the following two extremes. On one hand, regular 
switching algorithms consider only a single time slot during the matching computation 
and produce one matching per time slot. Such a matching usually has a relatively low quality except in the cases where 
matchings are computed by an impractical high-computational-complexity regular switching algorithm, 
such as the Maximum Weighted Matching (MWM) algorithm. 
% \textcolor{green}{not really?? MWM has high quality}
On the other hand, batch switching algorithms consider multiple (say $T$) consecutive time slots ({\it i.e.,} a batch) during 
the matching computation, and produce $T$ matchings, all at once, per batch. 
As explained earlier, such matchings usually have higher qualities. 
However, these matchings are not produced in a ``timely'' manner. As a result, a packet arriving at the beginning of 
a batch has to wait till at least the beginning of the next batch to be switched. 
This causes additional delay that is often referred to as the 
{\it batching delay}. This batching delay can result in unnecessarily high packet
delay when the traffic is light or moderate. The SW switching framework falls between the above two extremes: SW switching algorithms consider multiple time slots during the matching computation and produce one matching 
per time slot. Therefore, they can produce high-quality matchings in a timely manner. 

The second algorithm, called SW-QPS, also builds upon QPS-r and is the first SW switching 
algorithm that fully exploits the advantages of the new SW switching framework. SW-QPS 
gets the better of both worlds: 
It can attain similar or even higher throughput than SB-QPS, yet it does not suffer from the batching delay. 






%[say something about its communication complexity???]


the total time complexity of computing the batch of $T$ matchings is the lowest possible:  $O(NT)$ 

does not suffer from any of these two drawbacks.  

Since SW-QPS is based on a novel batch switching algorithm we propose called SB-QPS (Small Batch QPS), 
we describe SB-QPS first.  so it inherits the advantage of 
batching switching in achieving higher matching qualities, which translate into better throughput and delay performances:  
 it can achieve a high throughout of over 85\% under four standard traffic patterns.  
SB-QPS is a significant innovation that 
addresses all weaknesses of batch switching algorithms.   

First, using only a small batch size $T$ between 16 and 32,Second, the total time complexity of computing the batch of $T$ matchings is the lowest possible:  $O(NT)$ 
Second, it is a fully distributed algorithm so that the computational load can be efficiently divided evenly across $N$ input and output port ports.
The resulting time complexity is the lowest possible:  $O(1)$ per matching 
computation per port.  [say something about its communication complexity???]

 
%that can provably guarantee 100\% throughput 
%They all have a computational complexity 
%Second, all existing batch switching algorithms are centralized in the sense all $T$ matchings are computed by a single processor (say located at the switch controller).
%Hence, despite the aforementioned possible savings from the amortization, the average computational complexity per matching computation is still very high.  


First, $T$ has to be
quite or very large for all existing batch switching algorithms to achieve high throughout.   For example, it was reported in ... that ... has to be 3,000 for ...
Second, all existing batch switching algorithms are centralized in the sense all $T$ matchings are computed by a single processor (say located at the switch controller).
Hence, despite the aforementioned possible savings from the amortization, the average computational complexity per matching computation is still very high.  
For example, the algorithm proposed in~\cite{Neely2007FrameBased} that provably guarantees 100\% throughput and a low packet delay of $O(\log N)$ 
has a high time complexity of $O(N(\log N)(\log\log N))$ per matching computation, as we will elaborate in ???. 

%in~\cite{Neely2007FrameBased}, where $T$ is on the order of $O(\log N)$.  

%An alternative solution approach is the family of batch switching algorithms~\cite{}, 

In this work, we propose a novel switching algorithm, called SW-QPS (Small Window Queue Proportional Sampling), that has all the 
good virtues a switching algorithm can possibly possess.  Both its time and communication complexities are gimmick-free $O(1)$ 
(i.e., with small constant factors in the Big-O).  It can attain excellent throughput and delay performances.  
%all 
%advantages of both regular and batch switching algorithms.  

Since SW-QPS is based on a novel batch switching algorithm we propose called SB-QPS (Small Batch QPS), 
we describe SB-QPS first.  so it inherits the advantage of 
batching switching in achieving higher matching qualities, which translate into better throughput and delay performances:  
 it can achieve a high throughout of over 85\% under four standard traffic patterns.  
SB-QPS is a significant innovation that 
addresses all weaknesses of batch switching algorithms.   First, using only a small batch size $T$ between 16 and 32,Second, the total time complexity of computing the batch of $T$ matchings is the lowest possible:  $O(NT)$ 
Second, it is a fully distributed algorithm so that the computational load can be efficiently divided evenly across $N$ input and output port ports.
The resulting time complexity is the lowest possible:  $O(1)$ per matching 
computation per port.  [say something about its communication complexity???]



SW-QPS is a strict improvement over SB-QPS.  It inherits all advantages of ???.  It does not pay $O(T)$ delay penalty that dogs all 
batching algorithms.  Its throughput is even higher than SB-QPS.  

SW-QPS 
solves the switching problem under a new framework, 
called the {\it sliding-window (SW) switching}, that is first proposed in this work.  A sliding window algorithm is different than a batch algorithm only in the following aspect.  
In a batch switching algorithm, a batch of $T$ matchings are produced every $T$ cycles (say at the end of
$T^{th}$ cycle, $2T^{th}$ cycle, and so on).  In contrast, in a sliding-window switching algorithm, each window is still of size $T$ but 
a single matching is produced every cycle just like in a regular switching algorithm.   More precisely, at the beginning
of time slot $t$, the sliding window contains matchings-under-computation for the $T$ time slots $t$, $t+1$, $\cdots$, $t + T - 1$.   
The ``leading edge of the window", corresponding to the matching for the time slot $t$, ``graduates" and is used as the crossbar configuration for the current time slot $t$.   
Then at the end of time slot $t$, a new and currently empty matching is added to the ``tail end of the window" as the ``freshman class".  
This matching 
will be computed in the next $T$ cycles and hopefully becomes a high-quality matching by the time $t + T$, when it ``graduates".  
%This matching, which corresponds to the time slot $t + T$, 
%will be updated in the next $T$ cycles and hopefully populated into a high-quality matching by the time $t + T$, when it ``graduates" from the sliding window.  
\end{comment}


\begin{comment}
SW-QPS 
solves the switching problem under a new framework, 
called the {\it sliding-window (SW) switching}, that is first proposed in this work.  
The difference between a sliding window algorithm and a batch algorithm can be explained using a simple 
analogy.  A batch switching algorithm is like a bizarre school at which $T$ ``classes of students" (matchings) ``graduate" (get computed) at the same time every $T$ ``years" (time slots).
% (say at the end of
%$T^{th}$ cycle, $2T^{th}$ cycle, and so on), 
In contrast, a sliding-window switching algorithm is like a normal school at which there are also $T$ ``classes of students", but ``each year" it graduates a ``senior class" and welcomes 
a ``freshman class".  
%each window is still of size $T$ but 
%a single matching is produced every cycle just like in a regular switching algorithm.   
More precisely, at the beginning
of time slot $t$, the sliding window contains $T$ matchings-under-computation for the $T$ time slots $t$, $t+1$, $\cdots$, $t + T - 1$ respectively.   
The ``senior class", which entered the ``school" at ``year $(t - T)$" and has since gone through $T$ ``years of preparation", ``graduates" and is used for the crossbar configuration at time slot $t$.   
Then at the end of time slot $t$, a new and currently empty matching enters the school as the ``freshman class".  This matching 
will be ``trained" (computed) in the next $T$ cycles and hopefully becomes a high-quality matching by the time $t + T$, when it ``graduates".  
\end{comment}

\begin{comment}

In this framework, each batch is a sliding window that, at each time slot $t$, contains 

the sliding window contains 

 the matching computed for the earliest 
time slot in this batch is used as the current (i.e., for $t$) crossbar configuration.  

More precisely, at time slot %$

 All existing works are based on 
either the regular or the batching switching frameworks and fall victim to the following two extremes. On one hand, regular 
switching algorithms consider only a single time slot during the matching computation 
and produce one matching per time slot. Such a matching usually has a relatively low quality except in the cases where 
matchings are computed by an impractical high-computational-complexity regular switching algorithm, 
such as the Maximum Weighted Matching (MWM) algorithm. 
% \textcolor{green}{not really?? MWM has high quality}
On the other hand, batch switching algorithms consider multiple (say $T$) consecutive time slots ({\it i.e.,} a batch) during 
the matching computation, and produce $T$ matchings, all at once, per batch. 
As explained earlier, such matchings usually have higher qualities. 
However, these matchings are not produced in a ``timely'' manner. As a result, a packet arriving at the beginning of 
a batch has to wait till at least the beginning of the next batch to be switched. 
This causes additional delay that is often referred to as the 
{\it batching delay}. This batching delay can result in unnecessarily high packet
delay when the traffic is light or moderate. The SW switching framework falls between the above two extremes: SW switching algorithms consider multiple time slots during the matching computation and produce one matching 
per time slot. Therefore, they can produce high-quality matchings in a timely manner. 

The second algorithm, called SW-QPS, also builds upon QPS-r and is the first SW switching 
algorithm that fully exploits the advantages of the new SW switching framework. SW-QPS 
gets the better of both worlds: 
It can attain similar or even higher throughput than SB-QPS, yet it does not suffer from the batching delay. 



%Exacerbating this problem, the frame size $T$ is quite large and grows as at least $O(\log N)$ in almost all existing frame-based algorithms for reasons
%that we will explain in ...


%On the other hand, while many switching algorithms have lower complexities lower than $O(N)$, their throughput 
%performance is  (e.g., iSLIP has a time
%complexity of $O(\log^2 N)$ per port, 

%Take QPS-r~\cite{qpsr}, one state-of-the-art switching algorithm, as an example. 
%QPS-r, a parallel iterative algorithm, has the lowest possible per-port computational complexity of $O(1)$ and 
%has near-optimal delay performances under light and moderate traffic, but its throughput (even with $r$=3 iterations) is only around 
%80\% under the four standard traffic patterns (to be described in~\autoref{sec:eva}).   

% QPS-r \cite{Gong_QPSr_2019}, another recent example of a parallel iterative algorithm, generates each matching with $r$ iterations, each of which consists of two phases: proposing and accepting. In the proposing phase, each input port independently sends a proposal to at most one output port, and then in the accepting phase, each output port independently accepts the received proposals. When multiple proposals are sent to a single output port, at most one proposal can be accepted, and the only accepted proposal will never be changed or canceled. QPS-r has the lowest possible asymptotic complexity of $O(1)$ per port, but in return, it cannot generate matchings of enough quality to achieve 100\% throughput.

\subsection{Our Approaches}\label{subsec:ours}

In this work, 
% we aim at designing algorithms for switching in high-link-rate and high-radix input-queued switches, 
% that are low in computational complexities, yet have excellent throughput (equal or close to 100\%) and delay performances. 
we propose two switching algorithms for high-link-rate high-radix input-queued switches, 
that are low in computational complexities, yet have excellent throughput and delay performances, 
under two different switching frameworks. 

\smallskip
\noindent
{\bf Small-Batch QPS (SB-QPS).} The first algorithm, called SB-QPS, builds upon and significantly improves the throughput performance 
of QPS-r. The design of SB-QPS is based on the following insight: 
QPS-r and most other algorithms under the regular (slot-by-slot) switching framework that allows the matching 
computation considering only a single time slot, can be converted into algorithms under the 
batch switching framework that allows the matching computation considering multiple time slots. 
This gives SB-QPS an additional degree of freedom in the matching computation that
can result in better matchings and thus higher switch throughput and/or lower queueing delays.   
For example, an attempted connection between a ``busy'' input-output pair, more precisely, 
either the input port or the output port 
has already been paired with ``someone else'' (during the current time slot),  
during the matching computation, will fail in 
a regular switching algorithm, now may succeed (using a different time slot) in SB-QPS. 
We note that SB-QPS is a simple, but very subtle, batch switching adaptation for QPS-r. 
Hence, the per-port computational complexity of SB-QPS is also $O(1)$ per time slot.  
Yet, SB-QPS improves the throughput performance of QPS-3 ({\it i.e.,} QPS-r with $r$=3 iteration) by 
an additive term of between 0.03 to 0.12 under the four standard traffic patterns, as we will show in~\autoref{sec:eva}. 
We also note that QPS-r can attain 
the similar throughput performance (as SB-QPS) when running for approximately $r$=9 iterations, which, however, results in 
a computational complexity that is too high for a matching to be
computed in a short time slot in a high-radix switch. 

\smallskip
\noindent
{\bf Sliding-Window QPS (SW-QPS).} The second algorithm solves the switching problem under a new framework, 
called the {\it sliding-window (SW) switching}, that is first proposed in this work. This new switching framework will be 
detailed in~\autoref{sec:sws}. All existing works are based on 
either the regular or the batching switching frameworks and fall victim to the following two extremes. On one hand, regular 
switching algorithms consider only a single time slot during the matching computation 
and produce one matching per time slot. Such a matching usually has a relatively low quality except in the cases where 
matchings are computed by an impractical high-computational-complexity regular switching algorithm, 
such as the Maximum Weighted Matching (MWM) algorithm. 
% \textcolor{green}{not really?? MWM has high quality}
On the other hand, batch switching algorithms consider multiple (say $T$) consecutive time slots ({\it i.e.,} a batch) during 
the matching computation, and produce $T$ matchings, all at once, per batch. 
As explained earlier, such matchings usually have higher qualities. 
However, these matchings are not produced in a ``timely'' manner. As a result, a packet arriving at the beginning of 
a batch has to wait till at least the beginning of the next batch to be switched. 
This causes additional delay that is often referred to as the 
{\it batching delay}. This batching delay can result in unnecessarily high packet
delay when the traffic is light or moderate. The SW switching framework falls between the above two extremes: SW switching algorithms consider multiple time slots during the matching computation and produce one matching 
per time slot. Therefore, they can produce high-quality matchings in a timely manner. 

The second algorithm, called SW-QPS, also builds upon QPS-r and is the first SW switching 
algorithm that fully exploits the advantages of the new SW switching framework. SW-QPS 
gets the better of both worlds: 
It can attain similar or even higher throughput than SB-QPS, yet it does not suffer from the batching delay. 
\end{comment}

\begin{comment}
\begin{figure}[h]
	\centering
	\includegraphics[width=0.455\textwidth]{figures/IQ-sched-graph/scheduling-graph-standalone}
	\caption{A sample joint calendar of port number $N=8$ and batch size $T$: Cells with ``--" are unmatched.}\label{fig:sched-graph}
\end{figure}

In contrast to ``regular" (slot-by-slot) switching algorithms, which include MWM, iSLIP, QPS-r, and many other studies \cite{Anderson1993PIM, McKeown99iSLIP, GiacconePrabhakarShah2003SERENA, AtallaCudaGiacconeEtAl2013BPAssist, Hu2018HRF}, that produce each matching individually in each time slot, an alternative approach called batch switching \cite{bianco2002frame, rojas2007frame, Aggarwal2003EdgeColoring, Neely2007FrameBased, Wang2018ParallelEdgeColoring, Bianco2004BatchSched} groups multiple (say $T$) consecutive time slots as a batch and compute these matchings collectively. As is illustrated in \autoref{fig:sched-graph}, such a batch of matchings, usually called a {\it joint calendar}, is a $T \times N$ table with $TN$ cells. Each row of the joint calendar, which is a matching for the corresponding time slot, can be packed with packets not only in the corresponding time slot as in regular switching, but in any of the $T$ time slots within the current batch. Therefore, these matchings often have higher quality than those generated by regular switching algorithms. As a result, batch switching algorithms can achieve higher throughput than regular algorithms on the same complexity level under various traffic patterns ~\cite{bianco2002frame, rojas2007frame}.

However, compared with regular switching algorithms, batch switching algorithms suffer from an additional batching delay of $O(T)$: A packet arriving at the beginning of a batch has to wait till at least the beginning of the next batch to be switched. This $O(T)$ delay is a pronounced issue especially in the following two cases. Firstly, it is unnecessary when the traffic load is low, because in this case even regular switching algorithms can easily achieve packet delay as low as $O(1)$. Secondly, it is unacceptably high in many existing switching algorithms that use a large batch size $T$ to attain high throughputs ({\it e.g.} in ~\cite{Aggarwal2003EdgeColoring}, batch size $T$ is as large as $\omega(N^2)$ ).

\subsection{Our Work}\label{subsec:our-work}
To address the aforementioned challenges on packet switching, we combine parallel iterative algorithms and the batch switching approach for the advantages of both frameworks: low per-port complexity and high matching quality. To achieve this combination, we adopt a \textcolor{green}{novel} accepting strategy, which will be described in \autoref{subsec:sb-qps}. Furthermore, because of the greediness of our accepting strategy, our approach is applicable to a new framework called Sliding Window (SW) switching, which breaks the boundary of batches and solves the batching delay issue of batch switching algorithms.

The result of our study is the following two algorithms: Small-Batch QPS (SB-QPS) and Sliding-Window QPS (SW-QPS), corresponding to the batch switching and SW switching frameworks. The term QPS (short for Queue-Proportional Sampling) refers to an add-on matching technique that originally is proposed in~\cite{Gong2017QPS} and later extended to a standalone parallel iterative matching algorithm called QPS-r~\cite{Gong_QPSr_2019}, whose proposing phase (to be described in in~\autoref{subsec:qps}) is used in both of our algorithms, because it has low complexity and delivers high throughput. In fact, besides QPS, both of our algorithms are compatible with any parallel iterative switching algorithm with greedy packing schemes.

Our first algorithm, SB-QPS, has two advantages over previous works. Firstly, it is fully distributed with low per-port complexity. Most of the existing batch switching algorithms \cite{Aggarwal2003EdgeColoring, Neely2007FrameBased, Wang2018ParallelEdgeColoring} model the process to pack the joint calendar as an edge-coloring problem, but until now, all practical solutions to the latter problem are centralized and have high complexity. For example, the computation complexity of the Birkhoff von Neumann Decomposition (BvND)-based algorithm in \cite{Neely2007FrameBased} is $O(N^{1.5}T)$ per time slot. In contrast, SB-QPS packs the joint calendar by running two fully distributed phases that resemble those in QPS-r, keeping its computation complexity as low as $O(1)$ per port per time slot. 

The advantage feature of SB-QPS is that it reduces batching delay without sacrificing too much throughput. As we have mentioned above, batching delay is proportional to batch size, but larger batch sizes, associated with more chances to refine the joint calendar, are essential for the high throughput performances of previous batching algorithms. Because of the high efficiency of the QPS proposing scheme and our greedy accepting scheme, SB-QPS only requires $16$ refinements to achieve at least $87\%$ throughput under all four traffic patterns, so it can use a small batch size $T$ that is independent to $N$. Therefore, it has significantly low batching delay compared with the algorithm in \cite{Aggarwal2003EdgeColoring}, whose batch size is $\omega(N^2)$.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.295\textwidth]{figures//IQ-sched-graph/sliding-schedule}
	\caption{An illustration of the joint calendar of Sliding Window switching: The label of each row (matching) is its time slot of completion.}\label{fig:batch-vs-sw}
\end{figure}

Our second algorithm, SW-QPS, is based on a new switching framework called \emph{Sliding Window (SW) switching}, which overcoms the batching delay issue of batch switching algorithms. In the sliding window framework, at arbitrary time slot $t$, the scheduler also refines a joint calendar of $T$ matchings as in batch switching, shown as the bold frame in \autoref{fig:batch-vs-sw}. However, unlike batch switching, these $T$ matchings are not finalized all together at the end of this batch but at different time slots ranging from $t$ to $t+T-1$, one matching per time slot. 

As an intuitive analogy, we view the joint calendar as a ``school" of students. In batch switching, this school enrolls all students at the same time, packs them with packets, and bids farewell to them all before enrolling the next batch of students. In SW switching, pretty similar to a real-life school, only one class of students, which correspond to one matching in the joint calendar, are enrolled and only one class of students graduate at each time slot. We label the classes by their time slots of graduation. At an arbitrary time slot $t$, the school contains $T$ classes from Class $t$ to Class $t+T-1$, shown as the bold frame in \autoref{fig:batch-vs-sw}. From the perspective of students, Class $t$ is enrolled at time slot $t-T+1$, when the joint calendar covers Class $t-T+1$ to Class $t$ (the first three rows in \autoref{fig:batch-vs-sw}), and has $T$ time slots to be packed with packets before graduating at time slot $t$. After the graduation of Class $t$, the joint calendar moves one time slot downwards to cover Class $t+1$ to Class $t+T$ (the last four rows in \autoref{fig:batch-vs-sw}). 

As a SW switching algorithm, SW-QPS gets the better of both worlds:  high matching quality comparable to batch switching and low packet delay comparable to regular switching. Compared with SB-QPS, SW-QPS achieves similar matching qualities, because each matching also stays in the joint calendar for $T$ time slots and has similar chances to be packed as in SB-QPS. As is shown in \autoref{sec:eva}, SW-QPS achieves 87\% throughput under diagonal traffic and over 90\% throughput under other three traffic patterns.  Moreover, SW-QPS has significantly lower batching delay than SB-QPS, because it is allowed to pack packets directly to seniors students who will graduate soon in the joint calendar without having to wait for the next batch to begin. As in \autoref{sec:eva}, SW-QPS has excellent delay performance that is close to that of MWM when the traffic load is under $0.8$. 

\end{comment}

The rest of this paper is organized as follows. In \autoref{sec:sys-module}, we state assumptions and the problem model used in this work. 
\autoref{sec:sb-qps} and \autoref{sec:sw-qps} detail the SB-QPS and SW-QPS algorithms respectively.  
% framework. %that is first proposed in this work.  
% In \autoref{sec:schemes}, 
% we first review QPS proposing strategy, and then we describe the two proposed schemes: SB-QPS and SW-QPS. 
In~\autoref{sec:related}, we survey the related works. 
Then, we evaluate the performances of SB-QPS and SW-QPS in~\autoref{sec:eva} and in \autoref{sec:con}, we conclude this paper. 

==> SW-QPS-PERF2020(arxiv)/sections/intro.BK.tex <==
\section{Introduction}\label{sec:intro}
\begin{comment}
	from qps-r
\end{comment}
The volume of network traffic across the Internet and in data-centers continues to grow relentlessly,
thanks to existing and emerging data-intensive applications, such as big data analytics, cloud computing,
and video streaming.  At the same time, the number of network-connected devices is exploding,
fueled by the wide adoption of
%mobile hand-held devices
smart phones and the emergence of the Internet of things.
To transport and ``direct" this massive amount of traffic to their respective destinations,
%At the same time, the number of Internet-connected devices continues to,
switches and routers capable of
connecting a large number of ports (called {\it high-radix}~\cite{Cakir2015HighRadix,Cakir2016HighRadixCrossbar}) and operating
at very high line rates are badly needed.

% Most present day switching systems in Internet routers and
% data-center switches employ an input-queued crossbar switch to interconnect the $N$ input ports with the $N$ output ports.
Many present day switching systems in Internet routers and
data-center switches employ an input-queued crossbar to interconnect their input ports and output ports
({\it e.g.,} Cisco Nexus 5000 Series~\cite{cisco_nexus_5000_2017}, Arista 7500 Switch~\cite{arista_7500_2018},
and Juniper QFX 10000 Switches~\cite{juniper_qfx10000_2018}).
%{Note in this work, we only consider the switching systems that employ a single-stage crossbar, or a monolithic crossbar, as the scheduler
%for such a crossbar can have full visibility of the entire system thus can make better scheduling decisions~\cite{cisco_nexus_5000_2017}.
Though it was commonly believed that such a (monolithic) crossbar is difficult to scale beyond 64 (input/output) ports, recent advances in switching hardware
technologies ({\it e.g.,}~\cite{Passas2010HighRadix,Passas2012bHighRadix,Cakir2015HighRadix})
have made high-radix crossbars not only
technologically feasible but also
economically and environmentally ({\it i.e.}, more energy-efficient) favorable, as compared to low-radix crossbars.



\begin{comment}
from serenade
\end{comment}
\subsection{Matching Problem}

% the $N$ input ports with the $N$ output ports.
In an $N\times N$ input-queued crossbar switch, each input port can be connected to only one output
port and vice versa in each switching cycle or time slot.
Hence, in every time slot, the switch needs to compute
a one-to-one \textit{matching} between input and output ports ({\it i.e.}, the crossbar schedule).
A major research challenge
of designing high-link-rate high-radix
switches ({\it e.g.}, 128 ports or beyond of 40 Gbps each)
is to develop algorithms that can
compute ``high quality'' matchings -- {\it i.e.} those that result in
high switch throughput and low queueing
delays for packets -- in a few nanoseconds.
% For example, with a fixed packet (cell) length of 64 bytes (used in the crossbar of Cisco 12000 Series Internet
% Routers~\cite{ciscoCellSize}), a switch supporting 40 Gbps per-port rates has to compute a matching
% every 12.8  nanoseconds.
For example, with a cell\footnote{It is common practice in switches/routers to slice incoming
	packets into cells of a fixed size or a range of variable sizes~\cite[Chapter 2, Page 21]{aweya_switch_router_2018}.
	For example, Juniper QFX 10000 switch~\cite{juniper_qfx10000_2018} uses cell sizes varying
	between 96 and 176 bytes, and Huawei NE40E switch~\cite{huawei_ne40e_2018} uses
	a fixed cell size.} size of 64 bytes (the minimum cell size used in Arista 7500 Switch~\cite{arista_7500_2018}),
a switch supporting 40 Gbps per-port rates has to compute a matching
every 12.8  nanoseconds.
%(with speedup of $1$)

\begin{comment}
Due to the physical limitations of crossbars, each input port in an
input-queued switch can only connect with a single output port during each
switching cycle, \ie time slot, and vice versa. Therefore, the input-queued
switch has to determine at each time slot the one-to-one connection, or
one-to-one matching between the input ports and output ports. This makes the
switch scheduling problem, in which we need to design algorithms to produce
``good-quality'' matchings resulting in good throughput and low delays. The
switch scheduling problem is the primary research challenge in designing
large high-speed single-crossbar switches.
\end{comment}

Unfortunately, there appears to be a tradeoff
between the quality of a matching and the amount of 
time needed to compute it (\ie time complexity). 
% \modifiedHL{
% \modifiedHL{
For example, %when used for crossbar scheduling, 
using Maximum Weighted Matchings (MWM) as crossbar schedules
%, with a suitable weight measure,
is known to result in 100\% switch throughput and
near-optimal
%Tassiulas90Max,
queueing delays for various traffic patterns~\cite{McKeownMekkittikulAnantharamEtAl1999}, but
%For a switch with $N$ input/output ports, however,
each MWM takes $O(N^{2.5}\log W)$ time to compute using the state-of-the-art algorithm~\cite{Duan2012BpMWMScaling}, where
$W$ is the maximum possible length of a VOQ. 


\begin{comment}
%% [MWM is great, but too expensive]
The switch scheduling problem can be transformed into a matching problem for an
$N\times N$ weighted bipartite graph. Maximum Weight Matching (MWM), with
well-chosen quantities as weight for edges, is known to produce great
matchings which can achieve $100\%$ throughput and empirically optimal
delays for various traffic patterns~\cite
{McKeownMekkittikulAnantharamEtAl1999,ShahWischik2006MWM0}.
However, it takes $O(N^3)$ time to compute a matching in MWM~\cite
{EdmondsKarp1972}. Parallelized variants exist, some of them still need $O
(N^2)$ work at each input/output port~\cite
{BayatiShahSharma2008MWMMaxProduct}, some achieves sublinear but either
assumes
a concurrent-read concurrent-write parallel random access machine,
which is too complex to implement in hardware, or
requires $O(N^3)$ processing elements~\cite{Fayyazi2004pMWM} which is too
expensive to be adopted in switches. This reality motivates a lot of
researchers to pursuit practical switch scheduling algorithms with much lower
time complexity, but still has performance close to MWM.
%



Another example is iSLIP~\cite{McKeown99iSLIP},
a distributed iterative algorithm where input and
output ports compute a matching in parallel through
multiple iterations of message exchanges.  iSLIP has
a per-port computational complexity of $O(\log^2 N)$ ($O(\log N)$
iterations that each has $O(\log N)$ circuit depth) that is lower than Serena's overall complexity of $O(N)$.
%by using $2N$ identical hardware modules running in parallel.
However, iSLIP computes a different type of matching called a Maximum-Size Matching (MSM), which is of
lower quality than MWM.  Hence iSLIP cannot achieve 100\% throughput
except on uniform traffic, and has much longer
queueing delays than Serena on nonuniform traffic
patterns under heavy traffic loads.

\end{comment}

While considerable research has been performed on crossbar scheduling algorithms 
for decades, these algorithms~\cite{Anderson1993PIM,McKeown1995iLQF,Tassiulas1998TASS,Mekkittikul98stability,McKeownMekkittikulAnantharamEtAl1999,McKeown99iSLIP,Goudreau00Shakeup,ShahGiacconePrabhakar2002SerenaMicro,Giaccone2002Apsara,GiacconePrabhakarShah2003SerenaJSAC,Aggarwal2003EdgeColoring,Keslassy2003MSM,ZhangBhuyan2003iDRR,Fayyazi04ParallelMWM,ShahWischik2006MWM0,BayatiPrabhakarShahEtAl2007Iterative,Neely2007FrameBased,Gupta09Node,Ye10Variable,AtallaCudaGiacconeEtAl2013BPAssist,Wang2018ParallelEdgeColoring,Hu2018HRF} are not suitable 
for future high-speed large input-queued switches, since what was 
considered high-speed ({\it e.g.,} $1$ Gbps per port) and large ({\it e.g.,} 
$64$ ports) is pale in comparison with the type of speed ({\it e.g.,} $1$ Tbps per 
port) and large ({\it e.g.,} $1,000$ ports) we are aiming for today~\cite{DeCusatis2014FutureSwitch,Kim2005RouterDevTrand}, yet 
our expectation of delay and throughput performance are only going to become 
higher. \textcolor{green}{future is what we are aiming for today. Our expectation future is far beyond imagination.} For example, the two well-known among these algorithms are SERENA~\cite{ShahGiacconePrabhakar2002SerenaMicro,GiacconePrabhakarShah2003SerenaJSAC} and 
iSLIP~\cite{McKeown99iSLIP}, but neither is suitable for 
high-speed input-queued switches with $\textcolor{green}{a}$ large number of ports. On one hand, although SERENA 
can achieve 100\% throughput and has excellent delay performance close to 
that of MWM, its computational 
complexity for generating a matching is $O(N)$, which is too high for high-speed 
switches when $N$ is large. On the other hand, 
iSLIP only requires $O(\log N)$ 
iterations to compute a matching, but it can only guarantee to achieve at least 
$50\%$ throughput~\cite{Dai00Speedup} and it suffers from poor delay performance under heavy nonuniform 
traffic~\cite{GiacconePrabhakarShah2003SerenaJSAC}.

%% [SERENA is a very good approximation with O(N) complexity, without
% explaining the details of the algorithm, say
% that O(N) is still too expensive for large N so SERENA is not widely
% adopted]
\deletedHL{
Researchers have been searching for crossbar scheduling algorithms that have time complexity much lower
than $O(N^3)$, but performance
close to MWM. 
Some researchers have developed parallel or distributed MWM algorithms\cite{Fayyazi04ParallelMWM,Fayyazi2006ParaMWM,BayatiPrabhakarShahEtAl2007Iterative,BayatiShahSharma2008MWMMaxProduct} that, by 
distributing the computational cost across multiple processors (nodes), bring down 
the per-node computational complexity. However, these algorithms either require too many 
processors ~\cite{Fayyazi04ParallelMWM,Fayyazi2006ParaMWM} or have very high per-node computational complexity 
~\cite{BayatiPrabhakarShahEtAl2007Iterative,BayatiShahSharma2008MWMMaxProduct}, which are impractical to implement in today's IQ switches. 

Some researchers have proposed algorithms based on maximum 
cardinality matching or maximal matching, 
such as PIM~\cite{Anderson1993PIM} and iSLIP~\cite{McKeown99iSLIP}. 
Those types of matchings can be computed with lower computational complexity, they 
however have lower qualities than MWM: They can not achieve 100\% switch throughput and 
usually have much higher delays than MWM under non-uniform traffic. 

Some researchers have proposed  
low-complexity randomized algorithms~\cite{Tassiulas1998TASS,ShahGiacconePrabhakar2002SerenaMicro,GiacconePrabhakarShah2003SerenaJSAC,Ye10Variable}. 
Tassiulas~\cite{Tassiulas1998TASS} proposed the so-called ``pick-and-compare'' algorithm, which can achieve $100\%$ switch 
throughput with linear complexity but has very bad delay performance. Inspired by 
Tassiulas' work, 
% researchers have developed a few low-complexity algorithms which 
% can achieve $100\%$ switch throughput and have good delay performance. 
% So far, the best 
% known among them is 
Giaccone, Prabhakar, and Shah proposed 
SERENA~\cite{ShahGiacconePrabhakar2002SerenaMicro,GiacconePrabhakarShah2003SerenaJSAC}.
SERENA produces excellent matching decisions that result in $100\%$ switch throughput
and queueing delay close to that of MWM.
However, it is a centralized algorithm with $O(N)$ time complexity.  When $N$ is large,
this complexity is too high to support very high link rates.  Hence, as stated 
in~\cite{ShahGiacconePrabhakar2002SerenaMicro,GiacconePrabhakarShah2003SerenaJSAC},
SERENA is designed for high-aggregate-rate switches -- \ie those that have either a large number of ports 
%(but with relatively low line rates per port) 
or a
very high line rate per port -- but not for those that have both. } % end addedHL
%(but with a small number of ports)
%;  it is not suitable for switches that have both.
%However, its $O(N)$ time complexity is still too high for
%large $N$, which limits its wide adoptions in large input-queued switches.
\deletedHL{
While parallelizing the SERENA algorithm seems to be an obvious solution to this scalability problem,
we will show in \autoref{subsec: merge} that a key procedure in SERENA, namely MERGE,
is monolithic in nature, making SERENA hard to parallelize.}

\deletedHL{
Besides the above algorithms which make a matching decision per each time slot, some 
researchers have proposed another type of crossbar scheduling -- frame-based 
scheduling~\cite{Aggarwal2003EdgeColoring,Neely2007FrameBased,Wang2018ParallelEdgeColoring}. In frame-based scheduling, consecutive time slots are grouped 
into frames and the matching decisions are made on a per-frame basis. Since a frame 
typically spans many time slots ({\it e.g.,} $O(\log N)$), and a packet arriving at 
the beginning of a frame has to wait till the end of the frame, frame-based 
scheduling typically results in higher queueing delays.      
}
% \glong{To the best of our knowledge, no parallelization of SERENA, has been
% proposed in the literature.}
%
%parallelized variants which
%achieves sublinear work at each input/output port do not exist.
%
%rounds of
%
\subsection{Our Work}
\textbf{Our contributions}

The rest of this paper is organized as follows. In \autoref{sec:background}, we provide some
background on the input-queued crossbar switches.  In \autoref{sec:scheme},  we first review
QPS, and then describe QPS-r. Then in~\autoref{sec:throughput-and-delay-analysis}, we derive the throughput and
the queue length (and delay) bounds of QPS-r, followed by the
performance evaluation in~\autoref{sec:evaluation}. In~\autoref{sec: related-work}, we survey
related work before concluding this paper in~\autoref{sec:conclusion}.

==> SW-QPS-PERF2020(arxiv)/sections/intro.tex <==
\section{Introduction}\label{sec:intro}
% % [Long: faster traffic, large network]
The volume of network traffic across the Internet and in data-centers continues to grow relentlessly,
thanks to existing and emerging data-intensive applications, such as big data analytics, cloud computing,
and video streaming.  At the same time, the number of network-connected devices is exploding,
fueled by the wide adoption of 
%mobile hand-held devices
smart phones and the emergence of the Internet of things.
To transport and ``direct" this massive amount of traffic to their respective destinations,
%At the same time, the number of Internet-connected devices continues to,
switches and routers capable of 
connecting a large number of ports (called {\it high-radix}~\cite{Cakir2015HighRadix,Cakir2016HighRadixCrossbar}) and operating
at very high line rates are badly needed. Motivated by this rapidly growing need, much research has been devoted to, and significant breakthroughs
made, on the hardware designs for fast high-radix switching fabrics recently ({\it e.g.},~\cite{Cakir2016HighRadixCrossbar,Dai2017HighRadix}). Indeed,
these recent breakthroughs have made fast high-radix switching hardware not only technologically feasible
but also economically and environmentally (more energy-efficient) favorable, as compared to low-radix
switching hardware~\cite{Cakir2016HighRadixCrossbar}. 

% \subsection{Matching Problem}\label{subsec:mp}
\subsection{Matching Problem and Prior Work}\label{subsec:mp}
% % [Long: difficult]
% Most present day switching systems in Internet routers and
% data-center switches employ an input-queued crossbar switch to interconnect the $N$ input ports with the $N$ output ports. 
Many present day switching systems in Internet routers and
data-center switches employ an input-queued crossbar to interconnect their input ports and output ports. 
\begin{comment}
({\it e.g.,} Cisco Nexus 5000 Series~\cite{cisco_nexus_5000_2017}, Arista 7500 Switch~\cite{arista_7500_2018},
and Juniper QFX 10000 Switches~\cite{juniper_qfx10000_2018}).
%{Note in this work, we only consider the switching systems that employ a single-stage crossbar, or a monolithic crossbar, as the scheduler
%for such a crossbar can have full visibility of the entire system thus can make better scheduling decisions~\cite{cisco_nexus_5000_2017}.
Though it was commonly believed that such a (monolithic) crossbar is difficult to scale beyond 64 (input/output) ports, recent advances in switching hardware
technologies ({\it e.g.,}~\cite{Passas2010HighRadix,Passas2012bHighRadix,Cakir2015HighRadix})
have made high-radix crossbars not only
technologically feasible but also
economically and environmentally ({\it i.e.}, more energy-efficient) favorable, as compared to low-radix crossbars. 
\end{comment}
In an $N\times N$ input-queued crossbar switch, each input port can be connected to only one output
port and vice versa in each switching cycle or time slot.
Hence, in every time slot, the switch needs to compute
a one-to-one \textit{matching} between input and output ports ({\it i.e.}, the crossbar schedule).
A major research challenge
of designing high-link-rate high-radix
switches ({\it e.g.}, 128 ports or beyond of 40 Gbps each)
is to develop (switching) algorithms that can
compute ``high quality'' matchings -- {\it i.e.} those that result in
high switch throughput and low queueing
delays for packets -- in a few nanoseconds.
% For example, with a fixed packet (cell) length of 64 bytes (used in the crossbar of Cisco 12000 Series Internet
% Routers~\cite{ciscoCellSize}), a switch supporting 40 Gbps per-port rates has to compute a matching
% every 12.8  nanoseconds.
\begin{comment}
For example, with a cell\footnote{It is common practice in switches/routers to slice incoming
	packets into cells of a fixed size or a range of variable sizes~\cite[Chapter 2, Page 21]{aweya_switch_router_2018}.
	For example, Juniper QFX 10000 switch~\cite{juniper_qfx10000_2018} uses cell sizes varying
	between 96 and 176 bytes, and Huawei NE40E switch~\cite{huawei_ne40e_2018} uses
	a fixed cell size.} size of 64 bytes (the minimum cell size used in Arista 7500 Switch~\cite{arista_7500_2018}),
a switch supporting 40 Gbps per-port rates has to compute a matching
every 12.8  nanoseconds.
%(with speedup of $1$)
\end{comment}
\begin{comment}
Due to the physical limitations of crossbars, each input port in an
input-queued switch can only connect with a single output port during each
switching cycle, \ie time slot, and vice versa. Therefore, the input-queued
switch has to determine at each time slot the one-to-one connection, or
one-to-one matching between the input ports and output ports. This makes the
switch scheduling problem, in which we need to design algorithms to produce
``good-quality'' matchings resulting in good throughput and low delays. The
switch scheduling problem is the primary research challenge in designing
large high-speed single-crossbar switches.
\end{comment}

\begin{comment}
Unfortunately, there appears to be a tradeoff
between the quality of a matching and the amount of 
time needed to compute it (\ie time complexity). 
% \modifiedHL{
% \modifiedHL{
For example, %when used for crossbar scheduling, 
using Maximum Weighted Matchings (MWM) as crossbar schedules
%, with a suitable weight measure,
is known to result in 100\% switch throughput and
near-optimal
%Tassiulas90Max,
queueing delays for various traffic patterns~\cite{McKeownMekkittikulAnantharamEtAl1999}, but
%For a switch with $N$ input/output ports, however,
each MWM takes $O(N^{2.5}\log W)$ time to compute using the state-of-the-art algorithm~\cite{Duan2012BpMWMScaling}, where
$W$ is the maximum possible length of a VOQ. 
\end{comment}

\begin{comment}
%% [MWM is great, but too expensive]
The switch scheduling problem can be transformed into a matching problem for an
$N\times N$ weighted bipartite graph. Maximum Weight Matching (MWM), with
well-chosen quantities as weight for edges, is known to produce great
matchings which can achieve $100\%$ throughput and empirically optimal
delays for various traffic patterns~\cite
{McKeownMekkittikulAnantharamEtAl1999,ShahWischik2006MWM0}.
However, it takes $O(N^3)$ time to compute a matching in MWM~\cite
{EdmondsKarp1972}. Parallelized variants exist, some of them still need $O
(N^2)$ work at each input/output port~\cite
{BayatiShahSharma2008MWMMaxProduct}, some achieves sublinear but either
assumes
a concurrent-read concurrent-write parallel random access machine,
which is too complex to implement in hardware, or
requires $O(N^3)$ processing elements~\cite{Fayyazi2004pMWM} which is too
expensive to be adopted in switches. This reality motivates a lot of
researchers to pursuit practical switch scheduling algorithms with much lower
time complexity, but still has performance close to MWM.
%



Another example is iSLIP~\cite{McKeown99iSLIP},
a distributed iterative algorithm where input and
output ports compute a matching in parallel through
multiple iterations of message exchanges.  iSLIP has
a per-port computational complexity of $O(\log^2 N)$ ($O(\log N)$
iterations that each has $O(\log N)$ circuit depth) that is lower than Serena's overall complexity of $O(N)$.
%by using $2N$ identical hardware modules running in parallel.
However, iSLIP computes a different type of matching called a Maximum-Size Matching (MSM), which is of
lower quality than MWM.  Hence iSLIP cannot achieve 100\% throughput
except on uniform traffic, and has much longer
queueing delays than Serena on nonuniform traffic
patterns under heavy traffic loads.

\end{comment}
Unfortunately, there appears to be a tradeoff
between the quality of a matching and the amount of 
time needed to compute it (\ie time complexity). 
For example, %when used for crossbar scheduling, 
using Maximum Weighted Matchings (MWM) as crossbar schedules
%, with a suitable weight measure,
is known to result in 100\% switch throughput and
near-optimal 
queueing delays for various traffic patterns~\cite{McKeownMekkittikulAnantharamEtAl1999}, but
%For a switch with $N$ input/output ports, however,
each MWM takes $O(N^{2.5}\log W)$ time to compute using the state-of-the-art algorithm~\cite{Duan2012BpMWMScaling}, where
$W$ is the maximum possible length of a VOQ.  
While considerable research has been performed on switching algorithms 
% ~\cite{Anderson1993PIM,McKeown1995iLQF,Tassiulas1998TASS,Mekkittikul98stability,McKeownMekkittikulAnantharamEtAl1999,McKeown99iSLIP,Goudreau00Shakeup,ShahGiacconePrabhakar2002SerenaMicro,Giaccone2002Apsara,GiacconePrabhakarShah2003SERENA,Aggarwal2003EdgeColoring,Keslassy2003MSM,ZhangBhuyan2003iDRR,Fayyazi04ParallelMWM,ShahWischik2006MWM0,BayatiPrabhakarShahEtAl2007Iterative,Neely2007FrameBased,Gupta09Node,Ye10Variable,AtallaCudaGiacconeEtAl2013BPAssist,Wang2018ParallelEdgeColoring,Hu2018HRF} 
% % references are too many, only select some of them
for decades, these algorithms~\cite{Anderson1993PIM,McKeown99iSLIP,GiacconePrabhakarShah2003SERENA,AtallaCudaGiacconeEtAl2013BPAssist,Hu2018HRF} are not suitable 
for future high-speed large input-queued switches, since what was 
considered high-speed ({\it e.g.,} $1$ Gbps per port) and large ({\it e.g.,} 
$64$ ports) is pale in comparison with the type of speed ({\it e.g.,} $1$ Tbps per 
port) and large ({\it e.g.,} $1,000$ ports) we are aiming for today~\cite{DeCusatis2014FutureSwitch,Kim2005RouterDevTrand}, yet 
our expectation of delay and throughput performance are only going to become 
higher. 
% % Jingfan's comments
\lbrack\textcolor{green}{JM: can we simplify this sentence a little?}\rbrack  
For example, the two well-known among these algorithms are SERENA~\cite{GiacconePrabhakarShah2003SERENA} and 
iSLIP~\cite{McKeown99iSLIP} \textcolor{green}{[seems strange]}, but neither is suitable for 
% % Long: changed a large number of ports to "high-radix" as we have already defined it 
% %  with a large number of ports --> high-radix 
high-radix high-speed input-queued switches. On one hand, although SERENA 
can achieve 100\% throughput and 
% has excellent delay performance close to that of MWM, 
has reasonably good delay performance, 
% its computational 
% complexity for generating a matching is $O(N)$, which is too high for high-speed 
% switches when $N$ is large. 
it is a centralized algorithm with $O(N)$ computational 
complexity for generating a matching, which is too high for high-speed 
switches when $N$ is large. On the other hand, 
iSLIP is a parallel (more precisely distributed iterative) algorithm and has 
a lower per-port computational complexity of $O(\log^2 N)$ using $N$ processors (one at each port), 
but iSLIP cannot attain 100\% throughput 
except under uniform traffic. 
% iSLIP, a well-known parallel iterative algorithm, only requires $O(\log N)$ 
% iterations to compute a matching, but it can only guarantee to achieve at least 
% $50\%$ throughput~\cite{Dai00Speedup} and it suffers from poor delay performance under heavy nonuniform 
% traffic~\cite{GiacconePrabhakarShah2003SERENA}. 
% % Long: added communication complexity
Besides, iSLIP with a distributed implementation \textcolor{green}{[since the $O(\log^2 N)$ complexity is distributed, shall we move ``distributed" to the sentence above?]}has a high communication complexity of $O(N)$ per 
port, which makes it difficult to scale to switches with a large number of ports.  


% \subsection{SW-QPS}\label{subsec:sw-qps}

% % [Long: Alternative approach]
% In this work, we adopt an alternative approach -- batch 
% switching~\cite{Aggarwal2003EdgeColoring,Neely2007FrameBased,Wang2018ParallelEdgeColoring}. 
Besides the aforementioned regular switching algorithms ({\it e.g.,} iSLIP and SERENA), 
an alternative type of switching algorithms is batch-based. 
Unlike in a regular switching algorithm, where a matching decision is computed for every time slot, 
in a batch switching algorithm ({\it e.g.,} \cite{bianco2002frame,rojas2007frame,Aggarwal2003EdgeColoring,Neely2007FrameBased,Wang2018ParallelEdgeColoring,Bianco2004BatchSched}), multiple (say $T$) consecutive time slots are grouped 
as a batch and the $T$ matching decisions are batch-computed.  
Since the batch-computation of these $T$ matchings 
often has lower time complexity than 
$T$ independent matching computations, the amortized 
(over the $T$ time slots) time complexity of a batch switching
algorithm is often lower than that of a regular switching algorithm. 
Batch switching algorithms are also shown to have better throughput 
performance (than their regular switching counterparts) for various traffic patterns~\cite{bianco2002frame,rojas2007frame} %especially for non-uniform traffic 
when the batch size $T$ is well-chosen. 
% % may need to move
{\bf Long: Here, the logic flow is not good enough! Let's figure out a better one} 
It is %however \textcolor{green}{[however? why big batch is desirable?]} 
desirable for this batch size $T$ to be small because batch switching  
algorithm has a batching delay of $O(T)$: 
A packet arriving at the beginning of a batch has to wait till 
at least the beginning of the next batch to be switched. 
% 
% However, most of the existing batch switching algorithms 
% are centralized and cannot be effectively parallelized to reduce their computational complexities per port. 
However, to attain high throughputs, all existing batch switching algorithms have to either 
use a large batch size ({\it e.g.,} $O(N^2)$ 
in~\cite{Aggarwal2003EdgeColoring}) which leads to high batching delay, or still 
% ,Li2008BatchSched,Bianco2002BatchSched,Bianco2004BatchSched
incur a high computational complexity~\cite{Neely2007FrameBased,Bianco2004BatchSched}) even after the amortization.
{\bf Move (the following sentence) to related work section} 
Although a parallel batch switching algorithm recently 
proposed in~\cite{Wang2018ParallelEdgeColoring} 
has a computational complexity of $O(\log N)$ per time slot per port, it requires a large $T$: A batch size of $\num{3096}$ 
was needed for $N \!=\! 300$ as reported in~\cite{Wang2018ParallelEdgeColoring}.

Therefore, it remains a challenging problem for designing efficient switching algorithms that 
have low computational complexities, yet have excellent throughput and delay performances. 

\subsection{Our Work}\label{subsec:our-work}

% In this work, we aim at designing efficient parallel batch switching 
% algorithms that requires a small batch size and has low computational complexities per port, 
% yet they can attain very high throughputs and have excellent delay performances. 
In this work, we first propose Small-Batch QPS (SB-QPS), a batch 
switching algorithm that uses a small constant batch size
$T$ that is independent of $N$. 
Here QPS stands for Queue-Proportional Sampling, an add-on technique
proposed in~\cite{Gong2017QPS} that we will describe in~\autoref{subsec:qps}.  
Although QPS can also work as a stand-alone algorithm, we found that \textcolor{green}{no we found that} its throughput is only around 
$63\%$ under uniform traffic when running for a single iteration, and this throughput grows 
very slowly with the number of iterations. Benefiting from the advantages of batching, SB-QPS has much better throughput performance. \textbf{The throughput performance of SB-QPS is much better, benefiting from batching.}

However, SB-QPS has worse delay performances when the traffic is light because it suffers 
from the batching delay issue, the inherent disadvantage of all batching algorithms. 
\textbf{However, as with all batching algorithms, SB-QPS suffers from an inherent batching delay, which is negligible under heavy traffic loads, but is significant under light traffic loads.}
% % [TODO: emphasize BS usually has higher throughput]
% % [batching delay is a disadvantage when traffic load is light]
This batching delay is negligible when the traffic load is heavy, however, it dominates 
the packet delay when the traffic load is light. To overcome this disadvantage, 
we propose a new ``batch switching approach'' 
called Sliding-Window (SW) switching. Unlike 
in a batch switching algorithm, where $T$ matchings are produced at once \textcolor{green}{all together} per batch, in a 
SW switching algorithm, $T$ matchings for $T$ consecutive time slots 
(say time slot $t$ to $t\!+\!T\!-\!1$) are maintained and refined at each time slot and the 
matching for the earliest time slot ({\it i.e.,} time slot $t$) is finalized and 
used to switch packets for time slot $t$. \textbf{and at each time slot, one of these matchings becomes ready for switching.}
 Therefore, it gets the better of both worlds:  
Its delay performance is comparable to that of regular switching 
algorithms under light traffic (or in other words, it does not suffer from 
the batching delay issue) and similar to that of batch 
switching algorithms under moderate and heavy traffic, 
yet its throughput performance is similar to  
that of batch switching algorithm. \textbf{It achieves the high throughput performance and low amortized complexity that are comparable to batch switching algorithms, without paying the batching delay.}

Building upon SW switching, %and the recent switching work Queue-Proportional Sampling (QPS)~\cite{Gong2017QPS}, 
we then propose SW-QPS, a sliding-window \textcolor{green}{SW} switching algorithm that has 
a per-port computational complexity of $O(1)$ \textcolor{green}{$O(1)$ computational complexity per port}. %and a per-port communication complexity of $O(T)$. 
% Since in SW-QPS, $T$ is a small constant independent of $N$, SW-QPS has the lowest possible 
% (asymptotic) computational and communication complexity: $O(1)$ per port. 
Yet, SW-QPS has excellent 
throughput and delay performances. As we will \textcolor{green}{no will} show in~\autoref{sec:eva}, SW-QPS achieves at least $90\%$ 
throughput (except for the diagonal traffic, under which the throughput is slightly lower than $90\%$) and delay performance close to that of MWM when the 
traffic load is not extremely high (say $<0.8?$) under all $4$ standard traffic patterns (to be described in~\autoref{sec:eva}). In comparison, iSLIP~\cite{McKeown99iSLIP}, a well-known parallel iterative regular switching algorithm, can only attain roughly $80\%$ throughput under the $4$ standard traffic patterns except 
the uniform traffic and as mentioned earlier, it has a computational complexity of $O(\log^2 N)$ per port 
and a communication complexity of $O(N)$ per port. 

% \textbf{Our contributions}

The rest of this paper is organized as follows. In \autoref{sec:backg}, we provide some
background on the input-queued crossbar switches, batch switching and sliding-window \textcolor{green}{SW} switching.  
In \autoref{sec:schemes},  we first review
QPS, and then we describe our schemes: SB-QPS and SW-QPS. 
Then we evaluate the performance of our schemes in~\autoref{sec:eva}. 
In~\autoref{sec:related}, we survey
related work before concluding this paper in~\autoref{sec:con}.

==> SW-QPS-PERF2020(arxiv)/sections/marks.tex <==
\newpage
\textcolor{green}{\section{Marks}}
\begin{enumerate}
	\item: To change the tables and figures from QPS-3 to QPS-1, use comp\_qps1 and burst60\_qps1.
	use burst80\_wo for high load bursty without QPS-r.
\end{enumerate}


==> SW-QPS-PERF2020(arxiv)/sections/related_work.tex <==
\section{Related Work}\label{sec:related}

% Scheduling in crossbar switches
% Switching is a well-studied problem with a large amount of literature, so 
In this section, we provide a brief survey of prior studies that are directly related to ours. %We start with regular switching algorithms and then move to batch switching. 
%Since, in~\cite{Gong2017QPS}, L. Gong {\it et al.} have provided a
%thorough survey of existing work related to QPS from the
%algorithmic perspective, we will
% focusing on those
% we have not described earlier.

% \smallskip
\noindent
{\bf Regular Switching Algorithms.} 
Using MWM (Maximum Weighted Matching) as crossbar schedules
%, with a suitable weight measure,
is known to result in 100\% switch throughput and
near-optimal 
queueing delays under various traffic patterns~\cite{McKeownMekkittikulAnantharamEtAl1999}, but
%For a switch with $N$ input/output ports, however,
each MWM takes $O(N^{2.5}\log W)$ time to compute using the state-of-the-art algorithm~\cite{Duan2012BpMWMScaling}, where
$W$ is the maximum possible length of a VOQ. Motivated by this, 
various parallel exact or approximate 
%% AtallaCudaGiacconeEtAl2013BPAssist, BayatiShahSharma2008MWMMaxProduct
MWM algorithms ({\it e.g.,}~\cite{Fayyazi04ParallelMWM, BayatiPrabhakarShahEtAl2007Iterative}) have been proposed to reduce its time complexity. 
% Besides, several serial randomized algorithms ({\it e.g.,}~\cite{Tassiulas1998,GiacconePrabhakarShah2003SERENA}) have 
% been proposed. They have a total time complexity of only $O(N)$ yet can provably attain $100\%$ throughput. 
However, the time complexities of all these algorithms above are still too high to be used in high-line-rate high-radix switches. 

% Lin_SelectiveRequestRound_2011,
The family of parallel iterative algorithms~\cite{McKeown99iSLIP,Hu_HighestRankFirst_2018,Hu2016IterSched,Gong_QPSr_2019} generally has a low time complexity per port. However, 
their throughput and delay performances are generally much worse than those of MWM. 
We note that QPS-r~\cite{Gong_QPSr_2019}, the state-of-the-art algorithm in this family, also
builds on QPS~\cite{Gong2017QPS}.  It simply runs $r$ (a small constant) iterations of QPS to arrive at a final matching. 
We will compare our SB-QPS and SW-QPS with it in~\autoref{sec:eva}. 



% As we mentioned earlier, 
% \modifiedHL{
% MWM is the ideal crossbar schedule in that it has highest quality, can achieve 100\% throughput, and has a delay performance that is conjectured to be optimal.} However, it has a prohibitively high computational complexity of $O(N^3)$~\cite{EdmondsKarp1972}. 

% To bring down the per-node computational complexity, a few parallel or distributed algorithms have been developed that distribute this computational cost across multiple processors.
% Some representatives among them are \cite{Fayyazi04ParallelMWM, BayatiPrabhakarShahEtAl2007Iterative, BayatiShahSharma2008MWMMaxProduct, AtallaCudaGiacconeEtAl2013BPAssist}.
% A parallel algorithm with a sub-linear per-node computational complexity of $O(\sqrt{N}\log^2 N)$ was proposed 
% in~\cite{Fayyazi04ParallelMWM} for exact computation of MWM in a bipartite graph.  However, this algorithm requires the use of 
% $O(N^3)$ processors.   Another two studies, ~\cite{BayatiPrabhakarShahEtAl2007Iterative, BayatiShahSharma2008MWMMaxProduct} belong to
% the family of parallel iterative algorithms based on belief-propagation (BP). In this family, the input ports engage in multiple iterations of message 
% exchanges with the output ports to learn enough information about the lengths of all $N^2$ VOQs,
% %across 
% %the $N$ input ports, 
% so that each input port can decide on a distinct output port to match with, resulting in an MWM that is either exact or a close approximation.  Note that the BP-based algorithms do not reduce the total amount of computation or the total number of messages to exchanged, either of which is still $O(N^3)$, but the workload is distributed evenly across the input and the output ports (\ie $O(N^2)$ work for each input/output port).

% Several serial randomized algorithms, starting with TASS~\cite{Tassiulas1998} and culminating in SERENA~\cite{GiacconePrabhakarShah2003SERENA}, have been proposed that have a total computational complexity of only $O(N)$ yet can provably attain $100\%$ throughput; SERENA, the best among them, also delivers a good empirical delay performance. However, this $O(N)$ complexity is still too high for scheduling high-line-rate high-radix switches, and none of them has been successfully parallelized ({\it i.e.}, converted to a parallel iterative algorithm) yet. Notice that $O(N)$ computational complexity is not the complexity barrier for attaining $100\%$ throughput. For example, the $O(1)$ algorithm proposed in~\cite{Ye10Variable} can provably attain $100\%$ throughput, but it has very poor delay performance because it produces high-quality matchings only when the VOQs are very long. 

% \smallskip
\noindent
{\bf Batch Switching Algorithms.}
Most of the existing batch switching algorithms~\cite{Aggarwal2003EdgeColoring, Neely2007FrameBased, Wang2018ParallelEdgeColoring} 
model the process of packing the joint calendar as an edge-coloring problem, but until now, 
most practical solutions to the latter problem are centralized and have high complexity. 
For example, the Fair-Frame algorithm~\cite{Neely2007FrameBased} based on the Birkhoff von Neumann Decomposition (BvND) 
has a time complexity of $O(N^{1.5}\log N)$ per matching computation. 

A recent work, based on parallel edge coloring, has been proposed in~\cite{Wang2018ParallelEdgeColoring}. 
It pushes the per-port time complexity (per matching computation) down to $O(\log N)$.
It requires a bath size of only $O(\log N)$, but as mentioned in~\autoref{sec:intro}, the constant factor hidden in 
the big-O is very large.

% A recent work, based on parallel edge coloring, has been proposed in~\cite{Wang2018ParallelEdgeColoring}. 
% It pushes the per-port computational complexity down to $O(\log N)$ per time slot and requires a bath size of 
% $O(\log N)$. 
% However,  the constant factor hidden in the second $O(\log N)$ is very large: A batch size of $\num{3096}$ was needed for $N \!=\! 300$ as reported in~\cite{Wang2018ParallelEdgeColoring}.

% Recently, \cite{Wang2016ParallelEdgeColoring} proposes a parallel 
% batch switching algorithm based on the approach of edge coloring, 
% in which packets are grouped into batches based on their arrival times and the matching decisions are
% computed on a per-batch basis.  
% Although this algorithm has a time complexity of $O(\log N)$ 
% per time slot when using a batch size of $O(\log N)$,
% it cannot achieve $100\%$ throughput, and its delay performance appears to be much \textcolor{green}{worse than that of SERENA}. Moreover, this algorithm suffers from the batching delay issue that we have discussed in \autoref{subsec:mp}.

% The BvND-based approach \cite{Neely2007FrameBased} mentioned in \autoref{subsec:back-batching} achieves the best known provable delay guarantee for batch switching algorithms, which is $O(\log N)$ average delay for an $N\times N$ switch.  However, this algorithm has a high computational complexity of $O(N^{1.5}\log N)$ per time slot.

% CF switching \cite{rojas2007frame} is a batch switching approach that has no batching delay, which is designed to boost the throughput performance of certain parallel iterative maximal-size switching schemes ({\it e.g.,} PIM~\cite{Anderson1993PIM} and iSLIP~\cite{McKeown99iSLIP}). It dynamically selects the proper batch size for each input-output pair based on input loads, so unlike in all other algorithms mentioned in this paper, in a CF switching algorithm, the batch size for different input-output pairs could be different. More precisely, in a CF switching algorithm, each input-output pair maintains an independent counter that captures the number of remaining time slots in the current batch. When this counter decreases to zero, CF switching resets it to the length of the VOQ associated with this input-output pair. In this way, the batch size adapts to the current traffic loads, avoiding the batching delay issue.

% During each time slot, a parallel iterative algorithm ({\it e.g.} PIM or iSLIP) produces a matching, which is used to switch packets for this time slot. Here, the parallel iterative algorithm is slightly different from its regular switching counterpart in that it gives higher priority to the input-output pairs that are in the middle of their batches, completing them before serving other pairs. By doing so, the CF switching algorithm provides service to input-output pairs roughly in proportion to their arrival rates, because heavy input-output pairs are generally assigned large batch sizes. In other words, it makes ``weight-oblivious'' switching algorithms ({\it e.g.} PIM or iSLIP) ``weight-aware''. Therefore, it retains the good performance of PIM and iSLIP under uniform traffic and light traffic, yet achieves higher throughput under non-uniform traffic. 


==> SW-QPS-PERF2020(arxiv)/sections/sb-qps.tex <==
\section{Small-Batch QPS} \label{sec:sb-qps}

%In this section, we describe the design of the small-batch QPS (SB-QPS) algorithm in details.  


\subsection{Batch Switching Algorithms}\label{subsec:back-batching}


\begin{figure}[!ht]
\centering
% \includegraphics[width=0.70\columnwidth]{figures/IQ-sched-graph/joint-calendar-v2}
\includegraphics[width=0.60\columnwidth]{figures/IQ-sched-graph/scheduling-graph-standalone}
\caption{A joint calendar. ``--" means unmatched.}\label{fig:sched-graph}
%\Description{A joint calendar for batch switching algorithms.}
\end{figure}


Since Small-Batch QPS (SB-QPS) is a batch switching algorithm~\cite{Aggarwal2003EdgeColoring,Neely2007FrameBased,Wang2018ParallelEdgeColoring}, 
we first provide some background on batch switching. 
In a batch switching algorithm, the $T$ matchings for a batch of $T$ future time slots are batch-computed. 
These $T$ matchings form a joint calendar (schedule) of the $N$ output ports 
%As shown in~\autoref{fig:sched-graph}, 
%Clearly, the joint calendar (schedule) 
%of the $N$ output ports 
%over a batch of $T$ time slots 
that can be encoded  
as a $T \times N$ table with $TN$ cells in it, as illustrated by an example shown in~\autoref{fig:sched-graph}.
Each column corresponds to the calendar of an output port and each row a time slot.  
The content of the cell at the intersection of the $t^{th}$ row and the $j^{th}$ column is the input port that $O_j$ is to pair with during 
the $t^{th}$ time slot in this batch.  Hence, each cell also corresponds to an edge (between the input and the output port pair)
and each row also corresponds to a matching (under computation for the corresponding time slot).   
In the example shown in~\autoref{fig:sched-graph},
% shows an example joint calendar over a batch of $T$ (future) time slots.
% $t,t\!+\!1,\cdots,t\!+\!T\!-\!1$. 
%In this example, 
output port $O_1$ is to pair with $I_3$ during the $1^{st}$ time slot (in this batch), $I_5$ 
during the $2^{nd}$ time slot, and is unmatched during the $T^{th}$ time slot. 


At each input port, all packets that were in queue before a cutoff time (for the current batch), 
including those that belong to either the current batch, or previous batches but could not be served then,
are waiting to be inserted into the respective calendars ({\it i.e.,} columns of cells) of the corresponding output ports.  
The design objective of a batch switching algorithm is to pack as many such packets across the $N$ input ports as possible 
into the $TN$ cells in this joint calendar.   
After the computation of the current joint calendar is completed, the $T$ matchings in it will be used as the crossbar configurations for a batch of
$T$ future time slots.  In the meantime, the switch is switching packets according to the $T$ matchings specified 
in a past joint calendar that was computed earlier.  








\begin{comment}
\autoref{fig:sched-graph} shows an example joint calendar over a batch of $T$ (future) time slots.
% $t,t\!+\!1,\cdots,t\!+\!T\!-\!1$. 
In this example, output port $O_1$ is to pair with $I_3$ during the $1^{st}$ time slot (in this batch), $I_5$ 
during $2^{nd}$ time slot, and is unmatched during $T^{th}$ time slot. 
\end{comment}





\begin{comment}
% Note that the total number of such packets can exceed $TN$, in which case at 
% most $TN$ of them can be served ``in this batch''.   
At the end of this batch, the packing process finishes and the corresponding $T$ matchings are used as the crossbar 
configurations for the $T$ time slots in the next batch, or in other words, all packets packed in this 
joint calendar are switched in the next batch. % (instead of the current one).  
% As a result, batch switching algorithms suffer from the batching delay that does not exist in regular switching algorithms. 
% Clearly, the larger the batch size $T$ is, the higher this batch delay is. 
Then, at the beginning of the next batch, a new empty joint calendar is to be packed. 
Back to the example, the joint calendar shown in~\autoref{fig:sched-graph}, after finishing the packing process, is 
used to switch packets, and a new empty joint calendar corresponding to the next batch  
goes through the similar packing process, in time slots $t\!+\!T,t\!+\!T\!+\!1,\cdots,t+\!2T\!-1$.
\end{comment}

\subsection{The SB-QPS Algorithm}\label{subsec:sb-qps-alg}

In this section, we describe in detail SB-QPS, a batch switching algorithm that uses a small 
constant batch size $T$ that is independent of $N$. 
SB-QPS is a parallel iterative algorithm:  The input and output ports run 
$T$ QPS-like iterations (request-accept message exchanges) to collaboratively pack the joint calendar.     
The operation of each iteration is extremely simple:  Input ports request for cells in the joint calendar, 
and output ports accept or reject the requests.  More precisely, each iteration of SB-QPS, like that of QPS~\cite{Gong2017QPS}, 
consists of two phases: a proposing phase and an accepting phase. 

\noindent
{\bf Proposing Phase.} 
We adopt the same proposing strategy as in QPS~\cite{Gong2017QPS}. %the QPS strategy. 
In this phase, each input port, unless it has no packet to transmit, proposes to {\it exactly one} output port 
that is decided by the QPS strategy. Here, we will only describe the operations at input port $1$; 
those at any other input port are identical. Like in~\cite{Gong2017QPS}, we denote by $m_1,m_2, \cdots, m_N$ 
the respective queue lengths of the $N$ VOQs at input port $1$, and by $m$ their sum ({\it i.e.}, $m \!\triangleq\!\sum_{k=1}^N m_k$). 
At first, input port 1 simply samples an output port $j$ with probability $m_j/m$, % $\frac{m_j}{m}$, 
{\it i.e.,} proportional to $m_j$, the length of the corresponding VOQ; it then sends a proposal to output port $j$. 
The content of the proposal in SB-QPS is slightly different than that in QPS.  
In QPS, the proposal contains only the VOQ length information ({\it i.e.,} the value $m_j$),
whereas in SB-QPS, it contains also the following availability information (of input port $1$):  Out of the $T$ time slots in the batch,
what (time slots) are still available for input port $1$ to pair with an output port?
%since both will be used in the accepting phase (in SB-QPS). 
% attaching the value $m_j$ and the availability information of input $1$, 
% which will be used in the accepting phase. 
The time complexity of this QPS operation, 
% a simple 
carried out using the data structure proposed in~\cite{Gong2017QPS}, is $O(1)$ per input port.   

\noindent
{\bf Accepting Phase.} In SB-QPS, the accepting phase at an output port is quite different than that in QPS~\cite{Gong2017QPS}. 
Whereas the latter allows at most one proposal to be accepted at any output port (as QPS is a part of a regular switching algorithm that 
is concerned with only a single time slot at a time), 
the former allows an output port to accept multiple (up to $T$)  proposals (as each output port has up to $T$ cells in its calendar to be filled). 
Here, we describe the accepting phase at output port 1; that at any other output port is identical. 
The operations at output port 1 depend on the number of proposals it receives. If output port $1$ receives exactly one proposal from 
an input port (say input port $i$), it tries to accommodate this proposal using an accepting strategy we call {\it First Fit Accepting} (FFA).
The FFA strategy is to match in this case input port $i$ and output port $1$ at the earliest time slot (in the batch of $T$ time slots) 
during which both are still available (for pairing);  if they have ``schedule conflicts" over all $T$ time slots, this proposal is rejected. 
If output port $1$ receives proposals from multiple input ports, then it 
first sorts (with ties broken arbitrarily) these proposals in a 
descending order according to their corresponding VOQ lengths, and then tries to 
accept each of them using the FFA strategy.
 
%We propose the FFA strategy with the objectives of minimizing the 
%delay of each packet and of maximizing the number of packets that can be packed into the joint calendar.   
%Both objectives have clearly been achieved, as will be shown in~\ref{}.


%In SB-QPS, each output port considers and possibly accepts one or more proposals using a  {\it First Fit Accepting} (FFA) strategy, 



%If such a time slot (say the $k^{th}$ time slot) exists, then it accepts 
%the proposal and pairs with input port $i$ in $k^{th}$ time slot. 


In SB-QPS, opportunities -- in the form of proposals from input ports -- can arise, throughout the 
time window (up to $T$ time slots long) for computing the join calendar, to fill any of its $TN$ cells.  As explained earlier, 
this ``capturing every opportunity" to fill the joint calendar allows a batch switching algorithm to produce matchings of 
much higher qualities than a regular switching algorithm that is based on the same underlying bipartite matching algorithm can.   
Indeed, SB-QPS, the batch switching algorithm that is based on the QPS bipartite matching primitive, 
significantly outperforms QPS-1, the regular switching algorithm that is also based on QPS, as we will show in~\autoref{sec:eva}.



%any empty cell can possibly be 
%filled at any moment during the computation of the join calendar (that can last up to $T$ time slots).  As explained earlier, 


\noindent
{\bf Time Complexity.} 
The time complexity for the accepting phase at an output port is 
$O(1)$ on average, although in theory it can be as high as $O(N\log N)$ since an output port can receive up to $N$ 
proposals and have to sort them based on their corresponding VOQ lengths.  
Like in~\cite{Gong2017QPS}, this time complexity can be made $O(1)$ even in the worst case by letting the output port drop (``knock out") all proposals 
except the earliest few (say $3$) to arrive.
%The hardware logic for this ``dropping all but the first few" operation is quite simple and was first
%proposed in a classical output-queueing switching technology called knockout~\cite{}.  
%In our evaluations (\autoref{sec:eva}), 
In this work, we indeed 
set this threshold to $3$ and find that it has a negligible effect on the quality of resulting matchings.    

We now explain how to carry out an FFA operation in $O(1)$ time.  
%We note that the constant factor hidden in this big-O is very small when implementing with proper data 
%structures such as bitmaps. 
In SB-QPS, we encode the availability information of an input port $i$ as a $T$-bit-long bitmap $B_i[1..T]$, where $B_i[t]\!=\!1$ if input port $i$ is available (i.e., not 
already matched with an output port) at time slot $t$ and $B_i[t]\!=\!0$ otherwise.
The availability information of an output port $o$ is similarly encoded into a $T$-bit-long bitmap $B_o[1..T]$.  
%As shown in~\autoref{alg:ffa}, 
% As a result, 
When input port $i$ sends a proposal, which contains the availability information $B_i[1..T]$, to output port $o$, the corresponding FFA operation is for the output port $o$ to 
find the first bit in the bitmap $(B_i\&B_o)[1..T]$ that has value $1$, where ``$\&$" denotes bitwise-AND.  
Since the batch size $T$ in SB-QPS is a small constant 
(say $T$=16), both bitmaps can fit into a single CPU word and ``finding the first $1$" is an instruction on most modern CPUs.  

To summarize, the worst-case time complexity of SB-QPS is $O(T)$ per input or output port for the joint calendar consisting of $T$ matchings, 
since SB-QPS runs $T$ iterations and each iteration has $O(1)$ worst-case time complexity per input or output port.  Hence the worst-case 
time complexity for computing each matching is $O(1)$ per input or output port.

%process of a proposal (say one from input port $i$) at output port 1  
%is to first calculate the bitwise-AND bitmap $B$ of the availability bitmaps $B_I$ of input port $i$ 
%and $B_O$ of output port 1 (\autoref{accept:c-availability}) and then find first set (ffs) of $B$ (\autoref{accept:f-availability}), 
%{\it i.e.,} find the first (earliest) bit that is $1$ in $B$.  

 
%We note that each of the two bitmap operations ({\it i.e.,} bitwise-AND and ffs) can be accomplished in a single CPU cycle. 

%\begin{algorithm}[!ht]
%\caption{FFA process of a proposal at output port 1.}
%\label{alg:ffa}
%$B\leftarrow B_O \land B_I$\;  \label{accept:c-availability}
%$k\leftarrow\texttt{ffs}(B)$\; \label{accept:f-availability}
%\end{algorithm}

\noindent
{\bf Message Complexity.} The message complexity of each ``propose-accept'' iteration is $O(1)$ messages
per input or output port, because each input port sends at most one proposing message per iteration and each 
output port sends out at most 3 acceptance messages (where $3$ is the ``knockout" threshold explained above).  
%/output port transmits no more than one/three messages during
%the proposing/accepting phase. 
Each proposing message is $T\!+\!\lceil\log_2W\rceil$ bits long ($T$ bits for encoding the availability 
information and $\lceil\log_2W\rceil$ bits for encoding the corresponding VOQ length), where $W$ is the longest possible VOQ length. 
Each acceptance message is  
$\lceil \log_2 T\rceil$ bits long (for encoding the time slot the pairing is to be made).  
%To summarize, the worst-case message complexity of 
%SB-QPS for computing each of the $T$ matchings is $O(1)$ per port. %input or output port.  

%, with which the output port notifies the corresponding input port of each accepted proposal which time slot is assigned. 

\begin{comment}
We have considered and experimented with another accepting strategy: accepting as many as possible proposals, which we refer to as 
{\it Maximum Fit Accepting} (MFA). Unlike FFA that tries to accommodate proposals one after another 
(after sorting), during each of the $T$ iterations, MFA considers all proposals 
jointly and maximizes the number of proposals that can be accepted. 
Intuitively, MFA would pack more packets in the joint calendar and result in higher throughput than FFA.  
However, we found, through experimental evaluation, that MFA generally 
has similar or slightly worse throughput performance than FFA. 
Moreover, MFA suffers more severely from the batching delay especially when the traffic is light, since it 
does not take into the delay into consideration, more precisely, it 
might pair an output port with an input port in a time slot that is much later than the earliest available one. 
Therefore, we prefer FFA over MFA. 
\end{comment}

% The pseudocode of the FFA strategy at output port 1 is 
% shown in~\autoref{alg:accept}; that at any other output port is identical. 
% As shown in~\autoref{alg:accept}, when output port 1 receives one or more proposals, 
% it first sorts, with ties being broken arbitrarily, these proposals in a descending order of their corresponding VOQ lengths (\autoref{accept:sort})
% and then tries to accommodate them one after another in the following manner.   
% First, it gets the availability bitmap $B_I$ of the corresponding input port (input port $i$) 
% that sends the proposal $p$ (\autoref{accept:i-availability}). 
% Then, it compares $B_I$ with its own availability bitmap $B_O$, more precisely, it 
% computes their bitwise-AND bitmap $B$ (\autoref{accept:c-availability}).  
% Finally, it finds the earliest time slot during which both are available (\autoref{accept:f-availability}), {\it i.e.,} 
% the position of the first `$1$' (also referred to as the first set bit) in bitmap $B$. 
% If such a time slot $k$ exists, 
% it accepts this proposal and sends a message attached with the value $k$ to notify input 
% port $i$ (\autoref{accept:ac-availability}) so 
% that input port $i$ will update its availability bitmap, more precisely, 
% set the $k^{th}$ bit of its availability bitmap $B_I$ to $0$ ({\it i.e.,} unavailable). 
% It then updates its own availability bitmap $B_O$ similarly~(\autoref{accept:up-availability}) and 
% its own calendar (schedule)~(\autoref{accept:up-jc}). 
% The computational complexity for this ``first fit'' accepting strategy at an output port is 
% $O(1)$ on average and can be made $O(1)$ even in the worst case using the same technique as used in~\cite{Gong2017QPS}. 

==> SW-QPS-PERF2020(arxiv)/sections/scheme-long.tex <==
\section{Schemes}\label{sec:schemes}

% In this section, we describe our two batch switching algorithms in this work. Both of them use the proposal strategy as in a recent switching algorithm called Queue Proportional Sampling (QPS)~\cite{Gong2017QPS}, to be described in~\autoref{subsec:qps}. Then, we describe in detail in~\autoref{subsec:sb-qps} our first scheme, Small-Batch QPS (SB-QPS), which is a batch switching 
% algorithm. Finally, we describe in~\autoref{subsec:sw-qps} our second scheme, Sliding-Window QPS (SW-QPS), which is a SW switching algorithm.  

In this section, we describe the two proposed switching algorithms, namely SB-QPS (\autoref{subsec:sb-qps}) and SW-QPS (\autoref{subsec:sw-qps}). As mentioned earlier, both of them build upon QPS-r~\cite{qpsr}, more precisely, adopt the 
Queue Proportional Sampling (QPS) proposing strategy that is used in QPS-r. 
\begin{comment}
How many "proposals" do you want to use?
JM: most simple ... that was proposed in ~\cite{Gong2017QPS}
more specific ... Both of them use the proposal strategy from a recent switching algorithm called Queue Proportional Sampling (QPS)~\cite{Gong2017QPS}
\end{comment}
Hence, we describe the QPS proposing strategy first in~\autoref{subsec:qps}. 
% Then, we 
% describe in detail in~\autoref{subsec:sb-qps} our first scheme call Small-Batch QPS (SB-QPS), which is a traditional batch switching 
% algorithm. Finally, we describe in~\autoref{subsec:sw-qps} our second scheme, Sliding-Window QPS (SW-QPS), which is a SW switching algorithm.  

\begin{figure}
\centering
\includegraphics[width=0.80\columnwidth]{figures/IQ-sched-graph/scheduling-graph-standalone}
\caption{A joint calendar. ``--" means unmatched.}\label{fig:sched-graph}
\Description{A joint calendar for batch switching algorithms.}
\end{figure}
\subsection{Batch Switching Framework}\label{subsec:back-batching}
As mentioned earlier in~\autoref{subsec:ours},  in a batch switching algorithm, multiple (say $T$) consecutive 
time slots are grouped as a batch and these $T$ matching decisions are batch-computed. 
As shown in~\autoref{fig:sched-graph}, the joint calendar (schedule) of the $N$ output ports over a batch of $T$ time slots can be viewed as a $T \times N$ table with $TN$ cells in it.
Each column corresponds to the calendar of an output port and each row a time slot.  
The content of the cell at the $t^{th}$ row and $j^{th}$ column is the input port that $O_j$ is paired with during time slot $t$. 
For example, in~\autoref{fig:sched-graph}, output port $O_1$ is paired with $I_3$ in time slot $1$, $I_5$ in time slot $2$, and is unmatched 
in time slot $T$.
At each input port, 
all packets that were in queue before a cutoff time (for the current batch), including those that belong to either the current batch, 
or previous batches but could not be served then,
are waiting to be inserted into the respective calendars ({\it i.e.,} columns of cells) of the corresponding output ports.  
In a batch switching algorithm, the goal, 
is to pack as many such packets across the $N$ input ports as possible into the $TN$ cells in this joint calendar.  
Note that the total number of such packets can exceed $TN$, in which case at most $TN$ of them can be served in this batch.   

% \subsection{Queue Proportional Sampling (QPS)}\label{subsec:qps}
\subsection{QPS Proposing Strategy}\label{subsec:qps}
% \textcolor{green}{[We need to specify for the proposing strategy, QPS-r is the same as QPS, (and the difference of our algorithms is only in the proposal format). We directly describe our accepting strategy in 4.2, so we do not describe QPS accepting strategy here.]}
To explain QPS proposing strategy, we need first explain QPS-r, the first standalone switching algorithm that uses it. 
During each time slot, QPS-r simply runs $r$ iterations of 
QPS that is originally proposed in~\cite{Gong2017QPS} as an ``add-on'' technique to augment other switching algorithms. 
QPS computes a starter matching, which is then populated ({\it i.e.}, adding more edges to it) and refined, 
by other switching algorithms such as iSLIP~\cite{McKeown99iSLIP} and SERENA~\cite{GiacconePrabhakarShah2003SERENA}, 
into a final matching. 
To generate such a starter matching, QPS runs only one iteration that consists of two phases: a proposing phase and an accepting phase. 
Since both SB-QPS and SW-QPS use, with slight modifications that will be elaborated next, the QPS proposing strategy, %that was first proposed and used in the proposing phase in QPS, 
here we restate it for this paper to be self-contained. 
% that generates a starter matching, which is then populated ({\it i.e.}, adding more edges to it) into a final matching by other switching algorithms such as iSLIP~\cite{McKeown99iSLIP} and SERENA~\cite{GiacconePrabhakarShah2003SERENA} (such QPS-augmented algorithms are called QPS-iSLIP and QPS-SERENA, respectively). To generate such a starter matching, QPS runs only one iteration that consists of two phases: a proposing phase and an accepting phase. The proposing phase is used by both of our algorithms, but the accepting phase needs significant changes to be adapted to the frameworks of batch and SW switching. Therefore, we only describe the QPS proposing phase below, and postpone the description of our accepting strategy to \autoref{subsec:sb-qps}.

In the QPS proposing strategy, each input port, unless it has no packet to transmit, proposes to {\it exactly one} output port, which is decided by the QPS strategy. Here, we will only describe the operations at input port $1$;  those at any other input port are identical. Like in~\cite{Gong2017QPS}, we denote by $m_1,m_2, \cdots, m_N$ the respective queue lengths of the $N$ VOQs at input port $1$, and by $m$ their sum ({\it i.e.}, $m \!\triangleq\!\sum_{k=1}^N m_k$). At first, input port 1 simply samples an output port $j$ with probability $\frac{m_j}{m}$, {\it i.e.,} proportional to $m_j$, the length of the corresponding VOQ; it then sends a proposal to output port $j$, attaching the value $m_j$, which will be used in the accepting phase. The computational complexity of this QPS operation, carried out on a simple data structure that is proposed in~\cite{Gong2017QPS}, is $O(1)$ per input port.   

% In the QPS proposing phase, each input port, unless it has no packet to transmit, proposes to {\it exactly one} output port, which is decided by the QPS strategy. Here, we will only describe the operations at input port $1$;  those at any other input port are identical. Like in~\cite{Gong2017QPS}, we denote by $m_1,m_2, \cdots, m_N$ the respective queue lengths of the $N$ VOQs at input port $1$, and by $m$ their sum ({\it i.e.}, $m \!\triangleq\!\sum_{k=1}^N m_k$). At first, input port 1 simply samples an output port $j$ with probability $\frac{m_j}{m}$, {\it i.e.,} proportional to $m_j$, the length of the corresponding VOQ; it then sends a proposal to output port $j$, attaching the value $m_j$, which will be used in the accepting phase. The computational complexity of this QPS operation, carried out on a simple data structure that is proposed in~\cite{Gong2017QPS}, is $O(1)$ per input port.   

% QPS and its extensions have achieved good throughput and delay performances, but they do not achieve a perfect balance between matching quality and computation complexity. For example, QPS-SERENA achieves 100\% throughput and delay performance close to that of MWM, but it is a centralized algorithm with relatively high complexity ({\it i.e.,} $O(N)$), which prevents its applications in large high-speed switches. On the contrary, QPS-r, an extension of QPS proposed in \cite{Gong_QPSr_2019}, is a standalone parallel iterative switching algorithm that achieves the lowest possible computational complexity of $O(1)$ per port but can only attain roughly 63\% throughput in the first iteration under the uniform traffic. Although its throughput can be boosted by running multiple iterations, approximately 9 rounds are needed to achieve 90\% throughput under uniform traffic, which is also unaffordable in high-speed switches.

\subsection{Small-Batch QPS (SB-QPS)} \label{subsec:sb-qps}

% To better balance matching quality with computation complexity, we combine QPS with the batch switching framework, resulting in our first algorithm: SB-QPS. SB-QPS is a parallel iterative algorithm under the batch switching framework:  The input and output ports run a small constant number of QPS-like iterations to collaboratively pack the joint calendar. Each iteration consists of two phases, namely, a proposing phase and an accepting phase. In the proposing phase, input ports independently request for cells in the joint calendar, while in the accepting phase, output ports independently accept or reject the requests. The computational complexity of SB-QPS is $O(1)$ per port per time slot and its communication complexity is between {\bf \lbrack 2 and 3  ??\rbrack} bytes per port per time slot on average.  

% SB-QPS is a batch switching algorithm that uses a small constant batch size $T$ that is independent of $N$.
SB-QPS is a batch switching algorithm with a batch size of $T$ that is a small constant independent of $N$.
% Like QPS-r~\cite{qpsr},
Unlike most existing batch switching algorithms ({\it e.g.,}~\cite{Aggarwal2003EdgeColoring,Neely2007FrameBased}) that 
are centralized, SB-QPS is a parallel iterative algorithm: 
% \textcolor{green}{[To say it is parallel, different ports are independent in each phase. To say it is iterative, de we need to compare with regular algorithms?]} 
The input and output ports run 
$T$ QPS-like iterations (one per time slot) in a batch to collaboratively pack the joint calendar. 
Like in other batch switching algorithms, in SB-QPS, 
the final joint calendar (packed with these $T$ iterations), or in other words, the final $T$ matchings, are then 
used to transmit packets, and meanwhile a new joint calendar will be packed with another 
$T$ iterations,  in the next batch. 
% \textcolor{green}{[This part should belong to batch switching framework, not SB-QPS. It is confusing (what is batch, iteration, phase...) here.]} 
% The operation of each iteration is simple: Input ports request for cells in the joint calendar, 
% and output ports accept or reject the requests.  
% As we will show later in this section, in SB-QPS, the computational complexity of this calendar packing 
% is $O(1)$ per port per time slot. 
% and its communication complexity is between {\bf \lbrack 2 and 3  ??\rbrack} bytes per port per time slot on average.  
% Like in QPS~\cite{Gong2017QPS}, 
Each iteration of SB-QPS, like that of QPS-r described in~\autoref{subsec:qps}, 
consists of two phases: a proposing phase and an accepting phase.

\smallskip
% \noindent
% {\bf Proposing phase.} In this phase, every input port, unless all VOQs are empty, 
% proposes to a single output port in the QPS manner ({\it i.e.,} following the QPS proposing strategy). In the proposal, besides the length of the corresponding VOQ as in the original QPS, the input port also specifies its availability calendar during this batch, which is encoded as a $T$-bit bitmap $B_I[1..T]$, where $B_I[t]=1$ if this input port is available, in other words, unmatched, at the $t^{th}$ time slot in this batch; Otherwise, $B[t]=0$. 
% \smallskip
\noindent
{\bf The Proposing Phase.} 
In this phase, every input port $i$ proposes to a single output port using the QPS proposing strategy unless all VOQs 
are empty at this input port. Unlike in QPS-r where a proposal attaches only the value $m_j$ (the length of 
the corresponding VOQ), in SB-QPS, this proposal also attaches the availability of input port $i$. 

This availability information is encoded as a $T$-bit-long bitmap $B[1..T]$, where $B[t]\!=\!1$ if input port $i$ is available, 
or in other words, unmatched, at the $t^{th}$ time slot in this batch; otherwise, $B[t]\!=\!0$. 
This bitmap of each (input or output) port is initialized to all-$1$ ({\it i.e.,} all time slots in this batch are available) 
at the beginning of a batch, 
and then updated in each of the $T$ iterations, at the corresponding port. 
Since, as mentioned earlier, the batch size $T$ in SB-QPS is a small constant 
(say $T$=16) so that a $T$-bit-long bitmap can 
be fit into a single CPU word. As a result, all bitmap operations, such as bitwise-AND and find first set (ffs), that are involved in 
SB-QPS can be accomplished in one or a few CPU cycles, and thus have a computational complexity of $O(1)$.  
% In this phase, every input port, unless all VOQs are empty, 
% proposes to a single output port in the QPS manner ({\it i.e.,} following the QPS proposing strategy). In the proposal, besides the length of the corresponding VOQ as in the original QPS, the input port also specifies its availability calendar during this batch, which is encoded as a $T$-bit bitmap $B_I[1..T]$, where $B_I[t]=1$ if this input port is available, in other words, unmatched, at the $t^{th}$ time slot in this batch; Otherwise, $B[t]=0$. 

\begin{algorithm}[t]
\DontPrintSemicolon 
\SetKwProg{Proc}{Procedure}{}{}
\caption{Accepting phase at output port $1$.}
\label{alg:accept}

% \Proc{Accept()}{


    $B_O\leftarrow$ availability bitmap of output port\; \label{accept:o-availability}

    $\mathcal{P}\leftarrow$ proposals in descending order of VOQ lengths\; \label{accept:sort}

 	\ForEach{proposal $p\in \mathcal{P}$} {

 	    $i\leftarrow$ input port that sends $p$\;\label{accept:i-in}

 		$B_I\leftarrow$ availability bitmap from $p$\; \label{accept:i-availability}

 		$B\leftarrow B_O \land B_I$\; \label{accept:c-availability}

 		$k\leftarrow $ find the earliest available time slot in $B$\; \label{accept:f-availability}

 		\If{found}{

 			Accept $p$ and send $k$ to input port $i$\; \label{accept:ac-availability}

 			Update the availability bitmap $B_O$\; \label{accept:up-availability}

 			Update the calendar (of output port 1)\; \label{accept:up-jc}
 		}
 	}
            

    % }
\end{algorithm}

\smallskip
\noindent
{\bf The Accepting Phase.} The accepting phase at every output port is very different from that in QPS-r. 
The latter only allows at most one proposal to be accepted, whereas the former allows an output port to
accept multiple (up to $T$)  proposals. In this phase, we adopt the simple {\it First Fit Accepting} (FFA) strategy. 
The pseudocode of the FFA strategy at output port 1 is 
shown in~\autoref{alg:accept}; that at any other output port is identical. 
As shown in~\autoref{alg:accept}, when output port 1 receives one or more proposals, 
it first sorts, with ties being broken arbitrarily, these proposals in a descending order of their corresponding VOQ lengths (\autoref{accept:sort})
and then tries to accommodate them one after another in the following manner.   
First, it gets the availability bitmap $B_I$ of the corresponding input port (input port $i$) 
that sends the proposal $p$ (\autoref{accept:i-availability}). 
Then, it compares $B_I$ with its own availability bitmap $B_O$, more precisely, it 
computes their bitwise-AND bitmap $B$ (\autoref{accept:c-availability}).  
Finally, it finds the earliest time slot during which both are available (\autoref{accept:f-availability}), {\it i.e.,} 
the position of the first `$1$' (also referred to as the first set bit) in bitmap $B$. 
If such a time slot $k$ exists, 
it accepts this proposal and sends a message attached with the value $k$ to notify input 
port $i$ (\autoref{accept:ac-availability}) so 
that input port $i$ will update its availability bitmap, more precisely, 
set the $k^{th}$ bit of its availability bitmap $B_I$ to $0$ ({\it i.e.,} unavailable). 
It then updates its own availability bitmap $B_O$ similarly~(\autoref{accept:up-availability}) and 
its own calendar (schedule)~(\autoref{accept:up-jc}). 
The computational complexity for this ``first fit'' accepting strategy at an output port is 
$O(1)$ on average and can be made $O(1)$ even in the worst case using the same technique as used in~\cite{Gong2017QPS}. 

% {\bf Em joint calendar \& batch }
% \smallskip
% \noindent
% {\bf Accepting Phase.} The accepting phase at every output port differentiates from the Longest VOQ First (LVF) strategy in QPS-r in that an output port can accept more than one proposals in each iteration. As illustrated in \autoref{alg:accept}, if an output port receives only one proposal, it accommodates that proposal in the following steps. At first, it gets the availability bitmap $B_I$ of the corresponding input port from the proposal (\autoref{accept:i-availability}). Then, it compares $B_I$ with its own availability $B_O$, which has the same format as $B_I$, (\autoref{accept:c-availability}) and finds the earliest time slot during which both ports are available (\autoref{accept:f-availability}). If such a time slot $k$ exists, it updates its own availability bitmap $B_O[k]\gets 1$ and sends an acceptance message to remind the corresponding input port of updating its availability $B_I[k]\gets 1$ (\autoref{accept:ac-availability} and \autoref{accept:up-availability}). If an input port receives multiple proposals, it first sorts these proposals in non-increasing order of their corresponding VOQ lengths and then accommodates them one by one in the steps above. 

% \smallskip
% \noindent
% {\bf Computational Complexity.}   
% Although the operations at Lines \ref{accept:c-availability} and~\ref{accept:f-availability} in~\autoref{alg:accept} 
% appear to have a computational complexity of $O(T)$, each of them can be accomplished using a single CPU instruction within 
% one CPU cycle when $T$ is small and thus each $T$-bit-long bitmap can fit in a single CPU word. Since, as mentioned earlier, 
% $T$ in SB-QPS is a small constant (say $T$=16),  
% % This claim is based on the following observation: Both bitmaps $B_I$ and $B_O$ fit in one CPU word because their lengths equal to batch size $T$, which is a small constant independent of $N$(a typical value of $T$ is $16$). Therefore, \autoref{accept:c-availability} can be interpreted as a bitwise AND operation on two such words, while the search for the first $1$ bit in \autoref{accept:f-availability} resolves to one Bit Scan Forward (BSF) operation in x86 instruction set. Both of these operations take one clock cycle in an Intel CPU~\cite{intel-doc}. 
% the computational complexity for processing one proposal is $O(1)$. 
% The overall computational complexity for this accepting phase at an output port is 
% $O(1)$ on average and can be made $O(1)$ even in the worst case using the same technique as used in~\cite{Gong2017QPS}. 
% although in theory an output port can receive up to $N$ proposals. 
% This is because the probability for an output port to receive 
% because the the number of proposals to process can be bounded by $O(1)$. 
% Although in theory, an output port could receive up to $N$ proposals from different input ports, in practice, it can drop all subsequent proposals beyond the first three of them without significantly degrading the matching quality.

% \medskip
% \noindent
% {\bf Message Complexity.}   
% The message complexity of each ``propose-accept'' iteration in SB-QPS is no more than $\big{(}(T\!+\log_2W)\!+\!T\log_2T\big{)}$ bits per input or output port, where $W$ is the largest possible VOQ length. That is because each input/output port transmits no more than one message with $T\!+\log_2W$ bits (a $T$-bit-long bitmap and a VOQ length with $\log_2W$ bits) during the proposing phase and no more than $T$ messages each with $\log_2 T$ bits during the accepting phase.  


We have considered and experimented with another accepting strategy: accepting as many as possible proposals, which we refer to as 
{\it Maximum Fit Accepting} (MFA). Unlike FFA that tries to accommodate proposals one after another during each of the $T$ iterations, 
in each iteration, MFA considers all proposals 
jointly and maximizes the number of proposals that can be accepted. Intuitively, MFA would produce better 
matchings than FFA, however, we found, through experimental evaluation, that MFA generally 
has negligible (throughput and/or delay) performance gains over FFA. Therefore, we prefer FFA over MFA, since FFA has a much lower 
computational complexity. 


\subsection{SW Switching Framework}\label{subsec:sws}

% In this section, we present the SW switching framework. 
The SW switching framework can be viewed as a combination 
of the regular and the batch switching frameworks. On one hand, this framework, like batch switching, allows the 
matching computation (during each time slot $t$) to optimize for multiple consecutive time slots, 
say time slots $t$, $t\!+\!1$,$\cdots$, $t\!+\!T\!-\!1$. In other words, in an SW switching algorithm, the goal 
is also to pack the $TN$ cells in the corresponding joint calendar. On the other hand, this framework, like 
regular switching, produces one matching per time slot. More precisely, at the end of time slot $t$, the row in 
the joint calendar corresponding to time slot $t$ will be removed from the joint calendar and used to switch 
packets. At the same time, an empty row (all cells are ``--'') for time slot $t\!+\!T$ is added to the joint calendar as 
the last row. Clearly, in an SW switching algorithm, each row (matching) in the joint calendar can have 
up to $T$ opportunities (one per time slot) to be optimized (or refined). Therefore, these matchings can have higher qualities than 
those produced by regular switching algorithms. 

\subsection{Sliding Window QPS (SW-QPS)} \label{subsec:sw-qps} 

% In order to further reduce batching delay, Sliding Window Switching breaks the boundary of batches: By the ``student" analogy, at each time slot, one class of senior students graduate, while another class of freshmen are enrolled in the joint calendar. SW switching is able to output one matching per time slot, because in contrast to batch switching algorithms that pack the batch collectively, \autoref{alg:accept} greedily refines each matching in the joint calendar. In this manner, after a matching stays in the joint calendar for $T$ time slots, it has sufficiently accommodated the input proposals, has become ready for switching, and should be outputted immediately after that time point for the least possible packet delay. 

% Packing input proposals at the earliest commonly available time slot in \autoref{alg:accept} is not only delay optimal but also throughput optimal for greedy heuristics. It is obvious that the earliest time slots will leave the joint calendar first and have the least delay. Moreover, packing the earliest time slot leaves as many empty positions as possible on the other side of the joint calendar for future proposals. We are aware that schemes based on max-cardinal bipartite matching may accommodate more proposals than \autoref{alg:accept} for a particular iteration, but such schemes have a complexity of $O(T^{5/2})$ \cite{HopcroftKarp1973MSM}, which is not suitable for our algorithm.

The SW-QPS algorithm is a simple adaption of SB-QPS into the SW switching framework described in~\autoref{sec:sws}. 
% In each time slot $t$, each input port first sends a proposal to an output port,   
% attaching the length of the corresponding VOQ and its availability bitmap, according to the QPS proposing strategy; 
% each output port then accepts one or more proposals to pack the joint calendar according to the FFA strategy 
% described in~\autoref{alg:accept}. 
More precisely, SW-QPS is also a parallel iterative algorithm, each iteration of which is identical to that of SB-QPS. 
The only difference, caused by this adaption, is that, the joint calendar in SW-QPS slides over the time line 
(one time slot per iteration) to ``capture'' the schedules 
of $T$ (consecutive) time slots starting from the current one (or in other words, these $T$ time slots are 
different from one iteration to another) in each of the $T$ iterations, whereas in SB-QPS, the joint calendar captures the 
schedules for the same $T$ time slots ({\it i.e.,} the $T$ time slots in the current batch) during all the $T$ iterations. 

% after an iteration (say the iteration during time slot $t$), \textcolor{green}{the only difference is due to SW switching}
% the earliest row (the row corresponding to time slot $t$) of the 
% joint calendar is ``removed'' and used to transmit packets at the end of time slot $t$, and 
% meanwhile, an empty row is added to the joint calendar as the matching for time slot $t\!+\!T$. 

% \begin{figure}
% \centering
% \includegraphics[width=0.86\columnwidth]{figures/examples/sb-vs-sw}
% \caption{An illustrative example: SB-QPS vs. SW-QPS.}\label{fig:sb-vs-sw}
% \Description{The solid tables are the joint calendars that are being packed or to be packed. The dashed rows are the final matchings. 
% Here we assume the batch size $T$=2 and $\tau$ is the beginning time slot of a batch. $\tau^-$ (or $\tau^+$) means the beginning (or the end) of the time slot $\tau$.}
% \end{figure}

% \autoref{fig:sb-vs-sw} compares SB-QPS with SW-QPS using a simple example. In this example, we assume that the batch size 
% $T$=2 and time slot $\tau$ is the first time slot of a batch. Note that $\tau^-$ (or $\tau^+$) suggests the beginning (or the end) \textcolor{green}{compared with +/-, I would rather say in SW switching, the movement of the sliding window happens after the two phases in each iteration, so the beginning of each time slot is the same as the end of the last one.}
% of time slot $\tau$. In~\autoref{fig:sb-vs-sw}, the solid tables are the joint calenders that are being or to be packed, whereas 
% the dashes rows are the final matchings. The highlighted (in bold font) rows are the final matchings that are used 
% to transmit packet during corresponding time slots. As shown in~\autoref{fig:sb-vs-sw}, each row (matching) in both SB-QPS and 
% SW-QPS are ``refined'' twice thus have similar quality. 

Though both SW-QPS and SB-QPS have the lowest possible per-port computational complexity 
({\it i.e.}, $O(1)$), We prefer SW-QPS over SB-QPS for the following two reasons. 
First, SW-QPS produces matchings in 
a more timely manner so that it does not suffer from the batching delay. As a result, the delay performance of 
SW-QPS is generally better than, and, when the traffic is low or moderate, significantly better than, that of SB-QPS. 
Second, the throughput performance of SW-QPS is generally better than that of SB-QPS. 
Both will be shown in the next section. 
% SB-QPS has to 
% maintain $2T$ matchings: $T$ matchings for the schedules calculated in the previous batch and 
% $T$ matchings to be calculated in the current batch. 
% Therefore, it requires $2T\cdot\log_2 N$ bits of memory per output port. 
% SW-QPS only needs to maintain $T$ matchings. Thus, SW-QPS has much less memory overhead. 

==> SW-QPS-PERF2020(arxiv)/sections/scheme.tex <==

% from qpsr
\section{Queue Proportional Sampling}\label{sec:qps}
Queue Proportional Sampling (QPS) was used in~\cite{Gong2017QPS} as an ``add-on'' to augment other switching algorithms as follows.  It generates a starter matching, which is then
populated ({\it i.e.}, adding more edges to it) and refined, by other switching algorithms such as iSLIP~\cite{McKeown99iSLIP} and SERENA~\cite{GiacconePrabhakarShah2003SERENA}, into a final matching.
%Two such augmented switching algorithms
%were proposed in~\cite{Gong2017QPS}:  QPS-iSLIP and QPS-SERENA.
To generate such a starter matching, QPS needs to run only one iteration, 
which
%, \hlb{as mentioned earlier in~\autoref{sec:intro}},  
consists of two phases, namely,
a proposing phase and an accepting phase. \textbf{In this paper, we will use the proposing phase of QPS, so}
% The computational and communication complexities of QPS ({\it i.e.}, this single iteration)
% are both $O(1)$, as we will elaborate next.
we briefly describe it in this section for this paper to be self-contained.

In the proposing phase, each input port proposes
to {\it exactly one} output port -- decided by the QPS strategy
-- unless it has no packet to transmit.
Here we will only describe the operations
at input port $1$;  that at any other
input port is identical.
Like in~\cite{Gong2017QPS}, we denote by $m_1,m_2,\cdots,m_N$
the respective queue lengths of the $N$ VOQs at input port $1$,
and by $m$
their total ({\it i.e.}, $m \!\triangleq\!\sum_{k=1}^N m_k$).
Input port 1 simply samples an output
port $j$ with probability $\frac{m_j}{m}$,
{\it i.e.,} proportional to $m_j$, the length of the corresponding VOQ (hence the name QPS);
it then proposes to output port $j$, with the value $m_j$ that will be used in the next
phase.
The computational complexity of this QPS operation, carried out using a simple data structure proposed in~\cite{Gong2017QPS},
is $O(1)$ per (input) port.   
% The communication complexity of this phase is $\log W$ bits per port ($W$ is the maximum possible VOQ length), which can be viewed as a constant (independent of $N$).

%where $W$ is the maximum possible length of a VOQ (in number of cells).
%In almost all conceivable real-world switching scenarios, we can consider $\log W$ to be $O(\log N)$
\section{Schemes}\label{sec:scheme}
In this section, we present two schemes, called Small Batch QPS (SB-QPS) and Sliding Window QPS (SW-QPS). SB-QPS is a batch scheduling algorithm proposing in the QPS manner, while SW-QPS is the combination of QPS proposing with Sliding Window Switching, improving SB-QPS for better delay and throughput performances.
\subsection{SB-QPS}

Since the batch-computation of these $T$ matchings
often has lower time complexity than
$T$ independent matching computations, the amortized (over the $T$ time slots) time complexity of a batch switching
algorithm is often lower than that of a regular switching algorithm.  
It is desirable for this $T$ to  be small because the average packet delay is at least $T$:  
A packet arriving at
the beginning of a batch has to wait till at least the beginning of the next batch to be switched.
%Exacerbating this problem, the frame size $T$ is quite large and grows as at least $O(\log N)$ in almost all existing frame-based algorithms for reasons
%that we will explain in ...

\textbf{JM}
Batch switching algorithms have the advantage of lower amortized time complexity over running $T$ independent computations of a regular switching algorithm, but they pay large delays: packets arriving uniformly from $t+1$ to $t+T$ must wait for switching until $t+T$, the finish time of the current batch, resulting in an average batching delay of at least $T/2$ that is linear to batch size.\textbf{may be moved to motivation}

Many existing batch switching algorithms use big batches (e.g. the batch size of \cite{Aggarwal2003EdgeColoring} is $\omega(n^2$)) and consequently suffer from large batching delays. Therefore, aiming for less packet delay, it is desirable to reduce batch size without sacrificing much throughput.

% proposal
\textbf{The computation of a batch consists of multiple iterations of message exchanges, one iteration for a time slot.} Each iteration (say in the $t^{th}$ time slot of a batch, $1\leq t \leq T$) consists of two phases, namely, a QPS-proposing phase and an accepting phase.
\textcolor{green}{[JM: symbol $t$ is not clear at this point]}

\medskip
\noindent
{\bf Proposing phase.}
In this phase, each input port proposes to exactly one output port in the QPS manner.  In each proposal, the input port specifies its availability calendar during the previous $t-1$ time slots, encoded as a $(t-1)$-bit bitmap, \textbf{with a 1-bit for an available slot and a 0-bit for an occupied slot}. 

\medskip
\noindent
{\bf Accepting phase.}  
When an output port receives multiple proposals, it accommodates the proposals one by one ordered by 
their corresponding VOQ lengths.  For each proposal, it compares its own availability 
during the first $t$ time slots (i.e., up to ``now") with that of the input port, and pair with the input port at the earliest time slot during which both are available.  

\textcolor{green}{Dangling Sentences:}
The $t^{th}$ iteration refines the matchings in the first $t$ time slots of the joint calendar.

\medskip
\noindent
{\bf Complexity Analysis} The time complexity for comparing two availability calendars seems to be $O(t)$ at first sight, but in fact there is an $O(\log t)$ implementation: we can perform an AND operation of these two bitmaps, and then find the earliest commonly available slot with a priority encoder with $O(\log t)$ layers.

\textbf{QPS} %The computational complexity of this accepting strategy is $O(1)$ in practice although in theory an output port could receive up to $N$ proposals and have to compare their accompanying VOQ lengths. 
\textbf{The number of proposals received by each output is $O(1)$ in practice although it might be $O(N)$ in worst case.}  This is because the probability 
for an output port to receive proposals from more than several (say $3$) input ports is tiny, and even if this 
rare event happens, the output port can ignore/drop all proposals beyond the first several (say $3$) 
without affecting the quality of the final matching much.  In our evaluations, we indeed set this threshold to $3$.

Multiplying the complexity of each proposal by the number of proposals, the time complexity of the accepting phase at each output port is $O(\log T)$ in general.

\subsection{Sliding Window Scheduling}
With SB-QPS, the batching delay can be limited to a small constant $T$, but it is still a major component of packet delay under low traffic loads. (A typical value of $T$ is $30$ time slot, while average delay is below $1$ slot under normalized load $0.5$.)

The primary idea to reduce batching delay is to break the boundary of batches. In SB-QPS, we have already designed the accepting phase to pack proposals at the earliest commonly available time slot, but the problem is that they have to wait until the beginning of next batch to become ready for switching. Actually, we observe that the ``earliest commonly available time slot matching" does not need \textbf{monolithic} batches to compute, but can be incrementally refined by the unit of each time slot. 

This leads to the idea of Sliding Window Switching: at each time slot, the matching in the earliest slot of the joint calendar matures and leaves for switching, while an empty slot is added to the tail of the availability calendar. In this manner, a matching stays in the joint calendar for $T$ time slots, which is considered sufficient for accommodating proposals, and becomes ready for switching immediately after that for the least possible packet delay. Towards the end of its stay, it becomes one of the earliest time slots in the joint calendar and gains a high priority of accommodating proposals. Therefore, the choice of the earliest commonly available time slot to pack proposals is not only delay optimal but also throughput optimal: leaving as many empty positions as possible \textbf{at the far side} of the joint calendar for future proposals.

The availability calendar for SW-QPS proposals is always of fixed length, containing $T$ bits for the next $T$ time slots to come. The benefits of fixed length proposals are \textbf{higher hardware utilization} and higher throughputs because there are more positions to pack input proposals than SB-QPS.

Here we specify the scheme of the two phases of SW-QPS. Despite the differences in the availability calendar and the timing when matchings mature, the two phases of SW-QPS in each iteration resemble SB-QPS. 

\medskip
\noindent
{\bf Proposing phase.}
Every input port also proposes in the QPS manner, specifying its availability calendar for the next $T$ time slots with a $T$-bit bitmap. 

\medskip
\noindent
{\bf Accepting phase.}
In the accepting phase, as in SB-QPS, multiple proposals are accommodated one by one ordered by 
their corresponding VOQ lengths. For each proposal, the output port pairs with the input port at the earliest commonly available time slot. 

\medskip
\noindent
{\bf Complexity Analysis.}
The message complexity of SW-QPS is $O(T+W)$, where $W$ is the number of bits used to encode VOQ lengths, and the time complexity of SW-QPS is $O(\log T)$ for each port, the same as SB-QPS, if the availability calendar is implemented with a circular queue and the accepting phase is implemented with a priority encoder with (circular) programmable priorities. In simulation, we can achieve about 90\% throughput over various traffic patters with a small batch size $T=16$ and no penalty of batching delays.





==> SW-QPS-PERF2020(arxiv)/sections/sliding-window.tex <==
\section{Sliding-Window (SW) Switching }\label{sec:sws} 

In this section, we first describe the Sliding-Window (SW) switching in detail. 
% Then, we explain how SW 
% switching eliminates the batching delays in batch switching algorithms. 
We next compare SW switching with 
Captured-Frame (CF) switching~\cite{rojas2007frame}, another ``batch switching'' approach that can be used to eliminate the 
batching delays in batch switch algorithms. 

\subsection{SW Switching: A New Batch Switching Approach}\label{subsec:sws}

A straightforward idea to overcome the batching delay issue of a batch 
switching algorithm is to let the algorithm to 
output one matching per time slot during the current batch 
instead of producing $T$ matchings at the end of this batch. 
Unfortunately, in most of the existing 
batching algorithms, these $T$ matchings are computed and 
refined together, and can only have high enough quality at the end of 
each run of the algorithms. In other word, naively outputting one 
matching per time slot results in lower-quality matchings. 

% % may not be required
% {\bf Compare with other approaches!}  
% We note that an alternative approach to overcome this batching delay issue 
% is to adapting batch size dynamically according to traffic conditions, like 
% what is done in~\cite{rojas2007frame}. 
% Such an approach is not preferable because of two major reasons. 
% On one hand, it is not easy to measure the traffic accurately. 
% On the other hand, dynamically adapting batch size requires one extra round of message 
% exchange to determine the batch size before starting the switching algorithm, which 
% incur extra communication overhead and is difficult to implement in a distributed manner. 

% \textbf{JM: It is easy to measure the traffic load on each VOQ, but it is difficult to summarize these queue lengths to select a suitable batch size for all input ports. The throughput performance of \cite{rojas2007frame} relys on its 3-round request-grant-accept scheme, which has higher message and time complexity.}

In this work, we propose a new batch switching approach to overcome 
the batching delay issue. We call it the Sliding Window (SW) switching.  
Like a traditional batch switching algorithm, a SW switching algorithm 
packs the joint calendar with $TN$ cells for all input and output ports during 
each run. However, each run of a SW switching 
algorithm takes only a time slot (instead of a batch) and at the end of each run, 
the first row (say  the $t^{th}$ row) of 
the joint calendar is used to transmit the packets during this time slot and 
removed from the joint calendar. 
At the same time, a new row (an empty schedule for time slot $t+T$) corresponding 
to the schedule of time slot 
$t+T$ is added as the last one of the joint calendar. 
With such a switching framework, each schedule (each row of the joint calendar), 
after its initialization (adding \textcolor{green}{being added} to the 
joint calendar), is refined by $T$ runs of the switching algorithm. Thus, 
each matching has the same or even higher quality 
as those computed by the traditional batching switching algorithms. 
\autoref{fig:batch-vs-sw} shows compares the traditional batch switching with the SW switching. 


As in the left side of Figure \ref{fig:batch-vs-sw}, each batch in Batch Switching contains $T$ consecutive time slots and different batches do not overlap. The scheduler packs incoming packets into Batch 1 during the period $t+1$ to $t+T$. At time slot $t+T$, all $T$ matchings in Batch 1 become ready for switching and the scheduler moves to Batch 2. 

In Sliding Window Switching, however, consecutive batches overlap on $T-1$ time slots. At time slot $t+1$, the first time slot of the Batch 1 becomes ready for switching and leaves the batch. All other time slots then join Batch 2, together with a new empty time slot appended to the end of Batch 2.

In contrast to Batch Switching, Sliding Window Switching allows new packets to directly jump to the first time slot of the joint calendar and to be switched immediately, without having to wait for the beginning of next batch, as long as there are enough empty positions in the joint calendar. This flexible behavior, having one matching ready at each time slot, is crucial to the reduction of batching delay to a $O(1)$ order under low traffic loads. Meanwhile, Sliding Window Switching is simple to implement and preserves the advantage of of Batch Switching: achieving high throughput with low complexity. 

{\bf Maybe the following section should be moved to the related work}
\subsection{SW Switching vs. CF Switching}\label{subsec:sw-vs-cf}

As we have shown, SW switching is a batching-delay-free batch switching approach. 
In the literature, the only other batching-delay-free batch switching approach that we are aware of is CF switching~\cite{rojas2007frame}. 
CF switching is an approach to dynamically select proper \textcolor{green}{the} batch size for each input-output pair based on input loads, which was 
designed to boost the throughput performance of certain parallel iterative maximal-size switching schemes ({\it e.g.,} PIM~\cite{Anderson1993PIM} and iSLIP~\cite{McKeown99iSLIP}). 

Unlike in a traditional batch switching algorithm and a SW switching algorithm, in a CF switching algorithm, the batch size for 
different input-output pairs could be different. More precisely, in a CF switching algorithm, each input-output pair between the $i^{th}$ input port and the $j^{th}$ output port 
maintains a counter $c_{i,j}$ that captures the number of remaining time slots in the current batch of this input-output pair. When this 
counter $c_{i,j}$ decreases to zero ({\it i.e.,} the end of a batch), 
the batch size of a new batch is set to the length of the $j^{th}$ VOQ at input port $i$.  
% and the counter $c_{i,j}$ is updated to the new batch size. 
During each time slot, a matching (schedule) is computed 
with a parallel iterative maximal-size matching algorithm and used to switch packets for this time slot (thus batching-delay-free). Here, the parallel iterative algorithm is slightly different from its regular-switching counterpart in that it gives higher priority to the input-output pair whose counter $c_{i,j}$ 
at the previous time slot is larger than $1$ (or in other words, the current time slot is not the beginning of a new batch). Doing so, 
the CF switching algorithm roughly achieves to provide service to input-output pairs in proportion to their arrival rates, or in other words, 
it makes ``weight-oblivious'' switching algorithms ({\it e.g.} PIM or iSLIP) ``weight-aware''. Therefore, it retains the good performance 
under uniform traffic and light traffic, yet achieves higher throughput under non-uniform traffic. 

Both SW switching and CF switching resolve the batching delay issue of the traditional batching switching algorithms. However, there are three 
key differences. First, in a CF switching algorithm, $N^2$ counters are required to capture the number of remaining time slots for 
the $N^2$ input-output pairs, which makes it difficult to scale to switches with large $N$. Second, CF switching achieves high throughput 
by making ``weight-oblivious'' switching algorithms ``weight-aware'', where the batch concept is just used for poritorize \textcolor{green}{prioritize} input-output 
pairs, whereas SW switching achieves high throughput by refining each matching again and again before it is used to switch packets. Last, unlike in SW switching algorithms, there is only one matching being computed during each time slot in a CF switching algorithm.


==> SW-QPS-PERF2020(arxiv)/sections/sw-qps.tex <==
\section{Sliding-Window QPS}\label{sec:sw-qps}

In this section, we present in detail the Sliding-Window QPS (SW-QPS) algorithm, the final and only research product of this work.  
Before we do so, we describe next the sliding-window framework that SW-QPS builds on.  


%The SB-QPS algorithm has a shortcoming: the batching delay. In this section, we propose 
%a novel algorithm, call SW-QPS, that eliminates this batching delay, and retains and enhances all benefits of SB-QPS.

\subsection{Sliding-Window Switching}\label{sec:sw-s}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.95\columnwidth]{figures/IQ-sched-graph/sw-switching}
\caption{Sliding-window switching.}\label{fig:sws}
%\Description{Sliding-window switching.}
\end{figure}

As mentioned earlier, the only difference between SW-QPS and SB-QPS is that SW-QPS changes the batch switching operation of SB-QPS to a 
sliding-window switching operation.  
Sliding-window switching combines regular switching with batch switching and gets the better of both worlds, as follows.
On one hand, during each time slot, under a sliding-window switching operation,  
there are $T$ matchings under computation, just like under a batch switching operation.
Each such matching has had or will have a window of $T$ time slots to find opportunities to have its quality improved 
by the underlying bipartite matching algorithm before it ``graduates''.
%during any of the $T$ time slots in a sliding window (similar to a batch in the batch switching)  
Hence, each such matching, when it ``graduates", can have a similar or even better quality than that computed by 
the batch switching algorithm that is based on the same 
underlying bipartite matching algorithm, as will be confirmed in~\autoref{sec:eva}. 

On the other hand, under a sliding-window switching operation, the ``windows of opportunities" of these $T$ matchings are staggered so that 
one matching (``class") is output (``graduated") every time slot.   This matching is to be used as the crossbar configuration for the current time slot. 
In this respect, it behaves like a regular switching algorithm and hence 
completely eliminates the batching delay of the batch switching.    
More specifically, at the beginning of time slot $t$, the most senior matching (``class") 
in the window was added (``enrolled") to the window at the end of time slot $t - T - 1$ and is to ``graduate" at the beginning of time slot $t$, so its ``window of opportunity"
(to have its quality improved) is $[t - T, t-1]$.  The ``window of opportunity" for the second most senior matching is $[t - T + 1, t]$ and so on.  
%the sliding-window switching, like the regular switching, produces one matching every time slot. 
%More precisely, it ``graduates the most senior class'', the ``oldest'' matching (among the $T$ matchings) 
%whose quality has been improved for up to $T$ time slots, and uses this matching as the crossbar configuration for the current time slot. 
At the end of time slot $t$, a ``freshman class'' (an empty matching) is ``enrolled" and scheduled to ``graduate" at time slot $t + T + 1$ in the future.  

%, and thus there are still $T$ matchings under computation during the next time slot.
%Recall that a batch switching algorithm outputs, every $T$ time slots, a batch of 
%$T$ matchings to be used as the crossbar schedules for a batch of $T$ future time slots.   In comparison, a sliding-window switching algorithm 
%outputs (``graduates"), every time slot, one matching (``class") to be used now (i.e., for the current time slot).   

\autoref{fig:sws} shows how the sliding window evolves from time slot $t$ to time slot $t+1$.  In~\autoref{fig:sws}, each interval along the timeline corresponds to 
a ``class".   
As shown in~\autoref{fig:sws}, at the beginning of time slot $t$, the current window contains 
``classes of years" (matchings-under-computation to be used as crossbar schedules for time slots) 
$t$, $t+1$, $\cdots$, and $t + T - 1$.  Then, at the beginning of time slot $t+1$, the current window slides right by $1$ (time slot), and the
new window contains ``classes of years" $t+1$, $t+2$, $\cdots$, and $t+T$,
because the ``class of year $t$" just graduated and the ``class of year $t+T$" was just ``enrolled".   

In theory, almost any batch switching algorithm can be converted into a sliding-window switching algorithm by making the ``windows of opportunity" for 
the batch of $T$ matchings-under-computation staggered instead of aligned.   This conversion would in general improve switching performance by eliminating the batching delay. 
Hence, this sliding-window switching framework is itself a separate
contribution of this work.  



\begin{comment}

To the best of our knowledge, the 

Each ``class" corresponds to a matching being computed

The sliding window at time slot $t$ 

that can in theory be used to possibly boost the delay performance
of any batching switching algorithm.

SW-QPS 
As mentioned earlier, the  a novel sliding window algorithmic framework, SW-QPS eliminates this batching delay, and retains and enhances all benefits of SB-QPS


Recall from~\autoref{sec:intro} that SW-QPS is based on a novel switching framework, called the 
sliding-window switching, that was first proposed in this work. 
We describe it in detail here before delving into the SW-QPS algorithm. 



\noindent
{\bf An Illustrative Example.} The joint calendar, shown in~\autoref{fig:sched-graph}, 
can also illustrate the $T$ matchings-under-computation at the beginning of time slot $t$ in a slide-window switching algorithm. 
During time slot $t$, the qualities of some of all these matchings will be improved (by the underlying bipartite matching algorithm), {\it i.e.,} 
more packets being packed, 
and then at the end of time slot $t$, the matching corresponding to the oldest time slot, {\it i.e.,} time slot $t$, in this sliding window, 
will ``graduate'' (or the $1^{st}$ row of this joint calendar will be removed) and be used as the crossbar configuration for time slot $t$. 
At the same time, a new empty row, the matching corresponding to time slot $t\!+\!T$ will be added to arrive at a new joint calendar that also includes $T$ matchings. 


\end{comment}

\subsection{The SW-QPS Algorithm} \label{subsec:sw-qps-alg} 

% In order to further reduce batching delay, Sliding Window Switching breaks the boundary of batches: By the ``student" analogy, at each time slot, one class of senior students graduate, while another class of freshmen are enrolled in the joint calendar. SW switching is able to output one matching per time slot, because in contrast to batch switching algorithms that pack the batch collectively, \autoref{alg:accept} greedily refines each matching in the joint calendar. In this manner, after a matching stays in the joint calendar for $T$ time slots, it has sufficiently accommodated the input proposals, has become ready for switching, and should be outputted immediately after that time point for the least possible packet delay. 

% Packing input proposals at the earliest commonly available time slot in \autoref{alg:accept} is not only delay optimal but also throughput optimal for greedy heuristics. It is obvious that the earliest time slots will leave the joint calendar first and have the least delay. Moreover, packing the earliest time slot leaves as many empty positions as possible on the other side of the joint calendar for future proposals. We are aware that schemes based on max-cardinal bipartite matching may accommodate more proposals than \autoref{alg:accept} for a particular iteration, but such schemes have a complexity of $O(T^{5/2})$ \cite{HopcroftKarp1973MSM}, which is not suitable for our algorithm.

SW-QPS is exactly such a conversion of the batch switching algorithm SB-QPS into a sliding-window switching algorithm.  
%algorithm is a simple adaption of SB-QPS into the sliding-window switching framework described above. 
SW-QPS is also a parallel iterative algorithm whose each iteration is identical to that of SB-QPS.  Hence SW-QPS 
has the same $O(1)$ time and $O(1)$ message complexities (per port per matching computation)
as SB-QPS.  
The only major difference is that, SW-QPS ``graduates'' a matching every time slot whereas SB-QPS ``batch-graduates" $T$ matchings every $T$ time slots. 
This ``graduating a class each year" allows SW-QPS to completely eliminate the batching delay.
As explained earlier, in SW-QPS, at the beginning of time slot $t$, the joint calendar consists of the $T$ matchings-under-computation that are to ``graduate" in 
``years" (time slots) $t$, $t+1$, $\cdots$, $t + T - 1$ respectively.  Hence at time slot $t$, the $T$-bit-long availability bitmap of an input port $i$ indicates the availabilities of 
$i$ during $[t, t + T -1]$.   

Note that SW-QPS inherits the FFA (First Fit Accepting) strategy of SB-QPS that is to arrange for an input-output pairing -- 
and hence the switching of a packet
between the pair -- at the earliest mutually available time slot.  In other words, an incoming packet is always ``advanced to the most senior class that it can fit in
schedule-wise" so that it can ``graduate'' at the earliest ``year'' possible. 
This greedy strategy further reduces the queueing delay of a packet, as will be shown 
in~\autoref{sec:eva}.

%(described in~\autoref{subsec:sb-qps-alg}) also guarantees 
%that Hence, SW-QPS reduces the batching delay to zero. 

%This conversion provides more performance benefits when the
%batching switching algorithm is ``front-loaded" (defined earlier), as we will elaborate next.

\begin{comment}
Though both SW-QPS and SB-QPS have the lowest possible per-port time complexity 
({\it i.e.}, $O(1)$ per matching computation per port), 
we prefer SW-QPS over SB-QPS and consider SW-QPS as the only final product of this work for the following two reasons. 
First, as explained above, SW-QPS does not suffer from the batching delay. As a result, the delay performance of 
SW-QPS is generally better than, and, when the traffic is low to moderate, significantly better than, that of SB-QPS. 
Second, the throughput performance of SW-QPS is also better than that of SB-QPS. 
Both will be confirmed in~\autoref{sec:eva}.  
\end{comment}

==> SW-QPS-PERF2020(arxiv)/sections/sw-switching.tex <==
\section{SW Switching Framework}\label{sec:sws}

% In this section, we present the SW switching framework. 
The SW switching framework can be viewed as a combination 
of the regular and the batch switching frameworks. On one hand, this framework, like batch switching, allows the 
matching computation (during each time slot $t$) to optimize for multiple consecutive time slots, 
say time slots $t$, $t\!+\!1$,$\cdots$, $t\!+\!T\!-\!1$. In other words, in an SW switching algorithm, the goal 
is also to pack the $TN$ cells in the corresponding joint calendar. On the other hand, this framework, like 
regular switching, produces one matching per time slot. More precisely, at the end of time slot $t$, the row in 
the joint calendar corresponding to time slot $t$ will be removed from the joint calendar and used to switch 
packets. At the same time, an empty row (all cells are ``--'') for time slot $t\!+\!T$ is added to the joint calendar as 
the last row. Clearly, in an SW switching algorithm, each row (matching) in the joint calendar can have 
up to $T$ opportunities (one per time slot) to be optimized (or refined). Therefore, these matchings can have higher qualities than 
those produced by regular switching algorithms. 






% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.295\textwidth]{figures//IQ-sched-graph/sliding-schedule}
% 	% \caption{An illustration of the joint calendar of Sliding Window switching: The label of each row (matching) is its time slot of completion.}
% 		\caption{The SW scheduling framework.}
% 	\label{fig:batch-vs-sw}
% \end{figure}

% As shown in \autoref{fig:batch-vs-sw}, in contrast to batch switching, as long as there are enough empty positions in the joint calendar, SW switching allows new packets to directly jump to the first row of the joint calendar and to be switched immediately, without having to wait for the beginning of next batch. This flexible behavior, having one matching ready at each time slot, is crucial to the reduction of batching delay to a $O(1)$ order under low traffic loads. Meanwhile, Sliding Window Switching is simple to implement and preserves the advantage of of Batch Switching: achieving high throughput with low complexity. 

==> SW-QPS-PERF2020(arxiv)/sections/title_and_authors.tex <==
% \title{Sliding Window QPS (SW-QPS)}
%[SW-QPS]
\title{Sliding-Window QPS (SW-QPS):  A Perfect Parallel Iterative Switching Algorithm for Input-Queued Switches}

% Georgia Institute of Technology, USA
% \author{Jingfan Meng, \qquad\qquad\quad Long Gong, \qquad\qquad\quad Jun (Jim) Xu\\
% 	Georgia Institute of Technology\\
% 	jmeng40@gatech.edu,\quad gonglong@gatech.edu,\quad jx@cc.gatech.edu
% }

\def\saddr{Georgia Tech}
\numberofauthors{3}
\author{
\alignauthor Jingfan Meng\\
 \affaddr{\saddr}\\
 \email{jmeng40@gatech.edu}
\alignauthor Long Gong\\
 \affaddr{\saddr}\\
 \email{gonglong@gatech.edu}
 \alignauthor Jun (Jim) Xu\\
 \affaddr{\saddr}\\
 \email{jx@cc.gatech.edu}
}

% \date{dsa}
%\affiliation{Georgia Institute of Technology}\email{}
%\author{Long Gong}
%\affiliation{Georgia Institute of Technology}\email{gonglong@gatech.edu}
%\author{Jun (Jim) Xu}
%\affiliation{Georgia Institute of Technology}\email{jx@cc.gatech.edu}
\maketitle

==> libs/common_used_packages.tex <==
%% packages for figures
\usepackage{graphicx}
\usepackage{color}
\usepackage{graphics}

%\usepackage[sort,compress]{cite}
%\usepackage{enumerate}

%% packages for citation
% \usepackage[sort]{cite}
%% for highlighting
%\usepackage{soul}
\newcommand{\st}[1]{}

%% packages for math
%\usepackage{bbm}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
%\usepackage{latexsym}
%\usepackage{mathtools}
%\usepackage{cuted}
% This package reimplements the LATEX verbatim and verbatim* environments.
% In addition it provides a comment environment that skips any
% commands or text between \begin{comment} and the next \end{comment}.
\usepackage{verbatim}


\usepackage{textcomp}
% The pack­age trans­lates var­i­ous stan­dard and other in­put en­cod­ings into a 
% ‘LATEX in­ter­nal lan­guage’. The in­ter­nal lan­guage is ex­pressed en­tirely in
% TEX's base en­cod­ing (stan­dard ASCII print­able char­ac­ters, car­riage con­trol
% to­kens and TEX con­trol se­quences, the lat­ter mostly de­fined by LATEX).
\usepackage[latin1]{inputenc}


%% packages for multirow
\usepackage{multirow}


%% for tables 
\usepackage{booktabs}

%% packages for url
\usepackage{url}

%% newly added
% \usepackage{floatrow}

%% for balanced columns
\usepackage{balance}
% % captions and subcaptions
% % \usepackage[caption=false,position=bottom]{subfig}
% \usepackage{caption}
% % % \let\subcaption\relax
% % % \let\subfloat\relax
% % %\usepackage{subcaption}
% % % \usepackage[caption=false,position=bottom]{subcaption}
% % % \let\subbottom\subfloat % to allow use of \subbottom instead of \subfloat
% % %% comment out since acmart has its own setting
% \captionsetup[figure]{textfont={small}}
% \captionsetup[table]{textfont={small}}
% \captionsetup[subfloat]{textfont={footnotesize},subrefformat=parens}

% hyperlinks, which caused some fof the grief above
%\let\captioncaption\caption
% \usepackage{aliascnt} % for custom autoref
\hypersetup{
	colorlinks = true,
linkcolor=blue,
citecolor=blue,
urlcolor=blue,
pdftitle={Sliding Window QPS}
} % hyperref is load by acmart
%\PassOptionsToPackage{unicode}{hyperref}
% \usepackage[colorlinks,
% linkcolor={red!50!black},
% citecolor={blue!50!black},
% urlcolor={blue!80!black},
% pdftitle={SERENADE}]{hyperref}
%% packages for algorithms
% \usepackage[lined,boxed,linesnumbered,commentsnumbered]{algorithm2e}
\usepackage[lined,boxed,linesnumbered,vlined]{algorithm2e}
% \usepackage{algpseudocode}

% The etoolbox package is a toolbox of programming tools geared primarily towards
% LaTeX class and package authors. It provides LaTeX frontends to some of the new
% primitives provided by e-TeX as well as some generic tools which are not related to
% e-TeX but match the profile of this package.
\usepackage{etoolbox}


% use "autoref" the way I want
%   autoref is nice because the text or brackets of a ref are part of link
%   see http://tex.stackexchange.com/questions/36575/autorefs-inserted-text-has-not-the-correct-case
%       http://en.wikibooks.org/wiki/LaTeX/Labels_and_Cross-referencing
%       http://www.tug.org/applications/hyperref/manual.html#TBL-23

%% define autoref name for sections
% \ifx\sectionautorefname\defined
\def\sectionautorefname{\S\!\!}
\def\subsectionautorefname{\S\!\!}
\def\subsubsectionautorefname{\S\!\!}
% \fi
% from http://tex.stackexchange.com/questions/52410/how-to-use-the-command-autoref-to-implement-the-same-effect-when-use-the-comman
% \ifx\equationautorefname~#1\undefined
\def\equationautorefname~#1\null{%
  (#1)\null
}
% \fi

%% change ref of algorithm from 'algorithm x' to 'Procedure x'
\renewcommand*{\algorithmautorefname}{Procedure}
\renewcommand{\algorithmcfname}{Procedure}% Update algorithm name
\renewcommand{\algorithmcflinename}{Line}
\newcommand*{\subfigureautorefname}{Figure}


%% change alg settings
\setlength{\algomargin}{6mm}
\SetKwInput{Problem}{problem}
\SetKwInput{Input}{input}
\SetKwInput{Output}{output}
\SetAlgoSkip{smallskip} % default
\SetAlgoInsideSkip{smallskip} %
\setlength{\AlCapSkip}{1mm} 
\SetKwComment{tcp}{\#\ }{}
\SetKwComment{tcc}{\#\ }{}
% \SetAlFnt{\small}
% \SetAlCapFnt{\small}
% \SetAlCapNameFnt{\small}
% \SetAlCapHSkip{0pt}
% \IncMargin{-\parindent}
    
%% change theorem style
\usepackage{amsthm}
\newtheoremstyle{saber}% name
  {}%      Space above, empty = `usual value'
  {}%      Space below
  {\itshape}% Body font
  {}%         Indent amount (empty = no indent, \parindent = para indent)
  {\bfseries}% Thm head font
  {.}%        Punctuation after thm head
  {.5em}% Space after thm head: \newline = linebreak
  {}%         Thm head spec

\theoremstyle{saber}
%% definitions for theorem related environment and their autoref names
\ifcsundef{theorem}{% theorem is not defined yet
\newtheorem{theorem}{Theorem}%[section]
}{}
\ifcsundef{corollary}{%
\newtheorem{corollary}{Corollary}%[theorem]
}{}
\ifcsundef{lemma}{%
\newtheorem{lemma}{Lemma}%[theorem]
}{}
\ifcsundef{definition}{%
\newtheorem{definition}{Definition}%[theorem]
}{}
\ifcsundef{fact}{%
\newtheorem{fact}{Fact}%[theorem]
}{}
\ifcsundef{remark}{%
\newtheorem{remark}{Remark}%[theorem]
}{}
\ifcsundef{property}{%
\newtheorem{property}{Property}%[theorem]
}{}



%% change autoref names for theorem related
\ifx\theoremautorefname\undefined
\newcommand*{\theoremautorefname}{Theorem}
\fi
\ifx\lemmaautorefname\undefined
\newcommand*{\lemmaautorefname}{Lemma}
\fi
\ifx\definitionautorefname\undefined
\newcommand*{\definitionautorefname}{Definition}
\fi
\ifx\corollaryautorefname\undefined
\newcommand*{\corollaryautorefname}{Corollary}
\fi
\ifx\factautorefname\undefined
\newcommand*{\factautorefname}{Fact}
\fi
\ifx\propertyautorefname\undefined
\newcommand*{\propertyautorefname}{Property}
\fi


%% commonly used math commands
\ifx\argmax\undefined
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\fi
\ifx\argmin\undefined
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\fi
\ifx\limsup\undefined
\newcommand{\limsup}{\operatornamewithlimits{limsup}}
\fi
\ifx\liminf\undefined
\newcommand{\liminf}{\operatornamewithlimits{liminf}}
\fi
\ifx\norm\undefined
\newcommand{\norm}[1]{\lVert#1\rVert}
\fi
\ifx\abs\undefined
\newcommand{\abs}[1]{\lvert#1\rvert}
\fi
\ifx\set\undefined
\newcommand{\set}[1]{\left\{#1\right\}}
\fi
\ifx\mset\undefined
\newcommand{\mset}[1]{\lbrack #1\rbrack}
\fi
\ifx\etal\undefined
\newcommand{\etal}[1]{{\em #1 et al.}~}
\fi
\ifx\ie\undefined
\newcommand{\ie}{{\em i.e.,} }
\fi
\ifx\eg\undefined
\newcommand{\eg}{{\em e.g.,} }
\fi
\ifx\etc\undefined
\newcommand{\etc}{{\em etc.,} }
\fi
\ifx\wrt\undefined
\newcommand{\wrt}{{\em w.r.t.} }
\fi
\ifx\dotprod\undefined
\newcommand{\dotprod}[2]{
  \langle #1, #2 \rangle
}
\fi
\ifx\iid\undefined 
\newcommand{\iid}{i.i.d.}
\fi
\ifx\bigParenthes\undefined 
\newcommand{\bigParenthes}[1]{
  \big(#1\big)
}
\fi
\ifx\bigBracket\undefined 
\newcommand{\bigBracket}[1]{
  \big\{#1\big\}
}
\fi
\ifx\bigSqBracket\undefined 
\newcommand{\bigSqBracket}[1]{
  \big[#1\big]
}
\fi
\ifx\BigParenthes\undefined 
\newcommand{\BigParenthes}[1]{
  \Big(#1\Big)
}
\fi
\ifx\BigBracket\undefined 
\newcommand{\BigBracket}[1]{
  \Big\{#1\Big\}
}
\fi
\ifx\BigSqBracket\undefined 
\newcommand{\BigSqBracket}[1]{
  \Big[#1\Big]
}
\fi
\ifx\biggParenthes\undefined 
\newcommand{\biggParenthes}[1]{
  \bigg(#1\bigg)
}
\fi
\ifx\biggBracket\undefined 
\newcommand{\biggBracket}[1]{
  \bigg\{#1\bigg\}
}
\fi
\ifx\biggSqBracket\undefined 
\newcommand{\biggSqBracket}[1]{
  \bigg[#1\bigg]
}
\fi
\ifx\BiggParenthes\undefined 
\newcommand{\BiggParenthes}[1]{
  \Bigg(#1\Bigg)
}
\fi
\ifx\BiggBracket\undefined 
\newcommand{\BiggBracket}[1]{
  \Bigg\{#1\Bigg\}
}
\fi
\ifx\BiggSqBracket\undefined 
\newcommand{\BiggSqBracket}[1]{
  \Bigg[#1\Bigg]
}
\fi
\ifx\bracket\undefined
\newcommand{\bracket}[1]{
  \{#1\}
}
\fi
\ifx\parenthes\undefined
\newcommand{\parenthes}[1]{
  (#1)
}
\fi
\ifx\sqBracket\undefined
\newcommand{\sqBracket}[1]{
  [#1]
}
\fi
\ifx\prob\undefined 
\newcommand{\prob}[1]{\mathbb{P}[#1]}
\fi
\ifx\Prob\undefined 
\newcommand{\Prob}[1]{\mathbb{P}\big[#1\big]}
\fi
\ifx\probb\undefined 
\newcommand{\Probb}[1]{\mathbb{P}\bigg[#1\bigg]}
\fi
\ifx\expect\undefined 
\newcommand{\expect}[1]{\mathbb{E}[#1]}
\fi
\ifx\Expect\undefined 
\newcommand{\Expect}[1]{\mathbb{E}\big[#1\big]}
\fi
\ifx\expectt\undefined 
\newcommand{\expectt}[1]{\mathbb{E}\bigg[#1\bigg]}
\fi
\ifx\walk\undefined 
\makeatletter
\newcommand{\walk}[1]{%
  \@tempswafalse
  \@for\next:=#1\do
    {\if@tempswa\!\!\rightarrow\!\!\else\@tempswatrue\fi\next}%
}
\makeatother
\fi
\ifx\seq\undefined 
\newcommand{\seq}{\!=\!}
\fi
\ifx\sminus\undefined 
\newcommand{\sminus}{\!-\!}
\fi
\ifx\sm\undefined 
\newcommand{\sm}[1]{\!#1\!}
\fi

\ifx\union\undefined
\newcommand{\union}[2]{#1\!\cup\!#2}
\fi

\ifx\hl\undefined 
\newcommand{\hl}[2]{{\color{#1}#2}}
\fi

\ifx\hlb\undefined 
\newcommand{\hlb}[1]{{\color{blue}#1}}
\fi

\ifx\hlr\undefined 
\newcommand{\hlr}[1]{{\color{red}#1}}
\fi

\ifx\hlp\undefined 
\newcommand{\hlp}[1]{{\color{purple}#1}}
\fi

\ifx\hlc\undefined 
\newcommand{\hlc}[3]{{\color{#1}#2 [remark: #3]}}
\fi

%% reduce spacing
\setlength{\textfloatsep}{8.0pt plus 1.0pt minus 2.0pt}
%% Redefining itemize to save space
\ifcsdef{sitemize}{}{
\newenvironment{sitemize}{%
  \begin{list}{$\bullet$}{%
    %\setlength{\rightmargin}{\leftmargin}
    \setlength{\itemsep}{0.1cm}%
    \setlength{\leftmargin}{1.0em}%
    \setlength{\topsep}{0.1cm}%
    \setlength{\parsep}{0mm}}%
  }{\end{list}}
}

\ifcsdef{senumerate}{}{
\newenvironment{senumerate}{%
   \begin{list}{\arabic{enumi}.}{%
    \setlength\labelwidth{3.5em}%
    \setlength\leftmargin{2.5em}%
    \setlength{\topsep}{2pt plus 2pt minus 2pt}%
    \setlength\itemsep{0.0cm}%
    \usecounter{enumi}}%
  }{\end{list}}
}

\ifcsdef{spenumerate}{}{
\newenvironment{spenumerate}{%
   \begin{list}{(\arabic{enumi})}{%
    \setlength\labelwidth{3.5em}%
    \setlength\leftmargin{2.5em}%
    \setlength{\topsep}{2pt plus 2pt minus 2pt}%
    \setlength\itemsep{0.0cm}%
    \usecounter{enumi}}%
  }{\end{list}}
}

\ifcsdef{slenumerate}{}{
\newenvironment{slenumerate}{%
   \begin{list}{(\alph{enumi})}{%
    \setlength\labelwidth{3.5em}%
    \setlength\leftmargin{2.5em}%
    \setlength{\topsep}{2pt plus 2pt minus 2pt}%
    \setlength\itemsep{0.0cm}%
    \usecounter{enumi}}%
  }{\end{list}}
}



%% COPY from internet
%% This part goes in preamble
\newcommand{\dummyfig}[2]{
  \centering
  \fbox{
    \begin{minipage}[t][#1][t]{#2}
      \centering{Dummy figure}
    \end{minipage}
  }
}







==> libs/figure_confs.tex <==
\def \SerenaDemo {
    \input{figures/serena-demo-new}
}

\def \SerenaDemoSmall {
    \input{figures/serena-demo-new-small}
}

%% comparison for different serenade schemes
% \def \ComparisonSerenade   {\includegraphics[width=\fullup]{figures/v2/serenade_mean_delay_logy_new}}
%% remove hybrid
\def \ComparisonSerenade   {\includegraphics[width=\fullup]{figures/v2/serenade_woh_mean_delay_logy_new}}

==> sections/background.tex <==
\section{Background}\label{sec:backg}
% qpsr
In this section, we provide a brief introduction to the crossbar scheduling (switching) problem.
%Like the vast majority of other works in the switching
%literature~\cite{Anderson1993PIM,McKeownMekkittikulAnantharamEtAl1999,McKeown99iSLIP},
\begin{comment}
from serenade
\end{comment}
We assume that
all incoming
variable-length packets are segmented into fixed-length packets,
% (sometimes referred to as cells), 
which are then reassembled when \textcolor{green}{ before} leaving the switch.
Hence we consider the switching of only fixed-length packets in the sequel, and each
such fixed-length packet takes exactly one time slot to transmit.
% \modifiedHL{
We also assume that both the output ports and  
the crossbar operate at the same speed as the input ports. 
% }
Both assumptions above are widely adopted in the 
% Mekkittikul98stability,
literature~\cite{McKeownMekkittikulAnantharamEtAl1999,McKeown99iSLIP,GiacconePrabhakarShah2003SerenaJSAC,Gupta09Node}. 


%from serenade
%We assume that all incoming
%variable-size packets are segmented into fixed-size packets,
% (sometimes referred to as cells), 
%which are then reassembled when leaving the switch.
%Hence we consider the switching of only fixed-size packets in the sequel, and each
%such fixed-size packet takes exactly one time slot to transmit.
%\modifiedHL{
%We also assume that both the output ports and  
%the crossbar operate at the same speed as the input ports. 
%}
%Both assumptions above are widely adopted in the 
%literature~\cite {Mekkittikul98stability,McKeownMekkittikulAnantharamEtAl1999,McKeown99iSLIP,GiacconePrabhakarShah2003SerenaJSAC,Gupta09Node}. 
%\modifiedHL{
%Like in~\cite{GiacconePrabhakarShah2003SerenaJSAC}, we further assume that the arrival processes for those 
%fixed-size packets are {\it i.i.d.} Bernoulli. 
%}
\begin{comment}
from qps-r
\end{comment}
\subsection{Input-Queued Crossbar Switch}\label{subsec:sys-module}

%Almost all nowadays switches adopt an input-queued crossbar switch architecture.

In an $N\times N$ input-queued crossbar switch, 
% that
%interconnects $N$ input with $N$ output ports.
%is shown in~\autoref{fig:IQ}.
each input port has $N$ Virtual Output Queues
(VOQs)~\cite{Tamir_HighperformanceMulti_1988}.  The $j^{th}$ VOQ at input port $i$
% , denoted as VOQ$_{ij}$ in the sequel,
serves as a buffer for packets
going from input port $i$ to output port $j$. The use of VOQs solves the Head-of-Line
(HOL) blocking issue~\cite{Karol1987VOQHOL}, which
severely limits the throughput of the
switch system.


An $N\times N$ input-queued crossbar can be modeled as a weighted bipartite graph, of which the
two disjoint vertex sets are the $N$ input ports and the $N$ output ports
respectively.
% Note that we will use ``input/output port'' to stand for the
% vertices in the bipartite graph. For example, we will use ``input port i'' to represent the vertex
% corresponds to input port $i$ in the bipartite graph.
% The edges between those input ports and
% output ports are determined by the lengths of the respective VOQs.
In this bipartite graph, there is an
edge between input port $i$ and output port $j$, if and only if
% VOQ$_{ij}$,
the $j^{th}$ VOQ at input port $i$,
the corresponding VOQ,
is nonempty.  The weight of this edge is defined
as the length of ({\it i.e.,} the number of packets buffered at) this VOQ.
A set of such edges constitutes a {\it valid crossbar schedule}, or a {\it matching},
if any two of them do not share a common vertex. The weight of a matching
is the total weight of all the edges belonging to it ({\it i.e.,} the total length of all corresponding VOQs).

%serenade 

%An $N \!\times\! N$ input-queued crossbar switch is usually modeled as a weighted complete bipartite graph $G(I\bigcup O)$, with
%the $N$ input ports and the $N$ output ports represented as the two disjoint vertex sets $I \!=\! \{I_1, I_2, \dots, I_N\}$ and $O \!=\! \{O_1, O_2, \dots, O_N\}$ respectively.
% \existingHL{
%Each edge
%\footnote{Note that we use $(u, v)$ to represent a undirected edge, and $u\!\rightarrow\!v$ to represent a {\bf directed edge} throughout this paper.} 
% between two vertexes $(I_i, O_j)$
%$(I_i, O_j)$ corresponds to the $j^{th}$ VOQ at input port $i$ and its weight is defined as the number of packets in the VOQ. 
% }
% \addedHL{
%We denote this edge also as $I_i\!\rightarrow\!O_j$ when its direction is emphasized. 
% \modifiedHL{
% Unless otherwise stated, we shall follow the notational convention used in~\cite{Wilson1996GT} 
% for graph-related notations ({\it e.g.,} vertex sets and walks) throughout this paper. 
% }
% }
%(\ie the queue length of VOQ).
%(for $1 \!\le\! i,j \!\le\! N$)

%A valid schedule, or
%\textit{matching}, is a set of edges between $I$ and $O$
%n which no two distinct edges share a vertex.
%The weight of a matching is defined as the total weight of all edges belonging to the matching.
%A vertex is called {\bf matched} if it is an endpoint of an edge in the matching.
% its corresponding input/output port is called as {\bf matched}.  
%therwise the port is {\bf unmatched}. 
%We say that a matching is {\it full} if all vertices in $G(I\bigcup O)$ are an endpoint of an edge in the matching, and is {\it partial} otherwise.
%Clearly, in an $N \!\times\! N$ switch, any full matching contains exactly $N$ edges.  
\subsection{Batch Switching Algorithms}

Since SB-QPS is a batch switching algorithm~\cite{Aggarwal2003EdgeColoring,Neely2007FrameBased,Wang2018ParallelEdgeColoring}, 
we provide some background on it here.
Unlike in a regular switching algorithm, where a matching decision is computed for every time slot, 
in a batch switching algorithm, multiple (say $T$) consecutive time slots are grouped as
a batch and these $T$ matching decisions are batch-computed.  



\begin{wrapfigure}{R}{0.3\textwidth}
	\centering
	\includegraphics[width=0.295\textwidth]{figures/IQ-sched-graph/scheduling-graph-standalone}
	\caption{The joint calendar.}\label{fig:sched-graph}
\end{wrapfigure}

As shown in~\autoref{fig:sched-graph}, the joint calendar (schedule) of the $N$ output ports over a batch of $T$ time slots can be viewed as a $T \times N$ table with $TN$ cells in it.
Each column corresponds to the calendar of an output port and each row a time slot.  
The content of the cell at the $t^{th}$ row and $j^{th}$ column is the input port that $O_j$ is to pair with with during time slot $t$.  
For example, in~\autoref{fig:sched-graph}, output port $O_1$ is paired with $I_3$ in time slot $1$, $I_5$ in time slot $2$, and $I_N$
in time slot $T$.
At each input port, 
all packets that were in queue before a cutoff time (for the current batch), including those that belong to either the current batch, or a previous batch but could not be served then,
are waiting to be inserted into the respective calendars (i.e., columns of cells) of the corresponding output ports.  
In a batch switching algorithm, the goal, 
is to pack as many such packets across the $N$ input ports as possible into the $TN$ cells in this joint calendar.  
Note that the total number of such packets can exceed $TN$, in which case at most $TN$ of them can be served in this batch.   

Most of the existing batch switching algorithms are centralized.  In such algorithms, the switch controller packs this joint calendar for all input and output ports.  
%How to pack this joint calendar can be precisely modeled as a graph-algorithmic problem called edge-coloring. 
\textbf{For example, }an optimal way (generally not unique) of packing the joint calendar can be solved using Birkhoff von Neumann Decomposition (BvND)~\cite{vonNeumann53TwoPerson}, as was 
done in the batch switching algorithm proposed in~\cite{Neely2007FrameBased}, with $O(N^{1.5}T)$ complexity per time slot.
%note that in this particular application (of batch switching), in which the bipartite multigraph (that the crossbar is modeled as) to be edge-colored 
%often either already is or is populated (by adding
%artificial edges to it) into a regular bipartite multigraph (in which every vertex has the same degree), an optimal ({\it i.e.}, using minimum number of colors) edge-coloring
%roughly corresponds to a BvND, and vice versa.  
%%% By Long: here O(N^{1.5}T) should be O(N^{1.5}T^2) and O(N^{1.5}) should be O(N^{2.5})
%However, the computational complexities of BvND-based batching switching algorithms are quite high:  for example $O(N^{1.5}T^2)$ per batch or $O(N^{1.5}T)$ per time slot in~\cite{Neely2007FrameBased} 
%where the classical maximum matching algorithm~\cite{HopcroftKarp1973MSM} is
%used to find each of the $T$ matchings in the BvND;  
Although 
using~\cite{Goel2010PerfectMacthing} or the edge-coloring algorithm proposed in~\cite{cole2001edge} instead of BvND can reduce this asymptotic time complexity slightly, it is not clear whether that
can reduce the execution time.  Furthermore, most of these centralized algorithms cannot be effectively parallelized to reduce their computational complexities per port.  
%Later in \autoref{sec-related}, we will provide a brief survey of batching switching algorithms.

In this paper, we present two switching algorithms, both using small batches of constant size $T$ and having low complexity $O(\log T)$ per time slot. Specifically, in the second algorithm, SW-QPS, we propose a new batch switching framework called Sliding Window Switching, which is compared with Batch Switching in Figure \ref{fig:batch-vs-sw}.
 
\begin{figure}[ht]
	\centering
	\includegraphics[width=0.295\textwidth]{figures/drafts/batch-vs-sw.jpg}
	\caption{Comparison of Batch Switching with Sliding Window Switching.}\label{fig:batch-vs-sw}
\end{figure}

As in the left side of Figure \ref{fig:batch-vs-sw}, each batch in Batch Switching contains $T$ consecutive time slots and different batches do not overlap. The scheduler packs incoming packets into Batch 1 during the period $t+1$ to $t+T$. At time slot $t+T$, all $T$ matchings in Batch 1 become ready for switching and the scheduler moves to Batch 2. 

In Sliding Window Switching, however, consecutive batches overlap on $T-1$ time slots. At time slot $t+1$, the first time slot of the Batch 1 becomes ready for switching and leaves the batch. All other time slots then join Batch 2, together with a new empty time slot appended to the end of Batch 2.

In contrast to Batch Switching, Sliding Window Switching allows new packets to directly jump to the first time slot of the joint calendar and to be switched immediately, without having to wait for the beginning of next batch, as long as there are enough empty positions in the joint calendar. This flexible behavior, having one matching ready at each time slot, is crucial to the reduction of batching delay to a $O(1)$ order under low traffic loads. Meanwhile, Sliding Window Switching is simple to implement and preserves the advantage of of Batch Switching: achieving high throughput with low complexity. 
 

==> sections/evaluation.tex <==
\section{Evaluation}\label{sec:eva}

In this section, we evaluate, through simulations, the performance of
SB-QPS and SW-QPS under various load conditions and traffic patterns.
We compare its \st{delay} performance with
that of iSLIP~\cite{McKeown99iSLIP}, a refined and optimized representative parallel maximal matching
algorithm (adapted for switching).  The \st{delay} performance of the \st{ideal (but computationally
expensive) algorithm} MWM (Maximum Weighted Matching) is also included in the
comparison as a benchmark.  
\textbf{We might need to compare with state-of-art works.}
 Our simulations show bla..bla..
\subsection{Simulation Setup}
\label{subsec: sim-setting}

In our simulations, we fix the number of input/output ports, $N$ to $64$.
%, and the findings are reported
%in \autoref{subsec: delay-vs-port}.
To measure throughput and delay accurately, we assume each VOQ has an infinite
buffer size and hence there is no packet drop at any input port.
Each simulation run is guided by the following stopping
rule~\cite{Flegal2010MCStopRule,Glynn1992MCStopRule}:   The number of time slots simulated is the larger between $500N^2$ and
that is needed
for the difference between the estimated and the actual average delays to be within $0.01$ time slots
with probability at least $0.98$.



% Let $\hat{\sigma}_k$
% be the empirical standard deviation of the average delay up to the $k^{th}$
% time slot, $T^*$ be the minimum simulation effort ({\it i.e.,} number of
% time slots to be simulated), and $\delta$ be the desired half-width of the
% confidence interval. The
% simulation terminates the first time when the following condition holds
% \[
% A\frac{\hat{\sigma}_T}{T} + \delta I_{T\leq T^*} + \frac{1}{T} < \delta.
% \]
% Here $A$ is a Student's t quantile, $T$ is
% number of time slots to be simulated, and
% $I_{T\leq T^*}$ is an indicator, which equals
% $1$ if $T\leq T^*$, otherwise $0$. In all our simulations, we set $A\!=\!2.326$
% ({\it i.e.,} $98\%$ for two-sided when the degree of freedom is $\infty$),
% $T^*\!=\!500N^2$, and $\delta=0.01$.

We assume in our simulations that
each traffic arrival matrix $A(t)$ is Bernoulli {\it i.i.d.} with its traffic
rate matrix $\Lambda$ being equal to the product of the offered load $\rho$ and a traffic pattern
matrix (defined next). Similar Bernoulli arrivals were studied in  ~\cite{GiacconePrabhakarShah2003SERENA,McKeown99iSLIP,Gong2017QPS}.
% that the traffic arrival processes to different input ports are mutually independent, and each
% such arrival process is {\it i.i.d.}~Bernoulli (\ie at any given input port,
% a packet arrives with a constant probability $\rho \in (0,1)$ during each time slot).
\hlb{Note that only synthetic traffic (instead of that derived from packet traces) is used in our simulations
because, to the best of our knowledge, there is no meaningful way to combine
packet traces into switch-wide traffic workloads.}
The following four standard types of normalized (with each row or column sum equal to $1$) traffic patterns are used:
%for generating the switch's workloads:
% (I) \emph{Uniform}, (II) \emph{Quasi-diagonal},
% (III) \emph{Log-diagonal}, and (IV) \emph{Diagonal}. For detailed definitions
% of these traffic patterns, please refer to~\cite{GiacconePrabhakarShah2003SERENA,Gong2017QPS}.
% \begin{comment}
(I) \emph{Uniform}: packets arriving at any input port go
to each output port with probability $\frac{1}{N}$.
(II) \emph{Quasi-diagonal}: packets arriving at input port $i$ go to
output port $j \!=\! i$ with probability $\frac{1}{2}$ and go to any other output port
with probability $\frac{1}{2(N-1)}$.
(III) \emph{Log-diagonal}: packets arriving at input port $i$ go
to output port $j = i$ with probability $\frac{2^{(N-1)}}{2^N - 1}$ and
go to any other output port $j$ with probability equal $\frac{1}{2}$ of the
probability of output port $j - 1$ (note: output port $0$ equals output port $N$).
(IV) \emph{Diagonal}: packets arriving at input port $i$ go to
output port $j \!=\! i$ with probability $\frac{2}{3}$, or go to output port
$(i\, \text{mod} \, N) + 1$ with probability $\frac{1}{3}$.
These traffic patterns are listed in order of how skewed the volumes of traffic arrivals to different output
ports are: from uniform being the least skewed, to diagonal being the most skewed.

==> sections/intro-longlong.tex <==
\section{Introduction}\label{sec:intro}
% % [Long: faster traffic, large network]
The volume of network traffic across the Internet and in data-centers continues to grow relentlessly,
thanks to existing and emerging data-intensive applications, such as big data analytics, cloud computing,
and video streaming.  At the same time, the number of network-connected devices is exploding,
fueled by the wide adoption of 
%mobile hand-held devices
smart phones and the emergence of the Internet of things.
To transport and ``direct" such massive traffic volume to such a diverse range of destinations, 
switches and routers that are capable of 
connecting a large number of ports (called {\it high-radix} switching \cite{Cakir2015HighRadix, Cakir2016HighRadixCrossbar}) and operating at very high line rates are badly needed. However, the growing line rates and the number of ports are making it increasingly challenging to design the switching algorithm, whose functionality is to generate the crossbar schedule by solving the following matching problem.

% \subsection{Matching Problem}\label{subsec:mp}
\subsection{Matching Problem and Prior Work}\label{subsec:mp}
% % [Long: difficult]
% Most present day switching systems in Internet routers and
% data-center switches employ an input-queued crossbar switch to interconnect the $N$ input ports with the $N$ output ports. 

Many present day switching systems in Internet routers and
data-center switches employ an input-queued crossbar to interconnect their input ports and output ports. In an $N\times N$ input-queued crossbar switch, for each switching cycle or time slot, each input port can only connect to at most one output port and vice versa. In other words, the the connection patterns between input and output ports ({\it i.e.}, the crossbar schedule) is a one-to-one matching. In order to achieve high throughput and low delay performances, the switching algorithm has to generate ``high quality'' matchings, which have high cardinality and low VOQ starvation, as fast as one matching per time slot. 

Unfortunately, it appears to be hard to achieve both high matching quality and low computation complexity as required by high-link-rate high-radix switches. On one hand, Maximum Weighted Matchings (MWM) can achieve 100\% switch throughput and near-optimal queueing delays for various traffic patterns~\cite{McKeownMekkittikulAnantharamEtAl1999}, but each MWM takes $O(N^{2.5}\log W)$ time to compute using the state-of-the-art algorithm~\cite{Duan2012BpMWMScaling}, where
$W$ is the maximum possible length of a VOQ. \textbf{This complexity is too high to scale to high-radix switches.} On the other hand, a family of distributed switching algorithms, called parallel iterative algorithms, have lower computational complexity but worse throughput. A well-known example is iSLIP~\cite{McKeown99iSLIP}, which has $O(\log^2 N)$ per-port computational complexity but cannot attain 100\% throughput except under uniform traffic. Besides, even with hardware optimization, iSLIP has a high communication complexity of $O(N)$ per port in return for its low computational complexity.

Another recent example of parallel iterative algorithms, called QPS-r \cite{Gong_QPSr_2019}, generates each matching with $r$ iterations, each of which consists of two phases: proposing and accepting. In the proposing phase, each input port independently sends a proposal to at most one output port, and then in the accepting phase, each output port independently accepts the received proposals. When multiple proposals are sent to a single output port, at most one proposal can be accepted, and the only accepted proposal will never be changed or canceled. QPS-r has the lowest possible asymptotic complexity of $O(1)$ per port, but in return, it cannot achieve 100\% throughput.  

\begin{figure}[h]
	\centering
	\includegraphics[width=0.455\textwidth]{figures/IQ-sched-graph/scheduling-graph-standalone}
	\caption{A sample joint calendar of port number $N=8$ and batch size $T$: Cells with ``--" are unmatched.}\label{fig:sched-graph}
\end{figure}

Most of the switching algorithms \cite{Anderson1993PIM, McKeown99iSLIP, GiacconePrabhakarShah2003SERENA, AtallaCudaGiacconeEtAl2013BPAssist, Hu2018HRF}, including MWM, iSLIP, and QPS-r, are ``regular" (cycle-by-cycle) algorithms that produce each matching individually in each cycle (time slot), whereas an alternative approach called batch switching \cite{bianco2002frame, rojas2007frame, Aggarwal2003EdgeColoring, Neely2007FrameBased, Wang2018ParallelEdgeColoring, Bianco2004BatchSched} groups multiple (say $T$) consecutive time slots as a batch. Such a batch of matchings, called a {\it joint calendar}, as illustrated in \autoref{fig:sched-graph} as a $T \times N$ table with $TN$ cells, is computed collectively throughout the $T$-time-slot duration of this batch. Each row of the joint calendar, which is a matching for the corresponding time slot, can be packed with packets not only in the corresponding time slot as in regular switching, but in any of the $T$ time slots within the current batch. Therefore, batch switching algorithms can achieve higher throughput than their regular switching counterparts for various traffic patterns ~\cite{bianco2002frame, rojas2007frame}.

However, compared with regular switching algorithms, batch switching algorithms suffer from an additional batching delay of $O(T)$: A packet arriving at the beginning of a batch has to wait till at least the beginning of the next batch to be switched. This $O(T)$ delay is a pronounced issue especially in the following two cases. Firstly, it is unnecessary when the traffic load is low, because in this case even regular switching algorithms can easily achieve packet delay as low as $O(1)$. Secondly, it is unacceptably high in many existing switching algorithms that use a large batch size $T$ to attain high throughputs ({\it e.g.} in ~\cite{Aggarwal2003EdgeColoring}, batch size $T$ is as large as $\omega(N^2)$ ).

In summary, even with the batch switching framework available, designing efficient switching algorithms that achieve excellent throughput and delay performances yet have low computation complexities remains to be a challenging problem.

\subsection{Our Work}\label{subsec:our-work}
To address the aforementioned challenges, we combine parallel iterative algorithms with batch switching algorithms for the advantages of both frameworks: low per-port complexity and high throughput. To achieve this combination, we adopt a \textcolor{green}{novel} accepting strategy, which will be described in \autoref{subsec:sb-qps}. Furthermore, because of the greediness of our accepting strategy, we can break the boundary of batches and propose a new framework called Sliding Window (SW) switching, which solves the batching delay issue of batch switching algorithms.

The result of our study is the following two algorithms: Small-Batch QPS (SB-QPS) and Sliding-Window QPS (SW-QPS), corresponding to the batch switching and SW switching frameworks. The term QPS (short for Queue-Proportional Sampling) refers to an add-on matching technique that is proposed in~\cite{Gong2017QPS} and later extended to a standalone ``regular" parallel iterative matching algorithm called QPS-r~\cite{Gong_QPSr_2019}, whose proposing phase (to be described in in~\autoref{subsec:qps}) is used in both of our algorithms because it has low complexity and delivers high throughput. In fact, besides QPS, both of our algorithms are compatible with any parallel iterative switching algorithm with greedy packing schemes.

Our first algorithm, SB-QPS, has two features over previous works. The first feature is that it is fully distributed with low complexity. Most of the existing batch switching algorithms \cite{Aggarwal2003EdgeColoring, Neely2007FrameBased, Wang2018ParallelEdgeColoring} model the process to pack the joint calendar as an edge-coloring problem, but until now, all practical solutions to the latter problem are centralized and have high complexity. In contrast, SB-QPS is a fully distributed parallel iterative algorithm that resembles QPS-r, having a much lower $O(1)$ computation complexity per port per time slot, in contrast to the Birkhoff von Neumann Decomposition (BvND)-based algorithm in \cite{Neely2007FrameBased} that has $O(N^{1.5}T)$ complexity per time slot.

The second feature of SB-QPS is that it reduces batching delay without sacrificing too much throughput. As we have mentioned above, batching delay is proportional to batch size, but larger batch sizes, associated with more chances to refine the joint calendar, are essential for the high throughput performances of previous batching algorithms. Because of the high efficiency of the QPS proposing scheme and our greedy accepting scheme, SB-QPS only requires a small number of refinements to achieve at least 87\% throughput under all four traffic patterns, reducing its batch size to a small number $T$ that is independent to $N$. Therefore, it has significantly low batching delay compared with the algorithm in \cite{Aggarwal2003EdgeColoring}, whose batch size is $\omega(N^2)$.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.295\textwidth]{figures//IQ-sched-graph/sliding-schedule}
	\caption{An illustration of the joint calendar of Sliding Window switching: The label of each row (matching) is its time slot of completion.}\label{fig:batch-vs-sw}
\end{figure}

Our second algorithm, SW-QPS, is based on a new switching framework called \emph{Sliding Window (SW) switching}, which aims for overcoming the batching delay issue of batch switching algorithms. In the sliding window framework, at arbitrary time slot $t$, the scheduler also refines a joint calendar of $T$ matchings as in batch switching, shown as the bold frame in \autoref{fig:batch-vs-sw}. However, unlike batch switching, these $T$ matchings are not finalized all together at the end of this batch but at different time slots ranging from $t$ to $t+T-1$, one matching per time slot. 

We use the following analogy to illustrate the evolution of the joint calendar in a sliding window algorithm. An $N\times N$ crossbar switch can be viewed as a school with $N$ teachers (input ports) and $N$ departments (output ports), and the row (matching) that is finalized at time slot $t$ is referred to as Class $t$. Each cell (entry with fixed time slot and output port in the joint calendar) is a student, who needs to finish one course required by his corresponding department to receive a degree. Such a course may be taught by any teacher, but one teacher can only teach one student one course at each time slot. 

In the setting above, at an arbitrary time slot $t$, the joint calendar contains students of $T$ different grades from Class $t$ to Class $t+T-1$, shown as the bold frame in \autoref{fig:batch-vs-sw}. Students of Class $t$ are enrolled at the beginning of time slot $t-T+1$, when the joint calendar covers Class $t-T+1$ to Class $t$ (the first three rows of \autoref{fig:batch-vs-sw}), and have $T$ time slots to take the degree course before graduating at the end of time slot $t$. After the graduation of Class $t$, the joint calendar moves one time slot downwards to cover Classes $t+1$ to $t+T$ (the last four rows of \autoref{fig:batch-vs-sw}). 

As is mentioned above, a desirable switching algorithm achieves both high throughput and low delay. In order for high throughput, it maximizes the ratio of granted input requests, which is equivalent to matching many student as possible for courses given the teachers' schedules, and in order for low delay, it minimizes the waiting time from granting to switching, which is the time interval for a student from taking a degree course to graduation. Sliding window switching addresses both objectives by giving each teacher $T$ classes of students as candidates for the courses and giving priority to senior students who will graduate soon to take these courses. Therefore, it gets the better of both worlds:  
low packet delay comparable to regular switching and high throughput comparable to batch switching.

SW-QPS is a fully distributed iterative algorithm, which is an adaptation of SB-QPS to sliding window switching with same operations in the two phases of each time slot. As in \autoref{sec:eva},it achieves 87\% throughput under diagonal traffic, and over 90\% throughput under other three traffic patterns with only $O(1)$ computational complexity per port per time slot. It also has excellent delay performance that is close to that of MWM when the traffic load is under $0.8$. In comparison, iSLIP~\cite{McKeown99iSLIP}, a well-known parallel iterative regular switching algorithm, can only attain roughly $80\%$ throughput under the $4$ standard traffic patterns except the uniform traffic and as mentioned earlier, it has a computational complexity of $O(\log^2 N)$ per port and a communication complexity of $O(N)$ per port. 

% \textbf{Our contributions}

The rest of this paper is organized as follows. In \autoref{sec:backg}, we provide some
background on the input-queued crossbar switches, batch switching and sliding-window \textcolor{green}{SW} switching.  
In \autoref{sec:schemes},  we first review
QPS, and then we describe our schemes: SB-QPS and SW-QPS. 
Then we evaluate the performance of our schemes in~\autoref{sec:eva}. 
In~\autoref{sec:related}, we survey
related work before concluding this paper in~\autoref{sec:con}.

==> sections/intro.BK.tex <==
\section{Introduction}\label{sec:intro}
\begin{comment}
	from qps-r
\end{comment}
The volume of network traffic across the Internet and in data-centers continues to grow relentlessly,
thanks to existing and emerging data-intensive applications, such as big data analytics, cloud computing,
and video streaming.  At the same time, the number of network-connected devices is exploding,
fueled by the wide adoption of
%mobile hand-held devices
smart phones and the emergence of the Internet of things.
To transport and ``direct" this massive amount of traffic to their respective destinations,
%At the same time, the number of Internet-connected devices continues to,
switches and routers capable of
connecting a large number of ports (called {\it high-radix}~\cite{Cakir2015HighRadix,Cakir2016HighRadixCrossbar}) and operating
at very high line rates are badly needed.

% Most present day switching systems in Internet routers and
% data-center switches employ an input-queued crossbar switch to interconnect the $N$ input ports with the $N$ output ports.
Many present day switching systems in Internet routers and
data-center switches employ an input-queued crossbar to interconnect their input ports and output ports
({\it e.g.,} Cisco Nexus 5000 Series~\cite{cisco_nexus_5000_2017}, Arista 7500 Switch~\cite{arista_7500_2018},
and Juniper QFX 10000 Switches~\cite{juniper_qfx10000_2018}).
%{Note in this work, we only consider the switching systems that employ a single-stage crossbar, or a monolithic crossbar, as the scheduler
%for such a crossbar can have full visibility of the entire system thus can make better scheduling decisions~\cite{cisco_nexus_5000_2017}.
Though it was commonly believed that such a (monolithic) crossbar is difficult to scale beyond 64 (input/output) ports, recent advances in switching hardware
technologies ({\it e.g.,}~\cite{Passas2010HighRadix,Passas2012bHighRadix,Cakir2015HighRadix})
have made high-radix crossbars not only
technologically feasible but also
economically and environmentally ({\it i.e.}, more energy-efficient) favorable, as compared to low-radix crossbars.



\begin{comment}
from serenade
\end{comment}
\subsection{Matching Problem}

% the $N$ input ports with the $N$ output ports.
In an $N\times N$ input-queued crossbar switch, each input port can be connected to only one output
port and vice versa in each switching cycle or time slot.
Hence, in every time slot, the switch needs to compute
a one-to-one \textit{matching} between input and output ports ({\it i.e.}, the crossbar schedule).
A major research challenge
of designing high-link-rate high-radix
switches ({\it e.g.}, 128 ports or beyond of 40 Gbps each)
is to develop algorithms that can
compute ``high quality'' matchings -- {\it i.e.} those that result in
high switch throughput and low queueing
delays for packets -- in a few nanoseconds.
% For example, with a fixed packet (cell) length of 64 bytes (used in the crossbar of Cisco 12000 Series Internet
% Routers~\cite{ciscoCellSize}), a switch supporting 40 Gbps per-port rates has to compute a matching
% every 12.8  nanoseconds.
For example, with a cell\footnote{It is common practice in switches/routers to slice incoming
	packets into cells of a fixed size or a range of variable sizes~\cite[Chapter 2, Page 21]{aweya_switch_router_2018}.
	For example, Juniper QFX 10000 switch~\cite{juniper_qfx10000_2018} uses cell sizes varying
	between 96 and 176 bytes, and Huawei NE40E switch~\cite{huawei_ne40e_2018} uses
	a fixed cell size.} size of 64 bytes (the minimum cell size used in Arista 7500 Switch~\cite{arista_7500_2018}),
a switch supporting 40 Gbps per-port rates has to compute a matching
every 12.8  nanoseconds.
%(with speedup of $1$)

\begin{comment}
Due to the physical limitations of crossbars, each input port in an
input-queued switch can only connect with a single output port during each
switching cycle, \ie time slot, and vice versa. Therefore, the input-queued
switch has to determine at each time slot the one-to-one connection, or
one-to-one matching between the input ports and output ports. This makes the
switch scheduling problem, in which we need to design algorithms to produce
``good-quality'' matchings resulting in good throughput and low delays. The
switch scheduling problem is the primary research challenge in designing
large high-speed single-crossbar switches.
\end{comment}

Unfortunately, there appears to be a tradeoff
between the quality of a matching and the amount of 
time needed to compute it (\ie time complexity). 
% \modifiedHL{
% \modifiedHL{
For example, %when used for crossbar scheduling, 
using Maximum Weighted Matchings (MWM) as crossbar schedules
%, with a suitable weight measure,
is known to result in 100\% switch throughput and
near-optimal
%Tassiulas90Max,
queueing delays for various traffic patterns~\cite{McKeownMekkittikulAnantharamEtAl1999}, but
%For a switch with $N$ input/output ports, however,
each MWM takes $O(N^{2.5}\log W)$ time to compute using the state-of-the-art algorithm~\cite{Duan2012BpMWMScaling}, where
$W$ is the maximum possible length of a VOQ. 


\begin{comment}
%% [MWM is great, but too expensive]
The switch scheduling problem can be transformed into a matching problem for an
$N\times N$ weighted bipartite graph. Maximum Weight Matching (MWM), with
well-chosen quantities as weight for edges, is known to produce great
matchings which can achieve $100\%$ throughput and empirically optimal
delays for various traffic patterns~\cite
{McKeownMekkittikulAnantharamEtAl1999,ShahWischik2006MWM0}.
However, it takes $O(N^3)$ time to compute a matching in MWM~\cite
{EdmondsKarp1972}. Parallelized variants exist, some of them still need $O
(N^2)$ work at each input/output port~\cite
{BayatiShahSharma2008MWMMaxProduct}, some achieves sublinear but either
assumes
a concurrent-read concurrent-write parallel random access machine,
which is too complex to implement in hardware, or
requires $O(N^3)$ processing elements~\cite{Fayyazi2004pMWM} which is too
expensive to be adopted in switches. This reality motivates a lot of
researchers to pursuit practical switch scheduling algorithms with much lower
time complexity, but still has performance close to MWM.
%



Another example is iSLIP~\cite{McKeown99iSLIP},
a distributed iterative algorithm where input and
output ports compute a matching in parallel through
multiple iterations of message exchanges.  iSLIP has
a per-port computational complexity of $O(\log^2 N)$ ($O(\log N)$
iterations that each has $O(\log N)$ circuit depth) that is lower than Serena's overall complexity of $O(N)$.
%by using $2N$ identical hardware modules running in parallel.
However, iSLIP computes a different type of matching called a Maximum-Size Matching (MSM), which is of
lower quality than MWM.  Hence iSLIP cannot achieve 100\% throughput
except on uniform traffic, and has much longer
queueing delays than Serena on nonuniform traffic
patterns under heavy traffic loads.

\end{comment}

While considerable research has been performed on crossbar scheduling algorithms 
for decades, these algorithms~\cite{Anderson1993PIM,McKeown1995iLQF,Tassiulas1998TASS,Mekkittikul98stability,McKeownMekkittikulAnantharamEtAl1999,McKeown99iSLIP,Goudreau00Shakeup,ShahGiacconePrabhakar2002SerenaMicro,Giaccone2002Apsara,GiacconePrabhakarShah2003SerenaJSAC,Aggarwal2003EdgeColoring,Keslassy2003MSM,ZhangBhuyan2003iDRR,Fayyazi04ParallelMWM,ShahWischik2006MWM0,BayatiPrabhakarShahEtAl2007Iterative,Neely2007FrameBased,Gupta09Node,Ye10Variable,AtallaCudaGiacconeEtAl2013BPAssist,Wang2018ParallelEdgeColoring,Hu2018HRF} are not suitable 
for future high-speed large input-queued switches, since what was 
considered high-speed ({\it e.g.,} $1$ Gbps per port) and large ({\it e.g.,} 
$64$ ports) is pale in comparison with the type of speed ({\it e.g.,} $1$ Tbps per 
port) and large ({\it e.g.,} $1,000$ ports) we are aiming for today~\cite{DeCusatis2014FutureSwitch,Kim2005RouterDevTrand}, yet 
our expectation of delay and throughput performance are only going to become 
higher. \textcolor{green}{future is what we are aiming for today. Our expectation future is far beyond imagination.} For example, the two well-known among these algorithms are SERENA~\cite{ShahGiacconePrabhakar2002SerenaMicro,GiacconePrabhakarShah2003SerenaJSAC} and 
iSLIP~\cite{McKeown99iSLIP}, but neither is suitable for 
high-speed input-queued switches with $\textcolor{green}{a}$ large number of ports. On one hand, although SERENA 
can achieve 100\% throughput and has excellent delay performance close to 
that of MWM, its computational 
complexity for generating a matching is $O(N)$, which is too high for high-speed 
switches when $N$ is large. On the other hand, 
iSLIP only requires $O(\log N)$ 
iterations to compute a matching, but it can only guarantee to achieve at least 
$50\%$ throughput~\cite{Dai00Speedup} and it suffers from poor delay performance under heavy nonuniform 
traffic~\cite{GiacconePrabhakarShah2003SerenaJSAC}.

%% [SERENA is a very good approximation with O(N) complexity, without
% explaining the details of the algorithm, say
% that O(N) is still too expensive for large N so SERENA is not widely
% adopted]
\deletedHL{
Researchers have been searching for crossbar scheduling algorithms that have time complexity much lower
than $O(N^3)$, but performance
close to MWM. 
Some researchers have developed parallel or distributed MWM algorithms\cite{Fayyazi04ParallelMWM,Fayyazi2006ParaMWM,BayatiPrabhakarShahEtAl2007Iterative,BayatiShahSharma2008MWMMaxProduct} that, by 
distributing the computational cost across multiple processors (nodes), bring down 
the per-node computational complexity. However, these algorithms either require too many 
processors ~\cite{Fayyazi04ParallelMWM,Fayyazi2006ParaMWM} or have very high per-node computational complexity 
~\cite{BayatiPrabhakarShahEtAl2007Iterative,BayatiShahSharma2008MWMMaxProduct}, which are impractical to implement in today's IQ switches. 

Some researchers have proposed algorithms based on maximum 
cardinality matching or maximal matching, 
such as PIM~\cite{Anderson1993PIM} and iSLIP~\cite{McKeown99iSLIP}. 
Those types of matchings can be computed with lower computational complexity, they 
however have lower qualities than MWM: They can not achieve 100\% switch throughput and 
usually have much higher delays than MWM under non-uniform traffic. 

Some researchers have proposed  
low-complexity randomized algorithms~\cite{Tassiulas1998TASS,ShahGiacconePrabhakar2002SerenaMicro,GiacconePrabhakarShah2003SerenaJSAC,Ye10Variable}. 
Tassiulas~\cite{Tassiulas1998TASS} proposed the so-called ``pick-and-compare'' algorithm, which can achieve $100\%$ switch 
throughput with linear complexity but has very bad delay performance. Inspired by 
Tassiulas' work, 
% researchers have developed a few low-complexity algorithms which 
% can achieve $100\%$ switch throughput and have good delay performance. 
% So far, the best 
% known among them is 
Giaccone, Prabhakar, and Shah proposed 
SERENA~\cite{ShahGiacconePrabhakar2002SerenaMicro,GiacconePrabhakarShah2003SerenaJSAC}.
SERENA produces excellent matching decisions that result in $100\%$ switch throughput
and queueing delay close to that of MWM.
However, it is a centralized algorithm with $O(N)$ time complexity.  When $N$ is large,
this complexity is too high to support very high link rates.  Hence, as stated 
in~\cite{ShahGiacconePrabhakar2002SerenaMicro,GiacconePrabhakarShah2003SerenaJSAC},
SERENA is designed for high-aggregate-rate switches -- \ie those that have either a large number of ports 
%(but with relatively low line rates per port) 
or a
very high line rate per port -- but not for those that have both. } % end addedHL
%(but with a small number of ports)
%;  it is not suitable for switches that have both.
%However, its $O(N)$ time complexity is still too high for
%large $N$, which limits its wide adoptions in large input-queued switches.
\deletedHL{
While parallelizing the SERENA algorithm seems to be an obvious solution to this scalability problem,
we will show in \autoref{subsec: merge} that a key procedure in SERENA, namely MERGE,
is monolithic in nature, making SERENA hard to parallelize.}

\deletedHL{
Besides the above algorithms which make a matching decision per each time slot, some 
researchers have proposed another type of crossbar scheduling -- frame-based 
scheduling~\cite{Aggarwal2003EdgeColoring,Neely2007FrameBased,Wang2018ParallelEdgeColoring}. In frame-based scheduling, consecutive time slots are grouped 
into frames and the matching decisions are made on a per-frame basis. Since a frame 
typically spans many time slots ({\it e.g.,} $O(\log N)$), and a packet arriving at 
the beginning of a frame has to wait till the end of the frame, frame-based 
scheduling typically results in higher queueing delays.      
}
% \glong{To the best of our knowledge, no parallelization of SERENA, has been
% proposed in the literature.}
%
%parallelized variants which
%achieves sublinear work at each input/output port do not exist.
%
%rounds of
%
\subsection{Our Work}
\textbf{Our contributions}

The rest of this paper is organized as follows. In \autoref{sec:background}, we provide some
background on the input-queued crossbar switches.  In \autoref{sec:scheme},  we first review
QPS, and then describe QPS-r. Then in~\autoref{sec:throughput-and-delay-analysis}, we derive the throughput and
the queue length (and delay) bounds of QPS-r, followed by the
performance evaluation in~\autoref{sec:evaluation}. In~\autoref{sec: related-work}, we survey
related work before concluding this paper in~\autoref{sec:conclusion}.

==> sections/intro.tex <==
\section{Introduction}\label{sec:intro}
% % [Long: faster traffic, large network]
The volume of network traffic across the Internet and in data-centers continues to grow relentlessly,
thanks to existing and emerging data-intensive applications, such as big data analytics, cloud computing,
and video streaming.  At the same time, the number of network-connected devices is exploding,
fueled by the wide adoption of 
%mobile hand-held devices
smart phones and the emergence of the Internet of things.
To transport and ``direct" this massive amount of traffic to their respective destinations,
%At the same time, the number of Internet-connected devices continues to,
switches and routers capable of 
connecting a large number of ports (called {\it high-radix}~\cite{Cakir2015HighRadix,Cakir2016HighRadixCrossbar}) and operating
at very high line rates are badly needed. Motivated by this rapidly growing need, much research has been devoted to, and significant breakthroughs
made, on the hardware designs for fast high-radix switching fabrics recently ({\it e.g.},~\cite{Cakir2016HighRadixCrossbar,Dai2017HighRadix}). Indeed,
these recent breakthroughs have made fast high-radix switching hardware not only technologically feasible
but also economically and environmentally (more energy-efficient) favorable, as compared to low-radix
switching hardware~\cite{Cakir2016HighRadixCrossbar}. 

% \subsection{Matching Problem}\label{subsec:mp}
\subsection{Matching Problem and Prior Work}\label{subsec:mp}
% % [Long: difficult]
% Most present day switching systems in Internet routers and
% data-center switches employ an input-queued crossbar switch to interconnect the $N$ input ports with the $N$ output ports. 
Many present day switching systems in Internet routers and
data-center switches employ an input-queued crossbar to interconnect their input ports and output ports. 
\begin{comment}
({\it e.g.,} Cisco Nexus 5000 Series~\cite{cisco_nexus_5000_2017}, Arista 7500 Switch~\cite{arista_7500_2018},
and Juniper QFX 10000 Switches~\cite{juniper_qfx10000_2018}).
%{Note in this work, we only consider the switching systems that employ a single-stage crossbar, or a monolithic crossbar, as the scheduler
%for such a crossbar can have full visibility of the entire system thus can make better scheduling decisions~\cite{cisco_nexus_5000_2017}.
Though it was commonly believed that such a (monolithic) crossbar is difficult to scale beyond 64 (input/output) ports, recent advances in switching hardware
technologies ({\it e.g.,}~\cite{Passas2010HighRadix,Passas2012bHighRadix,Cakir2015HighRadix})
have made high-radix crossbars not only
technologically feasible but also
economically and environmentally ({\it i.e.}, more energy-efficient) favorable, as compared to low-radix crossbars. 
\end{comment}
In an $N\times N$ input-queued crossbar switch, each input port can be connected to only one output
port and vice versa in each switching cycle or time slot.
Hence, in every time slot, the switch needs to compute
a one-to-one \textit{matching} between input and output ports ({\it i.e.}, the crossbar schedule).
A major research challenge
of designing high-link-rate high-radix
switches ({\it e.g.}, 128 ports or beyond of 40 Gbps each)
is to develop (switching) algorithms that can
compute ``high quality'' matchings -- {\it i.e.} those that result in
high switch throughput and low queueing
delays for packets -- in a few nanoseconds.
% For example, with a fixed packet (cell) length of 64 bytes (used in the crossbar of Cisco 12000 Series Internet
% Routers~\cite{ciscoCellSize}), a switch supporting 40 Gbps per-port rates has to compute a matching
% every 12.8  nanoseconds.
\begin{comment}
For example, with a cell\footnote{It is common practice in switches/routers to slice incoming
	packets into cells of a fixed size or a range of variable sizes~\cite[Chapter 2, Page 21]{aweya_switch_router_2018}.
	For example, Juniper QFX 10000 switch~\cite{juniper_qfx10000_2018} uses cell sizes varying
	between 96 and 176 bytes, and Huawei NE40E switch~\cite{huawei_ne40e_2018} uses
	a fixed cell size.} size of 64 bytes (the minimum cell size used in Arista 7500 Switch~\cite{arista_7500_2018}),
a switch supporting 40 Gbps per-port rates has to compute a matching
every 12.8  nanoseconds.
%(with speedup of $1$)
\end{comment}
\begin{comment}
Due to the physical limitations of crossbars, each input port in an
input-queued switch can only connect with a single output port during each
switching cycle, \ie time slot, and vice versa. Therefore, the input-queued
switch has to determine at each time slot the one-to-one connection, or
one-to-one matching between the input ports and output ports. This makes the
switch scheduling problem, in which we need to design algorithms to produce
``good-quality'' matchings resulting in good throughput and low delays. The
switch scheduling problem is the primary research challenge in designing
large high-speed single-crossbar switches.
\end{comment}

\begin{comment}
Unfortunately, there appears to be a tradeoff
between the quality of a matching and the amount of 
time needed to compute it (\ie time complexity). 
% \modifiedHL{
% \modifiedHL{
For example, %when used for crossbar scheduling, 
using Maximum Weighted Matchings (MWM) as crossbar schedules
%, with a suitable weight measure,
is known to result in 100\% switch throughput and
near-optimal
%Tassiulas90Max,
queueing delays for various traffic patterns~\cite{McKeownMekkittikulAnantharamEtAl1999}, but
%For a switch with $N$ input/output ports, however,
each MWM takes $O(N^{2.5}\log W)$ time to compute using the state-of-the-art algorithm~\cite{Duan2012BpMWMScaling}, where
$W$ is the maximum possible length of a VOQ. 
\end{comment}

\begin{comment}
%% [MWM is great, but too expensive]
The switch scheduling problem can be transformed into a matching problem for an
$N\times N$ weighted bipartite graph. Maximum Weight Matching (MWM), with
well-chosen quantities as weight for edges, is known to produce great
matchings which can achieve $100\%$ throughput and empirically optimal
delays for various traffic patterns~\cite
{McKeownMekkittikulAnantharamEtAl1999,ShahWischik2006MWM0}.
However, it takes $O(N^3)$ time to compute a matching in MWM~\cite
{EdmondsKarp1972}. Parallelized variants exist, some of them still need $O
(N^2)$ work at each input/output port~\cite
{BayatiShahSharma2008MWMMaxProduct}, some achieves sublinear but either
assumes
a concurrent-read concurrent-write parallel random access machine,
which is too complex to implement in hardware, or
requires $O(N^3)$ processing elements~\cite{Fayyazi2004pMWM} which is too
expensive to be adopted in switches. This reality motivates a lot of
researchers to pursuit practical switch scheduling algorithms with much lower
time complexity, but still has performance close to MWM.
%



Another example is iSLIP~\cite{McKeown99iSLIP},
a distributed iterative algorithm where input and
output ports compute a matching in parallel through
multiple iterations of message exchanges.  iSLIP has
a per-port computational complexity of $O(\log^2 N)$ ($O(\log N)$
iterations that each has $O(\log N)$ circuit depth) that is lower than Serena's overall complexity of $O(N)$.
%by using $2N$ identical hardware modules running in parallel.
However, iSLIP computes a different type of matching called a Maximum-Size Matching (MSM), which is of
lower quality than MWM.  Hence iSLIP cannot achieve 100\% throughput
except on uniform traffic, and has much longer
queueing delays than Serena on nonuniform traffic
patterns under heavy traffic loads.

\end{comment}
Unfortunately, there appears to be a tradeoff
between the quality of a matching and the amount of 
time needed to compute it (\ie time complexity). 
For example, %when used for crossbar scheduling, 
using Maximum Weighted Matchings (MWM) as crossbar schedules
%, with a suitable weight measure,
is known to result in 100\% switch throughput and
near-optimal 
queueing delays for various traffic patterns~\cite{McKeownMekkittikulAnantharamEtAl1999}, but
%For a switch with $N$ input/output ports, however,
each MWM takes $O(N^{2.5}\log W)$ time to compute using the state-of-the-art algorithm~\cite{Duan2012BpMWMScaling}, where
$W$ is the maximum possible length of a VOQ.  
While considerable research has been performed on switching algorithms 
% ~\cite{Anderson1993PIM,McKeown1995iLQF,Tassiulas1998TASS,Mekkittikul98stability,McKeownMekkittikulAnantharamEtAl1999,McKeown99iSLIP,Goudreau00Shakeup,ShahGiacconePrabhakar2002SerenaMicro,Giaccone2002Apsara,GiacconePrabhakarShah2003SERENA,Aggarwal2003EdgeColoring,Keslassy2003MSM,ZhangBhuyan2003iDRR,Fayyazi04ParallelMWM,ShahWischik2006MWM0,BayatiPrabhakarShahEtAl2007Iterative,Neely2007FrameBased,Gupta09Node,Ye10Variable,AtallaCudaGiacconeEtAl2013BPAssist,Wang2018ParallelEdgeColoring,Hu2018HRF} 
% % references are too many, only select some of them
for decades, these algorithms~\cite{Anderson1993PIM,McKeown99iSLIP,GiacconePrabhakarShah2003SERENA,AtallaCudaGiacconeEtAl2013BPAssist,Hu2018HRF} are not suitable 
for future high-speed large input-queued switches, since what was 
considered high-speed ({\it e.g.,} $1$ Gbps per port) and large ({\it e.g.,} 
$64$ ports) is pale in comparison with the type of speed ({\it e.g.,} $1$ Tbps per 
port) and large ({\it e.g.,} $1,000$ ports) we are aiming for today~\cite{DeCusatis2014FutureSwitch,Kim2005RouterDevTrand}, yet 
our expectation of delay and throughput performance are only going to become 
higher. 
% % Jingfan's comments
\lbrack\textcolor{green}{JM: can we simplify this sentence a little?}\rbrack  
For example, the two well-known among these algorithms are SERENA~\cite{GiacconePrabhakarShah2003SERENA} and 
iSLIP~\cite{McKeown99iSLIP} \textcolor{green}{[seems strange]}, but neither is suitable for 
% % Long: changed a large number of ports to "high-radix" as we have already defined it 
% %  with a large number of ports --> high-radix 
high-radix high-speed input-queued switches. On one hand, although SERENA 
can achieve 100\% throughput and 
% has excellent delay performance close to that of MWM, 
has reasonably good delay performance, 
% its computational 
% complexity for generating a matching is $O(N)$, which is too high for high-speed 
% switches when $N$ is large. 
it is a centralized algorithm with $O(N)$ computational 
complexity for generating a matching, which is too high for high-speed 
switches when $N$ is large. On the other hand, 
iSLIP is a parallel (more precisely distributed iterative) algorithm and has 
a lower per-port computational complexity of $O(\log^2 N)$ using $N$ processors (one at each port), 
but iSLIP cannot attain 100\% throughput 
except under uniform traffic. 
% iSLIP, a well-known parallel iterative algorithm, only requires $O(\log N)$ 
% iterations to compute a matching, but it can only guarantee to achieve at least 
% $50\%$ throughput~\cite{Dai00Speedup} and it suffers from poor delay performance under heavy nonuniform 
% traffic~\cite{GiacconePrabhakarShah2003SERENA}. 
% % Long: added communication complexity
Besides, iSLIP with a distributed implementation \textcolor{green}{[since the $O(\log^2 N)$ complexity is distributed, shall we move ``distributed" to the sentence above?]}has a high communication complexity of $O(N)$ per 
port, which makes it difficult to scale to switches with a large number of ports.  


% \subsection{SW-QPS}\label{subsec:sw-qps}

% % [Long: Alternative approach]
% In this work, we adopt an alternative approach -- batch 
% switching~\cite{Aggarwal2003EdgeColoring,Neely2007FrameBased,Wang2018ParallelEdgeColoring}. 
Besides the aforementioned regular switching algorithms ({\it e.g.,} iSLIP and SERENA), 
an alternative type of switching algorithms is batch-based. 
Unlike in a regular switching algorithm, where a matching decision is computed for every time slot, 
in a batch switching algorithm ({\it e.g.,} \cite{bianco2002frame,rojas2007frame,Aggarwal2003EdgeColoring,Neely2007FrameBased,Wang2018ParallelEdgeColoring,Bianco2004BatchSched}), multiple (say $T$) consecutive time slots are grouped 
as a batch and the $T$ matching decisions are batch-computed.  
Since the batch-computation of these $T$ matchings 
often has lower time complexity than 
$T$ independent matching computations, the amortized 
(over the $T$ time slots) time complexity of a batch switching
algorithm is often lower than that of a regular switching algorithm. 
Batch switching algorithms are also shown to have better throughput 
performance (than their regular switching counterparts) for various traffic patterns~\cite{bianco2002frame,rojas2007frame} %especially for non-uniform traffic 
when the batch size $T$ is well-chosen. 
% % may need to move
{\bf Long: Here, the logic flow is not good enough! Let's figure out a better one} 
It is %however \textcolor{green}{[however? why big batch is desirable?]} 
desirable for this batch size $T$ to be small because batch switching  
algorithm has a batching delay of $O(T)$: 
A packet arriving at the beginning of a batch has to wait till 
at least the beginning of the next batch to be switched. 
% 
% However, most of the existing batch switching algorithms 
% are centralized and cannot be effectively parallelized to reduce their computational complexities per port. 
However, to attain high throughputs, all existing batch switching algorithms have to either 
use a large batch size ({\it e.g.,} $O(N^2)$ 
in~\cite{Aggarwal2003EdgeColoring}) which leads to high batching delay, or still 
% ,Li2008BatchSched,Bianco2002BatchSched,Bianco2004BatchSched
incur a high computational complexity~\cite{Neely2007FrameBased,Bianco2004BatchSched}) even after the amortization.
{\bf Move (the following sentence) to related work section} 
Although a parallel batch switching algorithm recently 
proposed in~\cite{Wang2018ParallelEdgeColoring} 
has a computational complexity of $O(\log N)$ per time slot per port, it requires a large $T$: A batch size of $\num{3096}$ 
was needed for $N \!=\! 300$ as reported in~\cite{Wang2018ParallelEdgeColoring}.

Therefore, it remains a challenging problem for designing efficient switching algorithms that 
have low computational complexities, yet have excellent throughput and delay performances. 

\subsection{Our Work}\label{subsec:our-work}

% In this work, we aim at designing efficient parallel batch switching 
% algorithms that requires a small batch size and has low computational complexities per port, 
% yet they can attain very high throughputs and have excellent delay performances. 
In this work, we first propose Small-Batch QPS (SB-QPS), a batch 
switching algorithm that uses a small constant batch size
$T$ that is independent of $N$. 
Here QPS stands for Queue-Proportional Sampling, an add-on technique
proposed in~\cite{Gong2017QPS} that we will describe in~\autoref{subsec:qps}.  
Although QPS can also work as a stand-alone algorithm, we found that \textcolor{green}{no we found that} its throughput is only around 
$63\%$ under uniform traffic when running for a single iteration, and this throughput grows 
very slowly with the number of iterations. Benefiting from the advantages of batching, SB-QPS has much better throughput performance. \textbf{The throughput performance of SB-QPS is much better, benefiting from batching.}

However, SB-QPS has worse delay performances when the traffic is light because it suffers 
from the batching delay issue, the inherent disadvantage of all batching algorithms. 
\textbf{However, as with all batching algorithms, SB-QPS suffers from an inherent batching delay, which is negligible under heavy traffic loads, but is significant under light traffic loads.}
% % [TODO: emphasize BS usually has higher throughput]
% % [batching delay is a disadvantage when traffic load is light]
This batching delay is negligible when the traffic load is heavy, however, it dominates 
the packet delay when the traffic load is light. To overcome this disadvantage, 
we propose a new ``batch switching approach'' 
called Sliding-Window (SW) switching. Unlike 
in a batch switching algorithm, where $T$ matchings are produced at once \textcolor{green}{all together} per batch, in a 
SW switching algorithm, $T$ matchings for $T$ consecutive time slots 
(say time slot $t$ to $t\!+\!T\!-\!1$) are maintained and refined at each time slot and the 
matching for the earliest time slot ({\it i.e.,} time slot $t$) is finalized and 
used to switch packets for time slot $t$. \textbf{and at each time slot, one of these matchings becomes ready for switching.}
 Therefore, it gets the better of both worlds:  
Its delay performance is comparable to that of regular switching 
algorithms under light traffic (or in other words, it does not suffer from 
the batching delay issue) and similar to that of batch 
switching algorithms under moderate and heavy traffic, 
yet its throughput performance is similar to  
that of batch switching algorithm. \textbf{It achieves the high throughput performance and low amortized complexity that are comparable to batch switching algorithms, without paying the batching delay.}

Building upon SW switching, %and the recent switching work Queue-Proportional Sampling (QPS)~\cite{Gong2017QPS}, 
we then propose SW-QPS, a sliding-window \textcolor{green}{SW} switching algorithm that has 
a per-port computational complexity of $O(1)$ \textcolor{green}{$O(1)$ computational complexity per port}. %and a per-port communication complexity of $O(T)$. 
% Since in SW-QPS, $T$ is a small constant independent of $N$, SW-QPS has the lowest possible 
% (asymptotic) computational and communication complexity: $O(1)$ per port. 
Yet, SW-QPS has excellent 
throughput and delay performances. As we will \textcolor{green}{no will} show in~\autoref{sec:eva}, SW-QPS achieves at least $90\%$ 
throughput (except for the diagonal traffic, under which the throughput is slightly lower than $90\%$) and delay performance close to that of MWM when the 
traffic load is not extremely high (say $<0.8?$) under all $4$ standard traffic patterns (to be described in~\autoref{sec:eva}). In comparison, iSLIP~\cite{McKeown99iSLIP}, a well-known parallel iterative regular switching algorithm, can only attain roughly $80\%$ throughput under the $4$ standard traffic patterns except 
the uniform traffic and as mentioned earlier, it has a computational complexity of $O(\log^2 N)$ per port 
and a communication complexity of $O(N)$ per port. 

% \textbf{Our contributions}

The rest of this paper is organized as follows. In \autoref{sec:backg}, we provide some
background on the input-queued crossbar switches, batch switching and sliding-window \textcolor{green}{SW} switching.  
In \autoref{sec:schemes},  we first review
QPS, and then we describe our schemes: SB-QPS and SW-QPS. 
Then we evaluate the performance of our schemes in~\autoref{sec:eva}. 
In~\autoref{sec:related}, we survey
related work before concluding this paper in~\autoref{sec:con}.

==> sections/marks.tex <==
\newpage
\textcolor{green}{\section{Marks}}
\begin{enumerate}
	\item: To change the tables and figures from QPS-3 to QPS-1, use comp\_qps1 and burst60\_qps1.
	use burst80\_wo for high load bursty without QPS-r.
\end{enumerate}


==> sections/scheme-long.tex <==
\section{Schemes}\label{sec:schemes}

% In this section, we describe our two batch switching algorithms in this work. Both of them use the proposal strategy as in a recent switching algorithm called Queue Proportional Sampling (QPS)~\cite{Gong2017QPS}, to be described in~\autoref{subsec:qps}. Then, we describe in detail in~\autoref{subsec:sb-qps} our first scheme, Small-Batch QPS (SB-QPS), which is a batch switching 
% algorithm. Finally, we describe in~\autoref{subsec:sw-qps} our second scheme, Sliding-Window QPS (SW-QPS), which is a SW switching algorithm.  

In this section, we describe the two proposed switching algorithms, namely SB-QPS (\autoref{subsec:sb-qps}) and SW-QPS (\autoref{subsec:sw-qps}). As mentioned earlier, both of them build upon QPS-r~\cite{qpsr}, more precisely, adopt the 
Queue Proportional Sampling (QPS) proposing strategy that is used in QPS-r. 
\begin{comment}
How many "proposals" do you want to use?
JM: most simple ... that was proposed in ~\cite{Gong2017QPS}
more specific ... Both of them use the proposal strategy from a recent switching algorithm called Queue Proportional Sampling (QPS)~\cite{Gong2017QPS}
\end{comment}
Hence, we describe the QPS proposing strategy first in~\autoref{subsec:qps}. 
% Then, we 
% describe in detail in~\autoref{subsec:sb-qps} our first scheme call Small-Batch QPS (SB-QPS), which is a traditional batch switching 
% algorithm. Finally, we describe in~\autoref{subsec:sw-qps} our second scheme, Sliding-Window QPS (SW-QPS), which is a SW switching algorithm.  

\begin{figure}
\centering
\includegraphics[width=0.80\columnwidth]{figures/IQ-sched-graph/scheduling-graph-standalone}
\caption{A joint calendar. ``--" means unmatched.}\label{fig:sched-graph}
\Description{A joint calendar for batch switching algorithms.}
\end{figure}
\subsection{Batch Switching Framework}\label{subsec:back-batching}
As mentioned earlier in~\autoref{subsec:ours},  in a batch switching algorithm, multiple (say $T$) consecutive 
time slots are grouped as a batch and these $T$ matching decisions are batch-computed. 
As shown in~\autoref{fig:sched-graph}, the joint calendar (schedule) of the $N$ output ports over a batch of $T$ time slots can be viewed as a $T \times N$ table with $TN$ cells in it.
Each column corresponds to the calendar of an output port and each row a time slot.  
The content of the cell at the $t^{th}$ row and $j^{th}$ column is the input port that $O_j$ is paired with during time slot $t$. 
For example, in~\autoref{fig:sched-graph}, output port $O_1$ is paired with $I_3$ in time slot $1$, $I_5$ in time slot $2$, and is unmatched 
in time slot $T$.
At each input port, 
all packets that were in queue before a cutoff time (for the current batch), including those that belong to either the current batch, 
or previous batches but could not be served then,
are waiting to be inserted into the respective calendars ({\it i.e.,} columns of cells) of the corresponding output ports.  
In a batch switching algorithm, the goal, 
is to pack as many such packets across the $N$ input ports as possible into the $TN$ cells in this joint calendar.  
Note that the total number of such packets can exceed $TN$, in which case at most $TN$ of them can be served in this batch.   

% \subsection{Queue Proportional Sampling (QPS)}\label{subsec:qps}
\subsection{QPS Proposing Strategy}\label{subsec:qps}
% \textcolor{green}{[We need to specify for the proposing strategy, QPS-r is the same as QPS, (and the difference of our algorithms is only in the proposal format). We directly describe our accepting strategy in 4.2, so we do not describe QPS accepting strategy here.]}
To explain QPS proposing strategy, we need first explain QPS-r, the first standalone switching algorithm that uses it. 
During each time slot, QPS-r simply runs $r$ iterations of 
QPS that is originally proposed in~\cite{Gong2017QPS} as an ``add-on'' technique to augment other switching algorithms. 
QPS computes a starter matching, which is then populated ({\it i.e.}, adding more edges to it) and refined, 
by other switching algorithms such as iSLIP~\cite{McKeown99iSLIP} and SERENA~\cite{GiacconePrabhakarShah2003SERENA}, 
into a final matching. 
To generate such a starter matching, QPS runs only one iteration that consists of two phases: a proposing phase and an accepting phase. 
Since both SB-QPS and SW-QPS use, with slight modifications that will be elaborated next, the QPS proposing strategy, %that was first proposed and used in the proposing phase in QPS, 
here we restate it for this paper to be self-contained. 
% that generates a starter matching, which is then populated ({\it i.e.}, adding more edges to it) into a final matching by other switching algorithms such as iSLIP~\cite{McKeown99iSLIP} and SERENA~\cite{GiacconePrabhakarShah2003SERENA} (such QPS-augmented algorithms are called QPS-iSLIP and QPS-SERENA, respectively). To generate such a starter matching, QPS runs only one iteration that consists of two phases: a proposing phase and an accepting phase. The proposing phase is used by both of our algorithms, but the accepting phase needs significant changes to be adapted to the frameworks of batch and SW switching. Therefore, we only describe the QPS proposing phase below, and postpone the description of our accepting strategy to \autoref{subsec:sb-qps}.

In the QPS proposing strategy, each input port, unless it has no packet to transmit, proposes to {\it exactly one} output port, which is decided by the QPS strategy. Here, we will only describe the operations at input port $1$;  those at any other input port are identical. Like in~\cite{Gong2017QPS}, we denote by $m_1,m_2, \cdots, m_N$ the respective queue lengths of the $N$ VOQs at input port $1$, and by $m$ their sum ({\it i.e.}, $m \!\triangleq\!\sum_{k=1}^N m_k$). At first, input port 1 simply samples an output port $j$ with probability $\frac{m_j}{m}$, {\it i.e.,} proportional to $m_j$, the length of the corresponding VOQ; it then sends a proposal to output port $j$, attaching the value $m_j$, which will be used in the accepting phase. The computational complexity of this QPS operation, carried out on a simple data structure that is proposed in~\cite{Gong2017QPS}, is $O(1)$ per input port.   

% In the QPS proposing phase, each input port, unless it has no packet to transmit, proposes to {\it exactly one} output port, which is decided by the QPS strategy. Here, we will only describe the operations at input port $1$;  those at any other input port are identical. Like in~\cite{Gong2017QPS}, we denote by $m_1,m_2, \cdots, m_N$ the respective queue lengths of the $N$ VOQs at input port $1$, and by $m$ their sum ({\it i.e.}, $m \!\triangleq\!\sum_{k=1}^N m_k$). At first, input port 1 simply samples an output port $j$ with probability $\frac{m_j}{m}$, {\it i.e.,} proportional to $m_j$, the length of the corresponding VOQ; it then sends a proposal to output port $j$, attaching the value $m_j$, which will be used in the accepting phase. The computational complexity of this QPS operation, carried out on a simple data structure that is proposed in~\cite{Gong2017QPS}, is $O(1)$ per input port.   

% QPS and its extensions have achieved good throughput and delay performances, but they do not achieve a perfect balance between matching quality and computation complexity. For example, QPS-SERENA achieves 100\% throughput and delay performance close to that of MWM, but it is a centralized algorithm with relatively high complexity ({\it i.e.,} $O(N)$), which prevents its applications in large high-speed switches. On the contrary, QPS-r, an extension of QPS proposed in \cite{Gong_QPSr_2019}, is a standalone parallel iterative switching algorithm that achieves the lowest possible computational complexity of $O(1)$ per port but can only attain roughly 63\% throughput in the first iteration under the uniform traffic. Although its throughput can be boosted by running multiple iterations, approximately 9 rounds are needed to achieve 90\% throughput under uniform traffic, which is also unaffordable in high-speed switches.

\subsection{Small-Batch QPS (SB-QPS)} \label{subsec:sb-qps}

% To better balance matching quality with computation complexity, we combine QPS with the batch switching framework, resulting in our first algorithm: SB-QPS. SB-QPS is a parallel iterative algorithm under the batch switching framework:  The input and output ports run a small constant number of QPS-like iterations to collaboratively pack the joint calendar. Each iteration consists of two phases, namely, a proposing phase and an accepting phase. In the proposing phase, input ports independently request for cells in the joint calendar, while in the accepting phase, output ports independently accept or reject the requests. The computational complexity of SB-QPS is $O(1)$ per port per time slot and its communication complexity is between {\bf \lbrack 2 and 3  ??\rbrack} bytes per port per time slot on average.  

% SB-QPS is a batch switching algorithm that uses a small constant batch size $T$ that is independent of $N$.
SB-QPS is a batch switching algorithm with a batch size of $T$ that is a small constant independent of $N$.
% Like QPS-r~\cite{qpsr},
Unlike most existing batch switching algorithms ({\it e.g.,}~\cite{Aggarwal2003EdgeColoring,Neely2007FrameBased}) that 
are centralized, SB-QPS is a parallel iterative algorithm: 
% \textcolor{green}{[To say it is parallel, different ports are independent in each phase. To say it is iterative, de we need to compare with regular algorithms?]} 
The input and output ports run 
$T$ QPS-like iterations (one per time slot) in a batch to collaboratively pack the joint calendar. 
Like in other batch switching algorithms, in SB-QPS, 
the final joint calendar (packed with these $T$ iterations), or in other words, the final $T$ matchings, are then 
used to transmit packets, and meanwhile a new joint calendar will be packed with another 
$T$ iterations,  in the next batch. 
% \textcolor{green}{[This part should belong to batch switching framework, not SB-QPS. It is confusing (what is batch, iteration, phase...) here.]} 
% The operation of each iteration is simple: Input ports request for cells in the joint calendar, 
% and output ports accept or reject the requests.  
% As we will show later in this section, in SB-QPS, the computational complexity of this calendar packing 
% is $O(1)$ per port per time slot. 
% and its communication complexity is between {\bf \lbrack 2 and 3  ??\rbrack} bytes per port per time slot on average.  
% Like in QPS~\cite{Gong2017QPS}, 
Each iteration of SB-QPS, like that of QPS-r described in~\autoref{subsec:qps}, 
consists of two phases: a proposing phase and an accepting phase.

\smallskip
% \noindent
% {\bf Proposing phase.} In this phase, every input port, unless all VOQs are empty, 
% proposes to a single output port in the QPS manner ({\it i.e.,} following the QPS proposing strategy). In the proposal, besides the length of the corresponding VOQ as in the original QPS, the input port also specifies its availability calendar during this batch, which is encoded as a $T$-bit bitmap $B_I[1..T]$, where $B_I[t]=1$ if this input port is available, in other words, unmatched, at the $t^{th}$ time slot in this batch; Otherwise, $B[t]=0$. 
% \smallskip
\noindent
{\bf The Proposing Phase.} 
In this phase, every input port $i$ proposes to a single output port using the QPS proposing strategy unless all VOQs 
are empty at this input port. Unlike in QPS-r where a proposal attaches only the value $m_j$ (the length of 
the corresponding VOQ), in SB-QPS, this proposal also attaches the availability of input port $i$. 

This availability information is encoded as a $T$-bit-long bitmap $B[1..T]$, where $B[t]\!=\!1$ if input port $i$ is available, 
or in other words, unmatched, at the $t^{th}$ time slot in this batch; otherwise, $B[t]\!=\!0$. 
This bitmap of each (input or output) port is initialized to all-$1$ ({\it i.e.,} all time slots in this batch are available) 
at the beginning of a batch, 
and then updated in each of the $T$ iterations, at the corresponding port. 
Since, as mentioned earlier, the batch size $T$ in SB-QPS is a small constant 
(say $T$=16) so that a $T$-bit-long bitmap can 
be fit into a single CPU word. As a result, all bitmap operations, such as bitwise-AND and find first set (ffs), that are involved in 
SB-QPS can be accomplished in one or a few CPU cycles, and thus have a computational complexity of $O(1)$.  
% In this phase, every input port, unless all VOQs are empty, 
% proposes to a single output port in the QPS manner ({\it i.e.,} following the QPS proposing strategy). In the proposal, besides the length of the corresponding VOQ as in the original QPS, the input port also specifies its availability calendar during this batch, which is encoded as a $T$-bit bitmap $B_I[1..T]$, where $B_I[t]=1$ if this input port is available, in other words, unmatched, at the $t^{th}$ time slot in this batch; Otherwise, $B[t]=0$. 

\begin{algorithm}[t]
\DontPrintSemicolon 
\SetKwProg{Proc}{Procedure}{}{}
\caption{Accepting phase at output port $1$.}
\label{alg:accept}

% \Proc{Accept()}{


    $B_O\leftarrow$ availability bitmap of output port\; \label{accept:o-availability}

    $\mathcal{P}\leftarrow$ proposals in descending order of VOQ lengths\; \label{accept:sort}

 	\ForEach{proposal $p\in \mathcal{P}$} {

 	    $i\leftarrow$ input port that sends $p$\;\label{accept:i-in}

 		$B_I\leftarrow$ availability bitmap from $p$\; \label{accept:i-availability}

 		$B\leftarrow B_O \land B_I$\; \label{accept:c-availability}

 		$k\leftarrow $ find the earliest available time slot in $B$\; \label{accept:f-availability}

 		\If{found}{

 			Accept $p$ and send $k$ to input port $i$\; \label{accept:ac-availability}

 			Update the availability bitmap $B_O$\; \label{accept:up-availability}

 			Update the calendar (of output port 1)\; \label{accept:up-jc}
 		}
 	}
            

    % }
\end{algorithm}

\smallskip
\noindent
{\bf The Accepting Phase.} The accepting phase at every output port is very different from that in QPS-r. 
The latter only allows at most one proposal to be accepted, whereas the former allows an output port to
accept multiple (up to $T$)  proposals. In this phase, we adopt the simple {\it First Fit Accepting} (FFA) strategy. 
The pseudocode of the FFA strategy at output port 1 is 
shown in~\autoref{alg:accept}; that at any other output port is identical. 
As shown in~\autoref{alg:accept}, when output port 1 receives one or more proposals, 
it first sorts, with ties being broken arbitrarily, these proposals in a descending order of their corresponding VOQ lengths (\autoref{accept:sort})
and then tries to accommodate them one after another in the following manner.   
First, it gets the availability bitmap $B_I$ of the corresponding input port (input port $i$) 
that sends the proposal $p$ (\autoref{accept:i-availability}). 
Then, it compares $B_I$ with its own availability bitmap $B_O$, more precisely, it 
computes their bitwise-AND bitmap $B$ (\autoref{accept:c-availability}).  
Finally, it finds the earliest time slot during which both are available (\autoref{accept:f-availability}), {\it i.e.,} 
the position of the first `$1$' (also referred to as the first set bit) in bitmap $B$. 
If such a time slot $k$ exists, 
it accepts this proposal and sends a message attached with the value $k$ to notify input 
port $i$ (\autoref{accept:ac-availability}) so 
that input port $i$ will update its availability bitmap, more precisely, 
set the $k^{th}$ bit of its availability bitmap $B_I$ to $0$ ({\it i.e.,} unavailable). 
It then updates its own availability bitmap $B_O$ similarly~(\autoref{accept:up-availability}) and 
its own calendar (schedule)~(\autoref{accept:up-jc}). 
The computational complexity for this ``first fit'' accepting strategy at an output port is 
$O(1)$ on average and can be made $O(1)$ even in the worst case using the same technique as used in~\cite{Gong2017QPS}. 

% {\bf Em joint calendar \& batch }
% \smallskip
% \noindent
% {\bf Accepting Phase.} The accepting phase at every output port differentiates from the Longest VOQ First (LVF) strategy in QPS-r in that an output port can accept more than one proposals in each iteration. As illustrated in \autoref{alg:accept}, if an output port receives only one proposal, it accommodates that proposal in the following steps. At first, it gets the availability bitmap $B_I$ of the corresponding input port from the proposal (\autoref{accept:i-availability}). Then, it compares $B_I$ with its own availability $B_O$, which has the same format as $B_I$, (\autoref{accept:c-availability}) and finds the earliest time slot during which both ports are available (\autoref{accept:f-availability}). If such a time slot $k$ exists, it updates its own availability bitmap $B_O[k]\gets 1$ and sends an acceptance message to remind the corresponding input port of updating its availability $B_I[k]\gets 1$ (\autoref{accept:ac-availability} and \autoref{accept:up-availability}). If an input port receives multiple proposals, it first sorts these proposals in non-increasing order of their corresponding VOQ lengths and then accommodates them one by one in the steps above. 

% \smallskip
% \noindent
% {\bf Computational Complexity.}   
% Although the operations at Lines \ref{accept:c-availability} and~\ref{accept:f-availability} in~\autoref{alg:accept} 
% appear to have a computational complexity of $O(T)$, each of them can be accomplished using a single CPU instruction within 
% one CPU cycle when $T$ is small and thus each $T$-bit-long bitmap can fit in a single CPU word. Since, as mentioned earlier, 
% $T$ in SB-QPS is a small constant (say $T$=16),  
% % This claim is based on the following observation: Both bitmaps $B_I$ and $B_O$ fit in one CPU word because their lengths equal to batch size $T$, which is a small constant independent of $N$(a typical value of $T$ is $16$). Therefore, \autoref{accept:c-availability} can be interpreted as a bitwise AND operation on two such words, while the search for the first $1$ bit in \autoref{accept:f-availability} resolves to one Bit Scan Forward (BSF) operation in x86 instruction set. Both of these operations take one clock cycle in an Intel CPU~\cite{intel-doc}. 
% the computational complexity for processing one proposal is $O(1)$. 
% The overall computational complexity for this accepting phase at an output port is 
% $O(1)$ on average and can be made $O(1)$ even in the worst case using the same technique as used in~\cite{Gong2017QPS}. 
% although in theory an output port can receive up to $N$ proposals. 
% This is because the probability for an output port to receive 
% because the the number of proposals to process can be bounded by $O(1)$. 
% Although in theory, an output port could receive up to $N$ proposals from different input ports, in practice, it can drop all subsequent proposals beyond the first three of them without significantly degrading the matching quality.

% \medskip
% \noindent
% {\bf Message Complexity.}   
% The message complexity of each ``propose-accept'' iteration in SB-QPS is no more than $\big{(}(T\!+\log_2W)\!+\!T\log_2T\big{)}$ bits per input or output port, where $W$ is the largest possible VOQ length. That is because each input/output port transmits no more than one message with $T\!+\log_2W$ bits (a $T$-bit-long bitmap and a VOQ length with $\log_2W$ bits) during the proposing phase and no more than $T$ messages each with $\log_2 T$ bits during the accepting phase.  


We have considered and experimented with another accepting strategy: accepting as many as possible proposals, which we refer to as 
{\it Maximum Fit Accepting} (MFA). Unlike FFA that tries to accommodate proposals one after another during each of the $T$ iterations, 
in each iteration, MFA considers all proposals 
jointly and maximizes the number of proposals that can be accepted. Intuitively, MFA would produce better 
matchings than FFA, however, we found, through experimental evaluation, that MFA generally 
has negligible (throughput and/or delay) performance gains over FFA. Therefore, we prefer FFA over MFA, since FFA has a much lower 
computational complexity. 


\subsection{SW Switching Framework}\label{subsec:sws}

% In this section, we present the SW switching framework. 
The SW switching framework can be viewed as a combination 
of the regular and the batch switching frameworks. On one hand, this framework, like batch switching, allows the 
matching computation (during each time slot $t$) to optimize for multiple consecutive time slots, 
say time slots $t$, $t\!+\!1$,$\cdots$, $t\!+\!T\!-\!1$. In other words, in an SW switching algorithm, the goal 
is also to pack the $TN$ cells in the corresponding joint calendar. On the other hand, this framework, like 
regular switching, produces one matching per time slot. More precisely, at the end of time slot $t$, the row in 
the joint calendar corresponding to time slot $t$ will be removed from the joint calendar and used to switch 
packets. At the same time, an empty row (all cells are ``--'') for time slot $t\!+\!T$ is added to the joint calendar as 
the last row. Clearly, in an SW switching algorithm, each row (matching) in the joint calendar can have 
up to $T$ opportunities (one per time slot) to be optimized (or refined). Therefore, these matchings can have higher qualities than 
those produced by regular switching algorithms. 

\subsection{Sliding Window QPS (SW-QPS)} \label{subsec:sw-qps} 

% In order to further reduce batching delay, Sliding Window Switching breaks the boundary of batches: By the ``student" analogy, at each time slot, one class of senior students graduate, while another class of freshmen are enrolled in the joint calendar. SW switching is able to output one matching per time slot, because in contrast to batch switching algorithms that pack the batch collectively, \autoref{alg:accept} greedily refines each matching in the joint calendar. In this manner, after a matching stays in the joint calendar for $T$ time slots, it has sufficiently accommodated the input proposals, has become ready for switching, and should be outputted immediately after that time point for the least possible packet delay. 

% Packing input proposals at the earliest commonly available time slot in \autoref{alg:accept} is not only delay optimal but also throughput optimal for greedy heuristics. It is obvious that the earliest time slots will leave the joint calendar first and have the least delay. Moreover, packing the earliest time slot leaves as many empty positions as possible on the other side of the joint calendar for future proposals. We are aware that schemes based on max-cardinal bipartite matching may accommodate more proposals than \autoref{alg:accept} for a particular iteration, but such schemes have a complexity of $O(T^{5/2})$ \cite{HopcroftKarp1973MSM}, which is not suitable for our algorithm.

The SW-QPS algorithm is a simple adaption of SB-QPS into the SW switching framework described in~\autoref{sec:sws}. 
% In each time slot $t$, each input port first sends a proposal to an output port,   
% attaching the length of the corresponding VOQ and its availability bitmap, according to the QPS proposing strategy; 
% each output port then accepts one or more proposals to pack the joint calendar according to the FFA strategy 
% described in~\autoref{alg:accept}. 
More precisely, SW-QPS is also a parallel iterative algorithm, each iteration of which is identical to that of SB-QPS. 
The only difference, caused by this adaption, is that, the joint calendar in SW-QPS slides over the time line 
(one time slot per iteration) to ``capture'' the schedules 
of $T$ (consecutive) time slots starting from the current one (or in other words, these $T$ time slots are 
different from one iteration to another) in each of the $T$ iterations, whereas in SB-QPS, the joint calendar captures the 
schedules for the same $T$ time slots ({\it i.e.,} the $T$ time slots in the current batch) during all the $T$ iterations. 

% after an iteration (say the iteration during time slot $t$), \textcolor{green}{the only difference is due to SW switching}
% the earliest row (the row corresponding to time slot $t$) of the 
% joint calendar is ``removed'' and used to transmit packets at the end of time slot $t$, and 
% meanwhile, an empty row is added to the joint calendar as the matching for time slot $t\!+\!T$. 

% \begin{figure}
% \centering
% \includegraphics[width=0.86\columnwidth]{figures/examples/sb-vs-sw}
% \caption{An illustrative example: SB-QPS vs. SW-QPS.}\label{fig:sb-vs-sw}
% \Description{The solid tables are the joint calendars that are being packed or to be packed. The dashed rows are the final matchings. 
% Here we assume the batch size $T$=2 and $\tau$ is the beginning time slot of a batch. $\tau^-$ (or $\tau^+$) means the beginning (or the end) of the time slot $\tau$.}
% \end{figure}

% \autoref{fig:sb-vs-sw} compares SB-QPS with SW-QPS using a simple example. In this example, we assume that the batch size 
% $T$=2 and time slot $\tau$ is the first time slot of a batch. Note that $\tau^-$ (or $\tau^+$) suggests the beginning (or the end) \textcolor{green}{compared with +/-, I would rather say in SW switching, the movement of the sliding window happens after the two phases in each iteration, so the beginning of each time slot is the same as the end of the last one.}
% of time slot $\tau$. In~\autoref{fig:sb-vs-sw}, the solid tables are the joint calenders that are being or to be packed, whereas 
% the dashes rows are the final matchings. The highlighted (in bold font) rows are the final matchings that are used 
% to transmit packet during corresponding time slots. As shown in~\autoref{fig:sb-vs-sw}, each row (matching) in both SB-QPS and 
% SW-QPS are ``refined'' twice thus have similar quality. 

Though both SW-QPS and SB-QPS have the lowest possible per-port computational complexity 
({\it i.e.}, $O(1)$), We prefer SW-QPS over SB-QPS for the following two reasons. 
First, SW-QPS produces matchings in 
a more timely manner so that it does not suffer from the batching delay. As a result, the delay performance of 
SW-QPS is generally better than, and, when the traffic is low or moderate, significantly better than, that of SB-QPS. 
Second, the throughput performance of SW-QPS is generally better than that of SB-QPS. 
Both will be shown in the next section. 
% SB-QPS has to 
% maintain $2T$ matchings: $T$ matchings for the schedules calculated in the previous batch and 
% $T$ matchings to be calculated in the current batch. 
% Therefore, it requires $2T\cdot\log_2 N$ bits of memory per output port. 
% SW-QPS only needs to maintain $T$ matchings. Thus, SW-QPS has much less memory overhead. 

==> sections/scheme.tex <==

% from qpsr
\section{Queue Proportional Sampling}\label{sec:qps}
Queue Proportional Sampling (QPS) was used in~\cite{Gong2017QPS} as an ``add-on'' to augment other switching algorithms as follows.  It generates a starter matching, which is then
populated ({\it i.e.}, adding more edges to it) and refined, by other switching algorithms such as iSLIP~\cite{McKeown99iSLIP} and SERENA~\cite{GiacconePrabhakarShah2003SERENA}, into a final matching.
%Two such augmented switching algorithms
%were proposed in~\cite{Gong2017QPS}:  QPS-iSLIP and QPS-SERENA.
To generate such a starter matching, QPS needs to run only one iteration, 
which
%, \hlb{as mentioned earlier in~\autoref{sec:intro}},  
consists of two phases, namely,
a proposing phase and an accepting phase. \textbf{In this paper, we will use the proposing phase of QPS, so}
% The computational and communication complexities of QPS ({\it i.e.}, this single iteration)
% are both $O(1)$, as we will elaborate next.
we briefly describe it in this section for this paper to be self-contained.

In the proposing phase, each input port proposes
to {\it exactly one} output port -- decided by the QPS strategy
-- unless it has no packet to transmit.
Here we will only describe the operations
at input port $1$;  that at any other
input port is identical.
Like in~\cite{Gong2017QPS}, we denote by $m_1,m_2,\cdots,m_N$
the respective queue lengths of the $N$ VOQs at input port $1$,
and by $m$
their total ({\it i.e.}, $m \!\triangleq\!\sum_{k=1}^N m_k$).
Input port 1 simply samples an output
port $j$ with probability $\frac{m_j}{m}$,
{\it i.e.,} proportional to $m_j$, the length of the corresponding VOQ (hence the name QPS);
it then proposes to output port $j$, with the value $m_j$ that will be used in the next
phase.
The computational complexity of this QPS operation, carried out using a simple data structure proposed in~\cite{Gong2017QPS},
is $O(1)$ per (input) port.   
% The communication complexity of this phase is $\log W$ bits per port ($W$ is the maximum possible VOQ length), which can be viewed as a constant (independent of $N$).

%where $W$ is the maximum possible length of a VOQ (in number of cells).
%In almost all conceivable real-world switching scenarios, we can consider $\log W$ to be $O(\log N)$
\section{Schemes}\label{sec:scheme}
In this section, we present two schemes, called Small Batch QPS (SB-QPS) and Sliding Window QPS (SW-QPS). SB-QPS is a batch scheduling algorithm proposing in the QPS manner, while SW-QPS is the combination of QPS proposing with Sliding Window Switching, improving SB-QPS for better delay and throughput performances.
\subsection{SB-QPS}

Since the batch-computation of these $T$ matchings
often has lower time complexity than
$T$ independent matching computations, the amortized (over the $T$ time slots) time complexity of a batch switching
algorithm is often lower than that of a regular switching algorithm.  
It is desirable for this $T$ to  be small because the average packet delay is at least $T$:  
A packet arriving at
the beginning of a batch has to wait till at least the beginning of the next batch to be switched.
%Exacerbating this problem, the frame size $T$ is quite large and grows as at least $O(\log N)$ in almost all existing frame-based algorithms for reasons
%that we will explain in ...

\textbf{JM}
Batch switching algorithms have the advantage of lower amortized time complexity over running $T$ independent computations of a regular switching algorithm, but they pay large delays: packets arriving uniformly from $t+1$ to $t+T$ must wait for switching until $t+T$, the finish time of the current batch, resulting in an average batching delay of at least $T/2$ that is linear to batch size.\textbf{may be moved to motivation}

Many existing batch switching algorithms use big batches (e.g. the batch size of \cite{Aggarwal2003EdgeColoring} is $\omega(n^2$)) and consequently suffer from large batching delays. Therefore, aiming for less packet delay, it is desirable to reduce batch size without sacrificing much throughput.

% proposal
\textbf{The computation of a batch consists of multiple iterations of message exchanges, one iteration for a time slot.} Each iteration (say in the $t^{th}$ time slot of a batch, $1\leq t \leq T$) consists of two phases, namely, a QPS-proposing phase and an accepting phase.
\textcolor{green}{[JM: symbol $t$ is not clear at this point]}

\medskip
\noindent
{\bf Proposing phase.}
In this phase, each input port proposes to exactly one output port in the QPS manner.  In each proposal, the input port specifies its availability calendar during the previous $t-1$ time slots, encoded as a $(t-1)$-bit bitmap, \textbf{with a 1-bit for an available slot and a 0-bit for an occupied slot}. 

\medskip
\noindent
{\bf Accepting phase.}  
When an output port receives multiple proposals, it accommodates the proposals one by one ordered by 
their corresponding VOQ lengths.  For each proposal, it compares its own availability 
during the first $t$ time slots (i.e., up to ``now") with that of the input port, and pair with the input port at the earliest time slot during which both are available.  

\textcolor{green}{Dangling Sentences:}
The $t^{th}$ iteration refines the matchings in the first $t$ time slots of the joint calendar.

\medskip
\noindent
{\bf Complexity Analysis} The time complexity for comparing two availability calendars seems to be $O(t)$ at first sight, but in fact there is an $O(\log t)$ implementation: we can perform an AND operation of these two bitmaps, and then find the earliest commonly available slot with a priority encoder with $O(\log t)$ layers.

\textbf{QPS} %The computational complexity of this accepting strategy is $O(1)$ in practice although in theory an output port could receive up to $N$ proposals and have to compare their accompanying VOQ lengths. 
\textbf{The number of proposals received by each output is $O(1)$ in practice although it might be $O(N)$ in worst case.}  This is because the probability 
for an output port to receive proposals from more than several (say $3$) input ports is tiny, and even if this 
rare event happens, the output port can ignore/drop all proposals beyond the first several (say $3$) 
without affecting the quality of the final matching much.  In our evaluations, we indeed set this threshold to $3$.

Multiplying the complexity of each proposal by the number of proposals, the time complexity of the accepting phase at each output port is $O(\log T)$ in general.

\subsection{Sliding Window Scheduling}
With SB-QPS, the batching delay can be limited to a small constant $T$, but it is still a major component of packet delay under low traffic loads. (A typical value of $T$ is $30$ time slot, while average delay is below $1$ slot under normalized load $0.5$.)

The primary idea to reduce batching delay is to break the boundary of batches. In SB-QPS, we have already designed the accepting phase to pack proposals at the earliest commonly available time slot, but the problem is that they have to wait until the beginning of next batch to become ready for switching. Actually, we observe that the ``earliest commonly available time slot matching" does not need \textbf{monolithic} batches to compute, but can be incrementally refined by the unit of each time slot. 

This leads to the idea of Sliding Window Switching: at each time slot, the matching in the earliest slot of the joint calendar matures and leaves for switching, while an empty slot is added to the tail of the availability calendar. In this manner, a matching stays in the joint calendar for $T$ time slots, which is considered sufficient for accommodating proposals, and becomes ready for switching immediately after that for the least possible packet delay. Towards the end of its stay, it becomes one of the earliest time slots in the joint calendar and gains a high priority of accommodating proposals. Therefore, the choice of the earliest commonly available time slot to pack proposals is not only delay optimal but also throughput optimal: leaving as many empty positions as possible \textbf{at the far side} of the joint calendar for future proposals.

The availability calendar for SW-QPS proposals is always of fixed length, containing $T$ bits for the next $T$ time slots to come. The benefits of fixed length proposals are \textbf{higher hardware utilization} and higher throughputs because there are more positions to pack input proposals than SB-QPS.

Here we specify the scheme of the two phases of SW-QPS. Despite the differences in the availability calendar and the timing when matchings mature, the two phases of SW-QPS in each iteration resemble SB-QPS. 

\medskip
\noindent
{\bf Proposing phase.}
Every input port also proposes in the QPS manner, specifying its availability calendar for the next $T$ time slots with a $T$-bit bitmap. 

\medskip
\noindent
{\bf Accepting phase.}
In the accepting phase, as in SB-QPS, multiple proposals are accommodated one by one ordered by 
their corresponding VOQ lengths. For each proposal, the output port pairs with the input port at the earliest commonly available time slot. 

\medskip
\noindent
{\bf Complexity Analysis.}
The message complexity of SW-QPS is $O(T+W)$, where $W$ is the number of bits used to encode VOQ lengths, and the time complexity of SW-QPS is $O(\log T)$ for each port, the same as SB-QPS, if the availability calendar is implemented with a circular queue and the accepting phase is implemented with a priority encoder with (circular) programmable priorities. In simulation, we can achieve about 90\% throughput over various traffic patters with a small batch size $T=16$ and no penalty of batching delays.





==> sections/sliding-window.tex <==
\section{Sliding-Window (SW) Switching }\label{sec:sws} 

In this section, we first describe the Sliding-Window (SW) switching in detail. 
% Then, we explain how SW 
% switching eliminates the batching delays in batch switching algorithms. 
We next compare SW switching with 
Captured-Frame (CF) switching~\cite{rojas2007frame}, another ``batch switching'' approach that can be used to eliminate the 
batching delays in batch switch algorithms. 

\subsection{SW Switching: A New Batch Switching Approach}\label{subsec:sws}

A straightforward idea to overcome the batching delay issue of a batch 
switching algorithm is to let the algorithm to 
output one matching per time slot during the current batch 
instead of producing $T$ matchings at the end of this batch. 
Unfortunately, in most of the existing 
batching algorithms, these $T$ matchings are computed and 
refined together, and can only have high enough quality at the end of 
each run of the algorithms. In other word, naively outputting one 
matching per time slot results in lower-quality matchings. 

% % may not be required
% {\bf Compare with other approaches!}  
% We note that an alternative approach to overcome this batching delay issue 
% is to adapting batch size dynamically according to traffic conditions, like 
% what is done in~\cite{rojas2007frame}. 
% Such an approach is not preferable because of two major reasons. 
% On one hand, it is not easy to measure the traffic accurately. 
% On the other hand, dynamically adapting batch size requires one extra round of message 
% exchange to determine the batch size before starting the switching algorithm, which 
% incur extra communication overhead and is difficult to implement in a distributed manner. 

% \textbf{JM: It is easy to measure the traffic load on each VOQ, but it is difficult to summarize these queue lengths to select a suitable batch size for all input ports. The throughput performance of \cite{rojas2007frame} relys on its 3-round request-grant-accept scheme, which has higher message and time complexity.}

In this work, we propose a new batch switching approach to overcome 
the batching delay issue. We call it the Sliding Window (SW) switching.  
Like a traditional batch switching algorithm, a SW switching algorithm 
packs the joint calendar with $TN$ cells for all input and output ports during 
each run. However, each run of a SW switching 
algorithm takes only a time slot (instead of a batch) and at the end of each run, 
the first row (say  the $t^{th}$ row) of 
the joint calendar is used to transmit the packets during this time slot and 
removed from the joint calendar. 
At the same time, a new row (an empty schedule for time slot $t+T$) corresponding 
to the schedule of time slot 
$t+T$ is added as the last one of the joint calendar. 
With such a switching framework, each schedule (each row of the joint calendar), 
after its initialization (adding \textcolor{green}{being added} to the 
joint calendar), is refined by $T$ runs of the switching algorithm. Thus, 
each matching has the same or even higher quality 
as those computed by the traditional batching switching algorithms. 
\autoref{fig:batch-vs-sw} shows compares the traditional batch switching with the SW switching. 


As in the left side of Figure \ref{fig:batch-vs-sw}, each batch in Batch Switching contains $T$ consecutive time slots and different batches do not overlap. The scheduler packs incoming packets into Batch 1 during the period $t+1$ to $t+T$. At time slot $t+T$, all $T$ matchings in Batch 1 become ready for switching and the scheduler moves to Batch 2. 

In Sliding Window Switching, however, consecutive batches overlap on $T-1$ time slots. At time slot $t+1$, the first time slot of the Batch 1 becomes ready for switching and leaves the batch. All other time slots then join Batch 2, together with a new empty time slot appended to the end of Batch 2.

In contrast to Batch Switching, Sliding Window Switching allows new packets to directly jump to the first time slot of the joint calendar and to be switched immediately, without having to wait for the beginning of next batch, as long as there are enough empty positions in the joint calendar. This flexible behavior, having one matching ready at each time slot, is crucial to the reduction of batching delay to a $O(1)$ order under low traffic loads. Meanwhile, Sliding Window Switching is simple to implement and preserves the advantage of of Batch Switching: achieving high throughput with low complexity. 

{\bf Maybe the following section should be moved to the related work}
\subsection{SW Switching vs. CF Switching}\label{subsec:sw-vs-cf}

As we have shown, SW switching is a batching-delay-free batch switching approach. 
In the literature, the only other batching-delay-free batch switching approach that we are aware of is CF switching~\cite{rojas2007frame}. 
CF switching is an approach to dynamically select proper \textcolor{green}{the} batch size for each input-output pair based on input loads, which was 
designed to boost the throughput performance of certain parallel iterative maximal-size switching schemes ({\it e.g.,} PIM~\cite{Anderson1993PIM} and iSLIP~\cite{McKeown99iSLIP}). 

Unlike in a traditional batch switching algorithm and a SW switching algorithm, in a CF switching algorithm, the batch size for 
different input-output pairs could be different. More precisely, in a CF switching algorithm, each input-output pair between the $i^{th}$ input port and the $j^{th}$ output port 
maintains a counter $c_{i,j}$ that captures the number of remaining time slots in the current batch of this input-output pair. When this 
counter $c_{i,j}$ decreases to zero ({\it i.e.,} the end of a batch), 
the batch size of a new batch is set to the length of the $j^{th}$ VOQ at input port $i$.  
% and the counter $c_{i,j}$ is updated to the new batch size. 
During each time slot, a matching (schedule) is computed 
with a parallel iterative maximal-size matching algorithm and used to switch packets for this time slot (thus batching-delay-free). Here, the parallel iterative algorithm is slightly different from its regular-switching counterpart in that it gives higher priority to the input-output pair whose counter $c_{i,j}$ 
at the previous time slot is larger than $1$ (or in other words, the current time slot is not the beginning of a new batch). Doing so, 
the CF switching algorithm roughly achieves to provide service to input-output pairs in proportion to their arrival rates, or in other words, 
it makes ``weight-oblivious'' switching algorithms ({\it e.g.} PIM or iSLIP) ``weight-aware''. Therefore, it retains the good performance 
under uniform traffic and light traffic, yet achieves higher throughput under non-uniform traffic. 

Both SW switching and CF switching resolve the batching delay issue of the traditional batching switching algorithms. However, there are three 
key differences. First, in a CF switching algorithm, $N^2$ counters are required to capture the number of remaining time slots for 
the $N^2$ input-output pairs, which makes it difficult to scale to switches with large $N$. Second, CF switching achieves high throughput 
by making ``weight-oblivious'' switching algorithms ``weight-aware'', where the batch concept is just used for poritorize \textcolor{green}{prioritize} input-output 
pairs, whereas SW switching achieves high throughput by refining each matching again and again before it is used to switch packets. Last, unlike in SW switching algorithms, there is only one matching being computed during each time slot in a CF switching algorithm.


==> sections/sw-switching.tex <==
\section{SW Switching Framework}\label{sec:sws}

% In this section, we present the SW switching framework. 
The SW switching framework can be viewed as a combination 
of the regular and the batch switching frameworks. On one hand, this framework, like batch switching, allows the 
matching computation (during each time slot $t$) to optimize for multiple consecutive time slots, 
say time slots $t$, $t\!+\!1$,$\cdots$, $t\!+\!T\!-\!1$. In other words, in an SW switching algorithm, the goal 
is also to pack the $TN$ cells in the corresponding joint calendar. On the other hand, this framework, like 
regular switching, produces one matching per time slot. More precisely, at the end of time slot $t$, the row in 
the joint calendar corresponding to time slot $t$ will be removed from the joint calendar and used to switch 
packets. At the same time, an empty row (all cells are ``--'') for time slot $t\!+\!T$ is added to the joint calendar as 
the last row. Clearly, in an SW switching algorithm, each row (matching) in the joint calendar can have 
up to $T$ opportunities (one per time slot) to be optimized (or refined). Therefore, these matchings can have higher qualities than 
those produced by regular switching algorithms. 






% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.295\textwidth]{figures//IQ-sched-graph/sliding-schedule}
% 	% \caption{An illustration of the joint calendar of Sliding Window switching: The label of each row (matching) is its time slot of completion.}
% 		\caption{The SW scheduling framework.}
% 	\label{fig:batch-vs-sw}
% \end{figure}

% As shown in \autoref{fig:batch-vs-sw}, in contrast to batch switching, as long as there are enough empty positions in the joint calendar, SW switching allows new packets to directly jump to the first row of the joint calendar and to be switched immediately, without having to wait for the beginning of next batch. This flexible behavior, having one matching ready at each time slot, is crucial to the reduction of batching delay to a $O(1)$ order under low traffic loads. Meanwhile, Sliding Window Switching is simple to implement and preserves the advantage of of Batch Switching: achieving high throughput with low complexity. 
